Automatic Hardware Pragma Insertion in High-Level Synthesis: A Non-Linear Programming Approach

High-Level Synthesis enables the rapid prototyping of hardware accelerators, by combining a high-level description of the functional behavior of a kernel with a set of micro-architecture optimizations as inputs. Such optimizations can be described by inserting pragmas e.g. pipelining and replication of units, or even higher level transformations for HLS such as automatic data caching using the AMD/Xilinx Merlin compiler. Selecting the best combination of pragmas, even within a restricted set, remains particularly challenging and the typical state-of-practice uses design-space exploration to navigate this space. But due to the highly irregular performance distribution of pragma configurations, typical DSE approaches are either extremely time consuming, or operating on a severely restricted search space. This work proposes a framework to automatically insert HLS pragmas in regular loop-based programs, supporting pipelining, unit replication, and data caching. We develop an analytical performance and resource model as a function of the input program properties and pragmas inserted, using non-linear constraints and objectives. We prove this model provides a lower bound on the actual performance after HLS. We then encode this model as a Non-Linear Program, by making the pragma configuration unknowns of the system, which is computed optimally by solving this NLP. This approach can also be used during DSE, to quickly prune points with a (possibly partial) pragma configuration, driven by lower bounds on achievable latency. We extensively evaluate our end-to-end, fully implemented system, showing it can effectively manipulate spaces of billions of designs in seconds to minutes for the kernels evaluated.

==> setup/macros.tex <==
\newcommand{\SET}[1]{{\ensuremath{\mathit{#1}}}}
\newcommand{\SETFULL}[3]{{\ensuremath{\mathit{#1}^{#2}_{#3}}}}

\newcommand{\MAP}[1]{{\ensuremath{\mathbf{#1}}}}
\newcommand{\MAPFULL}[3]{{\ensuremath{\mathbf{#1}^{#2}_{#3}}}}

\newcommand{\POINT}[1]{{\ensuremath{\bm{#1}}}}
\newcommand{\POINTINSET}[2]{{\ensuremath{{\bm{#1}} \in {#2}}}}


\newcommand{\MAPSTO}{{\ensuremath{\rightarrow}}}

\newcommand{\CARD}{{\ensuremath{\#}}}

\newcommand{\MAPCOMPOSE}{~{\ensuremath{\circ}}~}

\newcommand{\MAPRANGE}{{\ensuremath{\text{range}}}\xspace}

\newcommand{\MAPDOMAIN}{{\ensuremath{\text{domain}}}\xspace}

\newcommand{\INTERSECT}{~{\ensuremath{\cap}}~}

\newcommand{\UNION}{~{\ensuremath{\cup}}~}

\newcommand{\DIFFERENCE}{~{\ensuremath{-}}~}

\newcommand{\LEXMAX}{~{\ensuremath{\mathbf{lexmax}}}~}
\newcommand{\LEXMIN}{~{\ensuremath{\mathbf{lexmin}}}~}



==> setup/setup.tex <==
%%% LNP

\usepackage[utf8]{inputenc}


%% Some recommended packages.
\usepackage{booktabs} % For formal tables
\newcommand{\cL}{{\cal L}}
%\usepackage{courier}            % standard fixed width font
%\usepackage[scaled]{helvet} % see www.ctan.org/get/macros/latex/required/psnfss/psnfss2e.pdf
\usepackage{url}                  % format URLs
\usepackage{paralist}
\usepackage{enumitem}      % adjust spacing in enums
%\usepackage[colorlinks=true,allcolors=black,breaklinks,draft=false]{hyperref}   % hyperlinks, %including DOIs and URLs in bibliography

%% self include package
%\usepackage[cmex10]{amsmath}
\usepackage{breakurl}
\usepackage{amsfonts}
%% \usepackage{subfig}
\usepackage[caption=false]{subfig}

%\usepackage[tight,footnotesize]{subfigure}
\usepackage{stfloats}
\hyphenation{op-tical net-works semi-conduc-tor}

% For code
\usepackage{clrscode}
\usepackage{xcolor}
\usepackage{listings}
\usepackage{tikz}
%\usepackage{algpseudocode}
%% \usepackage{algorithm}
%% \usepackage{algorithmic}
%% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%% \renewcommand{\algorithmicensure}{\textbf{Output:}}

% \usepackage[noend]{algorithm2e}/
% \usepackage[ruled]{algorithm2e}
\usepackage[linesnumbered,lined,boxed,commentsnumbered,noend,ruled,longend]{algorithm2e}


\usepackage{graphicx} 	% For figures
%\usepackage{subfigure}
\usepackage{mathtools}	% For math function
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\usepackage{multirow}	% For table

%\renewcommand{\baselinestretch}{0.95}
%\setlength{\abovecaptionskip}{3pt}
%\setlength{\belowcaptionskip}{-8pt}

\usepackage{amsmath}
\usepackage{amsthm}

%%% LNP: packages added.
\usepackage{bm}
\usepackage{xspace}
%\usepackage{amssymb}
%%% !LNP

%%% LNP: file containing macros for sets, relations, etc.
% \input{setup/macros}
%%% !LNP


%\newtheorem{definition}{Definition}
%\newtheorem{observation}{Observation}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}

\newcommand{\ignore}[1]{}
\newcommand{\code}[1]{{\ttfamily\footnotesize #1}}
\newcommand\todo[1]{{\color{red}\bf [TODO: #1]}}

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\usepackage{caption}


\captionsetup[subfloat]{font={small,tt}}

\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\sffamily\footnotesize,        % the size of the fonts that are used for the code
  basicstyle=\ttfamily\footnotesize,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={--*}{*--},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  frame = none,
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\textbf,       % keyword style
  language=C++,                 % the language of the code
  morekeywords={*,assert,in,NIL,@initialize,@verify,@terminate,def,...},            % if you want to add more keywords to the set
  %numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  %numbersep=3pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
  %rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  %stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                   % show the filename of files included with \lstinputlisting; also try caption instead of title
  belowskip={-5ex},
  aboveskip={0ex}
}

\usepackage{rotating}
%%%%%
%%% LNP Macros.
\usepackage{balance}
\def\polycache{PolyCache\xspace}
\def\polyvul{PolyVul\xspace}
\def\polycheck{PolyCheck\xspace}
%%%%%

% Macros for language spec
\newcommand{\anywhere}[1]{\ensuremath{\mbox{#1}}}
\newcommand{\msf}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\bsf}[1]{\anywhere{\sffamily{\bfseries{#1}}}}
\newcommand{\mtt}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\mrm}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\ttt}[1]{\ensuremath{\mbox{\texttt{#1}}}}
\newcommand{\alt}{\ \mid\ }
\newcommand{\AffineExpr}{\ensuremath{\mtt{AffineExpr}}}
\newcommand{\AffineCond}{\ensuremath{\mtt{AffineCond}}}
\newcommand{\LowerBound}{\ensuremath{\mtt{LowerBound}}}
\newcommand{\UpperBound}{\ensuremath{\mtt{UpperBound}}}
\newcommand{\ArrayIndex}{\ensuremath{\mtt{ArrayIndex}}}
\newcommand{\Stmts}{\ensuremath{\mtt{Stmts}}}
\newcommand{\Programs}{\ensuremath{\mtt{Programs}}}
\newcommand{\ffor}[3]{\bsf{for }\ensuremath{{#1} = {#2}} \bsf{ to } \ensuremath{#3}}

\newcommand{\lexmin}{{$\mathit{lexmin}$}}
\newcommand{\lexmax}{{$\mathit{lexmax}$}}
\newcommand{\FirstWriter}{{$\mathit{FirstWriter}$}}
\newcommand{\NextWriter}{{$\mathit{NextWriter}$}}
\newcommand{\WriterBeforeRead}{{$\mathit{WriterBeforeRead}$}}

%\usepackage[numbers]{natbib}
\usepackage{ragged2e}
\usepackage{array}
\newcolumntype{R}[1]{>{\RaggedLeft\arraybackslash}p{#1}}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}


\usepackage[utf8]{inputenc}
\usepackage{listings}
\usepackage{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

% \lstdefinestyle{mystyle}{
%     backgroundcolor=\color{backcolour},   
%     commentstyle=\color{codegreen},
%     keywordstyle=\color{magenta},
%     numberstyle=\tiny\color{codegray},
%     stringstyle=\color{codepurple},
%     basicstyle=\ttfamily\footnotesize,
%     breakatwhitespace=false,         
%     breaklines=true,                 
%     captionpos=b,                    
%     keepspaces=true,                 
%     numbers=left,                    
%     numbersep=5pt,                  
%     showspaces=false,                
%     showstringspaces=false,
%     showtabs=false,                  
%     tabsize=2,
%     xleftmargin=1.8em
% }

% \lstset{style=mystyle}

%%% LNP: adding usual setup/packages.
\input{setup/macros}
%%%%%%%%%%%%%%%%%% !LNP

\usepackage{multirow}

\lstset{ %
	backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
	%basicstyle=\sffamily\footnotesize,        % the size of the fonts that are used for the code
	basicstyle=\ttfamily\footnotesize,        % the size of the fonts that are used for the code
	breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
	breaklines=true,                 % sets automatic line breaking
	captionpos=b,                    % sets the caption-position to bottom
	deletekeywords={...},            % if you want to delete keywords from the given language
	escapeinside={--*}{*--},          % if you want to add LaTeX within your code
	extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
	%frame=single,                    % adds a frame around the code
	frame = none,
	keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
	keywordstyle=\textbf,       % keyword style
	language=C++,                 % the language of the code
	morekeywords={*,assert,in,NIL,@initialize,@verify,@terminate,def,...},            % if you want to add more keywords to the set
	%numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
	%numbersep=3pt,                   % how far the line-numbers are from the code
	numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
	%rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g., comments (green here))
	showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
	showstringspaces=false,          % underline spaces within strings only
	showtabs=false,                  % show tabs within strings adding particular underscores
	%stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
	stringstyle=\color{mymauve},     % string literal style
	tabsize=2,                       % sets default tabsize to 2 spaces
	title=\lstname,                   % show the filename of files included with \lstinputlisting; also try caption instead of title
	belowskip={-5ex},
	aboveskip={0ex}
}


%%% !LNP


%\usepackage[dvipsnames,table,xcdraw]{xcolor}
%\usepackage[american]{babel}
%\settopmatter{printfolios=true,printccs=false,printacmref=false}
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
%\usepackage{cite}
%% \usepackage[numbers]{natbib}
\usepackage{caption}
\usepackage{amsmath,amsfonts}
% \usepackage{algorithmic}
%% \usepackage[ruled,vlined]{algorithm2e}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{hyperref}
\usepackage{listings}
\usepackage{placeins}
\usepackage{url}
\usepackage{csvsimple}
\usepackage{adjustbox}
\usepackage{float}
\usepackage{array}
\usepackage{titlesec}
\usepackage{units}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\usepackage{paralist}
\usepackage{balance}

\usepackage{enumitem}      % adjust spacing in enums
%\usepackage[colorlinks=true,allcolors=black,breaklinks,draft=false]{hyperref}   % hyperlinks, %including DOIs and URLs in bibliography

%% self include package
%\usepackage[cmex10]{amsmath}
\usepackage{breakurl}


%%% from marcos' thesis:
\usepackage{backnaur}
\usepackage{tikz}
\usetikzlibrary{shapes.geometric,fit}
\usepackage{subfiles}
\usepackage{soul}
\usepackage{lscape}
% \usepackage[ruled,lined,boxed,linesnumbered]{algorithm2e}
\usepackage{svg}
\usepackage{adjustbox}
\usepackage{float}
\usepackage{placeins}
\usetikzlibrary{arrows}
\usepackage{bookmark}
\usepackage{epigraph}
\renewcommand{\epigraphflush}{flushleft}

\definecolor{crimson}{rgb}{0.86, 0.08, 0.24}
\definecolor{crimsonglory}{rgb}{0.75, 0.0, 0.2}
\definecolor{light}{gray}{0.92}
\definecolor{dark}{gray}{0.50}
\definecolor{red}{rgb}{1,0,0}
\definecolor{azure}{rgb}{0, 0.5,1.0}
\definecolor{headertable}{gray}{0.65}
\definecolor{mygray}{gray}{1}


\lstdefinestyle{GACstyle}{
    basicstyle=\footnotesize\ttfamily,
    breakatwhitespace=false,
    breaklines=false,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2,
    xleftmargin=0.035\textwidth,
    language=python,
    linewidth=1.0\textwidth,
    %frame=tb,
    aboveskip=0.5cm,
}

\lstdefinestyle{MinStyle}{
    basicstyle=\footnotesize\ttfamily,
    breakatwhitespace=false,
    breaklines=false,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2,
    xleftmargin=0.035\textwidth,
    language=C,
    linewidth=1.0\textwidth,
    aboveskip=0.5cm,
}

\lstset{style=MinStyle}

\lstdefinestyle{customc}{
  belowcaptionskip=1\baselineskip,
  numbers=left,
  numbersep=8pt,
  stepnumber=1,
  float=tb,
  tabsize=4,
  breaklines=true,
  frame=single,
  xleftmargin=\parindent,
  language=C,
  showstringspaces=false,
  basicstyle=\footnotesize\ttfamily,
  keywordstyle=\bfseries\color{green!40!black},
  commentstyle=\itshape\color{purple!40!black},
  identifierstyle=\color{blue},
  stringstyle=\color{orange},
  morekeywords={\_\_m256i,\_\_m256,\_\_m128,\_\_m128i,\_\_m512,\_\_m512i,defined},
  columns = fullflexible,
}

\lstdefinestyle{customcminipage}{
  belowcaptionskip=1\baselineskip,
  numbers=left,
  numbersep=8pt,
  stepnumber=1,
  tabsize=4,
  breaklines=true,
  frame=single,
  xleftmargin=\parindent,
  language=C,
  showstringspaces=false,
  basicstyle=\footnotesize\ttfamily,
  keywordstyle=\bfseries\color{green!40!black},
  commentstyle=\itshape\color{purple!40!black},
  identifierstyle=\color{blue},
  stringstyle=\color{orange},
  morekeywords={\_\_m256i,\_\_m256,\_\_m128,\_\_m128i,\_\_m512,\_\_m512i,defined},
  columns = fullflexible,
}

\lstdefinestyle{custommrt}{
  belowcaptionskip=1\baselineskip,
  float=tb,
  numbers=left,
  numbersep=8pt,
  stepnumber=1,
  tabsize=4,
  breaklines=true,
  frame=single,
  xleftmargin=\parindent,
  language=C,
  columns = fullflexible,
}

\lstdefinestyle{customasm}{
  belowcaptionskip=1\baselineskip,
  float=tb,
  numbers=left,
  numbersep=8pt,
  stepnumber=1,
  tabsize=4,
  frame=single,
  xleftmargin=\parindent,
  language=[x86masm]Assembler,
  basicstyle=\footnotesize\ttfamily,
  commentstyle=\itshape\color{purple!40!black},
  identifierstyle=\color{blue},
  stringstyle=\color{orange},
  keywordstyle=\bfseries\color{red!40!black},
  keywordstyle=[1]\bfseries\color{red!40!black},
  morekeywords=[1]{QWORD,PTR,DWORD,YMMWORD,XMMWORD,ZMMWORD},
  deletekeywords=[1]{r1,r2,r3,r4,r5,r6,r7,r8,r9,r10,r11,r12,r13,r14,r15,%
  rax,rcx,rdx,rbx,rsp,rbp,rsi,rdi,rip,eax,ecx,edx,ebx,esp,ebp,esi,edi},
  keywordstyle=[2]\bfseries\color{blue!40!black},
  morekeywords=[2]{%
  r1,r2,r3,r4,r5,r6,r7,r8,r9,r10,r11,r12,r13,r14,r15,%
  rax,rcx,rdx,rbx,rsp,rbp,rsi,rdi,rip,eax,ecx,edx,ebx,esp,ebp,esi,edi,%
  xmm0,xmm1,xmm2,xmm3,xmm4,xmm5,xmm6,xmm7,xmm8,xmm9,xmm10,xmm11,xmm12,xmm13,xmm14,xmm15,%
  ymm0,ymm1,ymm2,ymm3,ymm4,ymm5,ymm6,ymm7},
  alsoletter=[2]{.,0,1,2,3,4,5,6,7,8,9},
  morecomment=[n][\bfseries\color{red!40!black}]{[}{]},
  morecomment=[f][\itshape\color{purple!40!black}][0]{;;},
  literate=*{,}{,}{1},
  columns = fullflexible,
}

\lstdefinestyle{custompython}{
  belowcaptionskip=1\baselineskip,
  float=tb,
  numbers=left,
  numbersep=8pt,
  stepnumber=1,
  tabsize=4,
  frame=single,
  xleftmargin=\parindent,
  language=Python,
  basicstyle=\footnotesize\ttfamily,
  commentstyle=\fontseries{lc}\selectfont\itshape\color{purple!40!black},
  identifierstyle=\color{blue},
  stringstyle=\color{orange},
}


%%% !marcos

\newcommand{\MACVETH}{MACVETH\xspace}
\newcommand{\TOOL}{\MACVETH}
\newcommand{\MARTA}{uBENCHTOOL\xspace}
%\newcommand{\MARTA}{ANALYSISTOOL\xspace}

\newcommand{\macvethfull}{Multi-Architectural C-VEc\-Torizer for HPC applications}
\newcommand{\martafull}{Multi-configuration Assembly pRofiler and Toolkit for performance Analysis}
\newcommand{\mrkvsfull}{Mega-Random Kernel Vector SMT}


%% Before submission, define to this:
% \newcommand{\FIXME}[1]{}
%% During writing, display fixmes:
\newcommand{\FIXME}[1]{\par\textbf{FIXME:~ #1}\par}

\newcommand{\REMARK}[1]{\par\textbf{REMARK:~ #1}\par}


%%%%%%%%%%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}

\newcommand{\myparagraph}[1]{\par\textit{ #1}\xspace}


==> sources/eq.tex <==
\begin{eqnarray}
% \left\{
\label{eq:UF}
 \forall l \in \mathcal{L}, 1 \leq loop_l\_UF \leq TC_l
\\
% \nonumber % to remove the +1 label without equation
% \end{eqnarray}
% \begin{eqnarray}
 % to remove the +1 label without equation
% 
\label{eq:tile}
\forall l \in \mathcal{L}, 1 \leq loop_l\_tile \leq TC_l
\\
% \nonumber % to remove the +1 label without equation
% \end{eqnarray}
% \begin{eqnarray}
 % to remove the +1 label without equation
% 
\label{eq:pip}
\forall l \in \mathcal{L}, loop_l\_pip \in \{0,1\}
\\
% \nonumber % to remove the +1 label without equation
% \end{eqnarray}
% \begin{eqnarray}
% 
\label{eq:cache}
\forall l \in \mathcal{L}, \forall a \in \mathcal{A}, loop_l\_cache\_array_a \in \{0,1\}
\\
% 
\label{eq:one_pip_per_nesteed_loop}
% \begin{cases}
\forall s \in \mathcal{S}, \sum_{l \in \mathcal{L}_s} loop_l\_pip \leq 1
% \end{cases}
\\
% 
\label{eq:uf_divide_tc}
% \begin{cases}
\forall l \in \mathcal{L}, loop_l\_UF \% TC_l == 0
% \end{cases}
\\
% 
\label{eq:tile_divide_tc}
% \begin{cases}
\forall l \in \mathcal{L}, loop_l\_tile \% TC_l == 0
% \end{cases}
\\
\label{eq:dd}
% \begin{cases}
\forall l \in \mathcal{L}, \text{ if } dd_l > 1,  loop_l\_UF \leq d_l
% \end{cases}
\\
% \nonumber % to remove the +1 label without equation
% \end{eqnarray}
% \begin{eqnarray}
% 
\label{eq:fine_grained}
% \begin{cases}
\forall l \in \mathcal{L}, \forall l' \in \mathcal{L}_{above\_l}, loop_l\_pip * loop_{l'}\_UF <= 1
% \end{cases}
\\
% \nonumber % to remove the +1 label without equation
% \end{eqnarray}
% \begin{eqnarray}
% 
\label{eq:max_part2}
% \begin{cases}
\forall s \in \mathcal{S},  \prod_{l \in {L}_s} loop_l\_UF \leq MAX\_PARTITIONING
% \end{cases}
\\
% 
% 
\label{eq:dsp_optimistic}
% \begin{cases}
% & DSPs\_used_{optimistic} = \\
%     & \sum_{op \in \{+,-,*,/ \}} \max_{s \in \mathcal{S}}(DSP_{s_{op}} / II_s)
% \end{cases}
 DSPs\_used_{optimistic} = 
     \sum_{op \in \{+,-,*,/ \}} \max_{s \in \mathcal{S}}(DSP_{s_{op}} / II_s) \leq DSP_{available}
\\
% 
\label{eq:on_chip}
% \begin{cases}
     \sum_{a \in \mathcal{A}} \sum_{l \in \mathcal{L}} loop_l\_cache\_array_a  \times footprint\_array_a\_loop_l \leq Mem
% \end{cases}
\\
\label{eq:max_part1}
% \begin{cases}
% & 
\forall a \in \mathcal{A}, \forall (d, d') \in \mathbb{N}^2 \text{ with } d \neq d', \forall l \in C_{a_d}, \forall l' \in C_{a_{d'}} ,
% \\
%     & 
    loop_l\_UF \times loop_{l'}\_UF \leq MAX\_PARTITIONING
% \end{cases}
\\
% \nonumber % to remove the +1 label without equation
% \end{eqnarray}
% \begin{eqnarray}
% 
\label{eq:no_cache_under_pip}
% \begin{cases}
% &
\forall p \in \mathcal{P}, \forall lp \in \mathcal{L}^p_{pip}, \forall lbp \in \mathcal{L}_{under\_pip_{lp}}
\forall a \in \mathcal{A}, 
% \\
% &
loop_{lbp}\_cache\_array_a == 0
% \end{cases}
\\
% 
\label{eq:under_pip_fully_unrolled}
% \begin{cases}
\forall p \in \mathcal{P}, \forall lp \in \mathcal{L}^p_{pip}, \forall lbp \in \mathcal{L}_{under\_pip_{lp}},  loop_{lp} \times loop_{lbp}\_UF == loop_{lp} \times TC_{lbp}
\\
% \end{cases}
% \\
\nonumber % to remove the +1 label without equation
\end{eqnarray}

==> sources/eq1.tex <==
\begin{eqnarray}
% \left\{
\label{eq:UF}
 \forall l \in \mathcal{L}, 1 \leq loop_l\_UF \leq TC_l
\\
 % to remove the +1 label without equation
% 
\label{eq:tile}
\forall l \in \mathcal{L}, 1 \leq loop_l\_tile \leq TC_l
\\
 % to remove the +1 label without equation
% 
\label{eq:pip}
\forall l \in \mathcal{L}, loop_l\_pip \in \{0,1\}
\\
% 
\label{eq:cache}
\forall l \in \mathcal{L}, \forall a \in \mathcal{A}, loop_l\_cache\_array_a \in \{0,1\}
\\
% 
\label{eq:one_pip_per_nesteed_loop}
% \begin{cases}
\forall s \in \mathcal{S}, \sum_{l \in \mathcal{L}_s} loop_l\_pip \leq 1
% \end{cases}
\\
\nonumber % to remove the +1 label without equation
\end{eqnarray}
\begin{eqnarray}
% 
\label{eq:uf_divide_tc}
% \begin{cases}
\forall l \in \mathcal{L}, loop_l\_UF \% TC_l == 0
% \end{cases}
\\
% 
\label{eq:tile_divide_tc}
% \begin{cases}
\forall l \in \mathcal{L}, loop_l\_tile \% TC_l == 0
% \end{cases}
\\
% 
\label{eq:fine_grained}
% \begin{cases}
\forall l \in \mathcal{L}, \forall l' \in \mathcal{L}_{above\_l}, loop_l\_pip * loop_{l'}\_UF <= 1
% \end{cases}
\\
% 
% 
\label{eq:max_part2}
% \begin{cases}
\forall s \in \mathcal{S},  \prod_{l \in {L}_s} loop_l\_UF \leq MAX\_PARTITIONING
% \end{cases}
\\
% 
% 
\label{eq:dsp_optimistic}
% \begin{cases}
% & DSPs\_used_{optimistic} = \\
%     & \sum_{op \in \{+,-,*,/ \}} \max_{s \in \mathcal{S}}(DSP_{s_{op}} / II_s)
% \end{cases}
 DSPs\_used_{optimistic} = 
     \sum_{op \in \{+,-,*,/ \}} \max_{s \in \mathcal{S}}(DSP_{s_{op}} / II_s)
\\
% 
\label{eq:on_chip}
% \begin{cases}
     \sum_{a \in \mathcal{A}} \sum_{l \in \mathcal{L}} loop_l\_cache\_array_a \times footprint\_array_a\_loop_l \leq Mem
% \end{cases}
\\
\label{eq:max_part1}
\begin{cases}
& \forall a \in \mathcal{A}, \forall (d, d') \in \mathbb{N}^2 \text{ with } d \neq d', \forall l \in C_{a_d}, \forall l' \in C_{a_{d'}} , \\
    & loop_l\_UF \times loop_{l'}\_UF \leq MAX\_PARTITIONING
\end{cases}
\\
% 
\label{eq:no_cache_under_pip}
\begin{cases}
& \forall p \in \mathcal{P}, \forall lp \in \mathcal{L}^p_{pip}, \forall lbp \in \mathcal{L}_{under\_pip_{lp}}
\forall a \in \mathcal{A}, \\
&
loop_{lbp}\_cache\_array_a == 0
\end{cases}
\\
% 
\label{eq:under_pip_fully_unrolled}
\begin{cases}
&\forall p \in \mathcal{P}, \forall lp \in \mathcal{L}^p_{pip}, \forall lbp \in \mathcal{L}_{under\_pip_{lp}}, \\
    & loop_{lp} \times loop_{lbp}\_UF == loop_{lp} \times TC_{lbp} \\
\end{cases}
\\
\nonumber % to remove the +1 label without equation
\end{eqnarray}

==> sources/eq2.tex <==

\begin{multicols}{2}
  \begin{equation}
    \label{eq:UF} \forall l \in \mathcal{L}, 1 \leq loop_l\_UF \leq TC_l \\
  \end{equation}\break
  \begin{equation}
    \label{eq:tile}  \forall l \in \mathcal{L}, 1 \leq loop_l\_tile \leq TC_l \\
  \end{equation}
\end{multicols}

\begin{align}
\begin{split}


\end{split} \\
\begin{split}
\label{eq:pip} & \forall l \in \mathcal{L}, loop_l\_pip \in \{0,1\} \\
\label{eq:cache} & \forall l \in \mathcal{L}, \forall a \in \mathcal{A}, loop_l\_cache\_array_a \in \{0,1\} \\
\end{split} \\
\begin{split}
\label{eq:one_pip_per_nesteed_loop} & \forall s \in \mathcal{S}, \sum_{l \in \mathcal{L}_s} loop_l\_pip \leq 1 \\
\label{eq:uf_divide_tc} & \forall l \in \mathcal{L}, loop_l\_UF \% TC_l == 0 \\
\end{split} \\
\begin{split}
\label{eq:tile_divide_tc} & \forall l \in \mathcal{L}, loop_l\_tile \% TC_l == 0 \\
\label{eq:dd} & \forall l \in \mathcal{L}, \text{ if } dd_l > 1,  loop_l\_UF \leq dd_l \\
\end{split} \\
\begin{split}
\label{eq:fine_grained} & \forall l \in \mathcal{L}, \forall l' \in \mathcal{L}_{above\_l}, loop_l\_pip \cdot loop_{l'}\_UF \leq 1 \\
\label{eq:max_part2} & \forall s \in \mathcal{S},  \prod_{l \in {L}_s} loop_l\_UF \leq MAX\_PARTITIONING \\
\end{split} \\
\begin{split}
\label{eq:dsp_optimistic} & DSPs\_used_{optimistic} = \sum_{op \in \{+,-,*,/ \}} \max_{s \in \mathcal{S}}(DSP_{s_{op}} / II_s) \\
\label{eq:on_chip} & \begin{cases}
    \sum_{a \in \mathcal{A}} \sum_{l \in \mathcal{L}} loop_l\_cache\_array_a \cdot footprint\_array_a\_loop_l \leq Mem
\end{cases} \\
\end{split} \\
\begin{split}
\label{eq:max_part1} & \begin{cases}
    \forall a \in \mathcal{A}, \forall (d, d') \in \mathbb{N}^2 \text{ with } d \neq d', \forall l \in C_{a_d}, \forall l' \in C_{a_{d'}} , \\
    loop_l\_UF \cdot loop_{l'}\_UF \leq MAX\_PARTITIONING
\end{cases} \\
\label{eq:no_cache_under_pip} & \begin{cases}
    \forall p \in \mathcal{P}, \forall lp \in \mathcal{L}^p_{pip}, \forall lbp \in \mathcal{L}_{under\_pip_{lp}} \forall a \in \mathcal{A}, \\
    loop_{lbp}\_cache\_array_a == 0
\end{cases} \\
\end{split} \\
\begin{split}
\label{eq:under_pip_fully_unrolled} & \begin{cases}
    \forall p \in \mathcal{P}, \forall lp \in \mathcal{L}^p_{pip}, \forall lbp \in \mathcal{L}_{under\_pip_{lp}}, \\
    loop_{lp} \cdot loop_{lbp}\_UF == loop_{lp} \cdot TC_{lbp}
\end{cases} \\
\end{split}
\end{align}


==> sources/new_table.tex <==

\begin{table*}[htb]
\centering

% \begin{tabular}{|l rrrr|r|rrrr|rrrrr|rr|}
\begin{tabular}{@{}l @{\hspace{-1mm}}rrrrrrrrrr@{\hspace{-1.2mm}}rrrrrrrrrr@{}}
\toprule
 &  &  &  &  & FS & & \multicolumn{3}{l}{\textbf{NLP}} & & & \multicolumn{4}{l}{\textbf{AutoDSE}} & &  & \multicolumn{3}{l}{\textbf{Perf. Improvement}}   \\
% \cmidrule{6-17}
\cmidrule{6-6}
\cmidrule{8-11}
\cmidrule{13-17}
\cmidrule{19-21}
\textbf{Kernel} &  \textbf{NL} & \textbf{ND} & \textbf{S} & \textbf{Space S} & \textbf{GF/s} & &\textbf{GF/s} & \textbf{T} & \textbf{DE} & \textbf{DT} & & \textbf{GF/s} & \textbf{T} & \textbf{DE} & \textbf{DT} & \textbf{ER} & & \textbf{T} & \textbf{GF/s} & \textbf{R} \\

\midrule
2mm & 6 & 13 & M & 1.37E+10 & 13.19 &  & 117.48 & 70 & 18 & 0 &  & 0.41 & 1870 & 101 & 37 & 49 &  & 26.7x & 288.88x & 7,654.6x \\ 
        2mm & 6 & 13 & L & 1.15E+12 & 0.57 &  & 2.17 & 456 & 17 & 3 &  & 0.40 & 1835 & 291 & 38 & 240 &  & 4.0x & 5.41x & 21.8x \\ 
        3mm & 9 & 19 & M & 1.20E+15 & 13.86 &  & 138.73 & 242 & 18 & 0 &  & 0.39 & 698 & 82 & 15 & 57 &  & 2.9x & 354.12x & 1,026.0x \\ 
        3mm & 9 & 19 & L & 6.18E+17 & 0.18 &  & 1.01 & 486 & 19 & 3 &  & 0.59 & 968 & 112 & 18 & 81 &  & 2.0x & 1.71x & 3.4x \\ 
        atAx & 4 & 12 & M & 1.40E+05 & 1.96 &  & 1.96 & 194 & 10 & 1 &  & 1.98 & 1653 & 175 & 13 & 136 &  & 8.5x & 0.99x & 8.4x \\ 
        atAx & 4 & 12 & L & 1.60E+07 & 0.47 &  & 1.52 & 205 & 11 & 2 &  & 0.44 & 2325 & 166 & 30 & 106 &  & 11.3x & 3.46x & 39.2x \\ 
        bicg & 3 & 10 & M & 1.90E+04 & 0.99 &  & 0.99 & 248 & 12 & 1 &  & 0.98 & 729 & 65 & 2 & 28 &  & 2.9x & 1.01x & 3.0x \\ 
        bicg & 3 & 10 & L & 4.44E+05 & 1.68 &  & 1.68 & 218 & 12 & 1 &  & 0.50 & 3355 & 236 & 42 & 176 &  & 15.4x & 3.38x & 51.7x \\ 
        covariance & 7 & 34 & M & 1.80E+11 & 0.08 &  & 0.75 & 336 & 21 & 7 &  & 0.28 & 645 & 161 & 15 & 115 &  & 1.9x & 2.64x & 5.1x \\ 
        covariance & 7 & 34 & L & 1.92E+13 & 0.39 &  & 0.73 & 466 & 21 & 9 &  & 0.62 & 2849 & 209 & 68 & 118 &  & 6.1x & 1.16x & 7.2x \\ 
        doitgen & 5 & 30 & M & 8.64E+06 & 19.75 &  & 19.75 & 193 & 13 & 0 &  & 18.95 & 819 & 296 & 14 & 248 &  & 4.2x & 1.04x & 4.4x \\ 
        doitgen & 5 & 30 & L & 3.63E+07 & 0.08 &  & 102.62 & 241 & 20 & 1 &  & 110.66 & 1299 & 222 & 24 & 169 &  & 5.4x & 0.93x & 5.0x \\ 
        durbin & 4 & 55 & M & 1.08E+02 & 0.01 &  & 0.20 & 193 & 7 & 4 &  & 0.12 & 134 & 25 & 0 & 23 &  & 0.7x & 1.65x & 1.2x \\ 
        durbin & 4 & 55 & L & 9.00E+00 & 0.12 &  & 0.12 & 212 & 3 & 1 &  & 0.12 & 31 & 7 & 0 & 5 &  & 0.1x & 1.00x & 0.2x \\ 
        % fdtd-2d & 8 & 28 & M & 3.30E+08 & 166.33 &  & 166.33 & 342 & 14 & 2 &  & 162.53 & 1135 & 81 & 12 & 37 &  & 3.3x & 1.02x & 3.4x \\ 
        % fdtd-2d & 8 & 28 & L & 6.47E+11 & 0.88 &  & 0.92 & 630 & 19 & 17 &  & 0.92 & 1103 & 62 & 20 & 24 &  & 1.8x & 1.00x & 1.8x \\ 
        floyd-warshall & 3 & 21 & M & 8.65E+04 & 0.17 &  & 0.61 & 246 & 17 & 3 &  & 0.10 & 1605 & 60 & 22 & 29 &  & 6.5x & 6.15x & 39.8x \\ 
        floyd-warshall & 3 & 21 & L & 3.29E+06 & 0.17 &  & 1.31 & 381 & 20 & 6 &  & 0.10 & 2728 & 150 & 71 & 77 &  & 7.2x & 13.09x & 93.8x \\ 
        gemm & 4 & 6 & M & 2.30E+06 & 105.18 &  & 105.18 & 185 & 21 & 1 &  & 68.91 & 1345 & 86 & 27 & 34 &  & 7.3x & 1.53x & 11.1x \\ 
        gemm & 4 & 6 & L & 1.47E+07 & 32.98 &  & 32.98 & 450 & 18 & 7 &  & 2.77 & 2810 & 188 & 47 & 133 &  & 6.2x & 11.89x & 74.4x \\ 
        gemver & 7 & 13 & M & 7.72E+11 & 0.78 &  & 9.45 & 218 & 21 & 4 &  & 2.99 & 847 & 65 & 5 & 28 &  & 3.9x & 3.16x & 12.3x \\ 
        gemver & 7 & 13 & L & 1.28E+13 & 9.94 &  & 9.94 & 290 & 21 & 7 &  & 0.18 & 1756 & 221 & 206 & 10 &  & 6.1x & 54.69x & 334.4x \\ 
        gesummv & 2 & 17 & M & 6.12E+02 & 1.97 &  & 1.97 & 220 & 14 & 3 &  & 1.97 & 836 & 80 & 8 & 47 &  & 3.8x & 1.00x & 3.8x \\ 
        gesummv & 2 & 17 & L & 6.33E+03 & 1.82 &  & 2.64 & 236 & 18 & 1 &  & 0.56 & 692 & 94 & 29 & 60 &  & 2.9x & 4.73x & 13.8x \\ 
        gramschmidt & 6 & 34 & M & 1.75E+07 & 1.58 &  & 1.58 & 364 & 7 & 3 &  & 0.44 & 934 & 109 & 92 & 8 &  & 2.6x & 3.56x & 9.2x \\ 
        gramschmidt & 6 & 34 & L & 1.22E+08 & 2.34 &  & 2.34 & 420 & 6 & 4 &  & 0.95 & 819 & 265 & 11 & 239 &  & 1.9x & 2.47x & 4.8x \\ 
        heat-3d & 7 & 42 & M & 3.04E+07 & 0.23 &  & 3.75 & 402 & 17 & 7 &  & 3.75 & 928 & 75 & 33 & 35 &  & 2.3x & 1.00x & 2.3x \\ 
        heat-3d & 7 & 42 & L & 4.37E+07 & 0.13 &  & 0.62 & 520 & 13 & 6 &  & 0.63 & 740 & 109 & 70 & 35 &  & 1.4x & 0.99x & 1.4x \\ 
        jacobi-1d & 3 & 14 & M & 1.48E+03 & 11.43 &  & 11.43 & 55 & 4 & 0 &  & 11.53 & 948 & 126 & 3 & 74 &  & 17.2x & 0.99x & 17.1x \\ 
        jacobi-1d & 3 & 14 & L & 4.00E+04 & 5.95 &  & 5.95 & 386 & 9 & 6 &  & 2.65 & 1283 & 173 & 21 & 123 &  & 3.3x & 2.25x & 7.5x \\ 
        jacobi-2d & 5 & 22 & M & 8.07E+06 & 0.20 &  & 3.32 & 379 & 12 & 5 &  & 3.32 & 674 & 158 & 26 & 98 &  & 1.8x & 1.00x & 1.8x \\ 
        jacobi-2d & 5 & 22 & L & 1.14E+07 & 0.26 &  & 1.25 & 427 & 9 & 6 &  & 1.25 & 1106 & 231 & 39 & 171 &  & 2.6x & 1.00x & 2.6x \\ 
        lu & 5 & 16 & M & 2.28E+03 & 0.03 &  & 0.03 & 614 & 19 & 11 &  & 0.04 & 849 & 193 & 1 & 159 &  & 1.4x & 0.98x & 1.0x \\ 
        lu & 5 & 16 & L & 3.99E+03 & 0.03 &  & 0.04 & 335 & 9 & 2 &  & 0.03 & 812 & 258 & 5 & 219 &  & 2.4x & 1.03x & 3.2x \\ 
        mvt & 4 & 6 & M & 1.38E+07 & 7.77 &  & 7.77 & 212 & 17 & 1 &  & 7.77 & 893 & 166 & 6 & 106 &  & 4.2x & 1.00x & 4.2x \\ 
        mvt & 4 & 6 & L & 7.41E+07 & 12.90 &  & 12.90 & 181 & 20 & 3 &  & 1.10 & 1240 & 249 & 20 & 189 &  & 6.9x & 11.78x & 80.3x \\ 
        seidel-2d & 3 & 27 & M & 4.26E+03 & 0.05 &  & 0.05 & 365 & 5 & 1 &  & 0.05 & 796 & 103 & 27 & 68 &  & 2.2x & 1.01x & 2.2x \\ 
        seidel-2d & 3 & 27 & L & 1.77E+05 & 0.05 &  & 0.05 & 540 & 13 & 7 &  & 0.05 & 880 & 91 & 33 & 48 &  & 1.6x & 1.00x & 1.6x \\ 
        symm & 3 & 33 & M & 2.31E+04 & 0.04 &  & 0.20 & 63 & 5 & 0 &  & 0.20 & 691 & 142 & 35 & 89 &  & 11.0x & 1.00x & 11.0x \\ 
        symm & 3 & 33 & L & 6.64E+04 & 0.21 &  & 0.31 & 540 & 8 & 5 &  & 0.21 & 612 & 731 & 0 & 692 &  & 1.1x & 1.52x & 1.7x \\ 
        syr2k & 4 & 6 & M & 2.32E+04 & 0.07 &  & 1.74 & 224 & 16 & 2 &  & 1.20 & 685 & 230 & 17 & 203 &  & 3.1x & 1.45x & 4.4x \\ 
        syr2k & 4 & 6 & L & 6.67E+04 & 1.30 &  & 1.42 & 420 & 15 & 7 &  & 1.30 & 768 & 293 & 21 & 262 &  & 1.8x & 1.09x & 2.0x \\ 
        syrk & 4 & 6 & M & 2.32E+04 & 0.49 &  & 1.32 & 224 & 16 & 2 &  & 0.61 & 631 & 280 & 4 & 264 &  & 2.8x & 2.15x & 6.1x \\ 
        syrk & 4 & 6 & L & 6.67E+04 & 0.94 &  & 2.07 & 466 & 17 & 7 &  & 0.65 & 643 & 410 & 0 & 398 &  & 1.4x & 3.16x & 4.4x \\ 
        trisolv & 2 & 13 & M & 3.60E+02 & 0.03 &  & 0.03 & 69 & 12 & 0 &  & 0.04 & 694 & 69 & 33 & 23 &  & 10.1x & 0.98x & 7.5x \\ 
        trisolv & 2 & 13 & L & 6.30E+02 & 0.04 &  & 0.04 & 75 & 18 & 0 &  & 0.04 & 651 & 127 & 2 & 98 &  & 8.7x & 0.99x & 8.7x \\ 
        trmm & 3 & 8 & M & 2.31E+04 & 0.01 &  & 0.05 & 20 & 16 & 0 &  & 0.04 & 630 & 401 & 4 & 367 &  & 31.5x & 1.29x & 39.4x \\ 
        trmm & 3 & 8 & L & 6.64E+04 & 0.02 &  & 0.06 & 425 & 17 & 2 &  & 0.03 & 760 & 167 & 159 & 4 &  & 1.8x & 1.79x & 3.6x \\ 
\bottomrule

\end{tabular}

\caption{Comparison with AutoDSE}
\label{tab:eval}

\end{table*}

% % % \vspace{-1cm}
% why there is this probleme to the table ? TODO


==> sources/table_ori.tex <==

% \begin{table*}[htb]
\begin{table*}[]
\centering

% \begin{tabular}{|l rrrr|r|rrrr|rrrrr|rr|}
\begin{tabular}{@{}l @{\hspace{-1mm}}rrrrrrrrrr@{\hspace{-1.2mm}}rrrrrrrrr@{}}
\toprule
 &  &  &  &  & FS & & \multicolumn{3}{l}{\textbf{\framework}} & & & \multicolumn{4}{l}{\textbf{AutoDSE}} & &  & \multicolumn{2}{l}{\textbf{Perf. Improvement}}   \\
% \cmidrule{6-17}
\cmidrule{6-6}
\cmidrule{8-11}
\cmidrule{13-17}
\cmidrule{19-20}
\textbf{Kernel} &  \textbf{NL} & \textbf{ND} & \textbf{S} & \textbf{Space S} & \textbf{GF/s} & &\textbf{GF/s} & \textbf{T} & \textbf{DE} & \textbf{DT} & & \textbf{GF/s} & \textbf{T} & \textbf{DE} & \textbf{DT} & \textbf{ER} & & \textbf{T} & \textbf{GF/s} \\

\midrule

% \input{sources/table2}
        2mm & 6 & 13 & M & 1.37E+10 & 13.19 &  & 117.48 & 70 & 18 & 0 &  & 0.41 & 1,870 & 101 & 37 & 49 &  & 26.71x & 288.88x \\ 
        2mm & 6 & 13 & L & 1.15E+12 & 0.57 &  & 2.17 & 456 & 17 & 3 &  & 0.40 & 1,835 & 291 & 38 & 240 &  & 4.02x & 5.41x \\ 
        3mm & 9 & 19 & M & 1.20E+15 & 13.86 &  & 138.73 & 242 & 18 & 0 &  & 0.39 & 698 & 82 & 15 & 57 &  & 2.88x & 354.12x \\ 
        3mm & 9 & 19 & L & 6.18E+17 & 0.18 &  & 1.01 & 486 & 19 & 3 &  & 0.59 & 968 & 112 & 18 & 81 &  & 1.99x & 1.71x \\ 
        atAx & 4 & 12 & M & 1.40E+05 & 1.96 &  & 1.96 & 194 & 10 & 1 &  & 1.98 & 1,653 & 175 & 13 & 136 &  & 8.52x & 0.99x \\ 
        atAx & 4 & 12 & L & 1.60E+07 & 0.47 &  & 1.52 & 205 & 11 & 2 &  & 0.44 & 2,325 & 166 & 30 & 106 &  & 11.34x & 3.46x \\ 
        bicg & 3 & 10 & M & 1.90E+04 & 0.99 &  & 0.99 & 248 & 12 & 1 &  & 0.98 & 729 & 65 & 2 & 28 &  & 2.94x & 1.01x \\ 
        bicg & 3 & 10 & L & 4.44E+05 & 1.68 &  & 1.68 & 218 & 12 & 1 &  & 0.50 & 3,355 & 236 & 42 & 176 &  & 15.39x & 3.38x \\ 
    cnn & 6 & 2 & - & 6.43E+06 & 0.39 && 97.99 & 20.84 & 16 & 1 && 97.99 & 275 & 28 & 19 & 480 && 13.19x & 1.00x \\
        covariance & 7 & 34 & M & 1.80E+11 & 0.08 &  & 0.75 & 336 & 21 & 8 &  & 0.28 & 645 & 161 & 15 & 115 &  & 1.92x & 2.64x \\ 
        covariance & 7 & 34 & L & 1.92E+13 & 0.39 &  & 0.73 & 466 & 21 & 9 &  & 0.62 & 2,849 & 209 & 68 & 118 &  & 6.11x & 1.16x \\ 
        doitgen & 5 & 30 & M & 8.64E+06 & 19.75 &  & 19.75 & 193 & 13 & 0 &  & 18.95 & 819 & 296 & 14 & 248 &  & 4.24x & 1.04x \\ 
        doitgen & 5 & 30 & L & 3.63E+07 & 0.08 &  & 102.62 & 241 & 20 & 1 &  & 110.66 & 1,299 & 222 & 24 & 169 &  & 5.39x & 0.93x \\ 
        durbin & 4 & 55 & M & 1.08E+02 & 0.01 &  & 0.20 & 193 & 7 & 4 &  & 0.12 & 134 & 25 & 0 & 23 &  & 0.69x & 1.65x \\ 
        durbin & 4 & 55 & L & 9.00E+00 & 0.12 &  & 0.12 & 212 & 3 & 1 &  & 0.12 & 31 & 7 & 0 & 5 &  & 0.15x & 1.00x \\ 
        floyd-warshall & 3 & 21 & M & 8.65E+04 & 0.17 &  & 0.61 & 246 & 17 & 3 &  & 0.10 & 1,605 & 60 & 22 & 29 &  & 6.52x & 6.15x \\ 
        floyd-warshall & 3 & 21 & L & 3.29E+06 & 0.17 &  & 1.31 & 381 & 20 & 6 &  & 0.10 & 2,728 & 150 & 71 & 77 &  & 7.16x & 13.09x \\ 
        gemm & 4 & 6 & M & 2.30E+06 & 105.18 &  & 105.18 & 185 & 21 & 1 &  & 68.91 & 1,345 & 86 & 27 & 34 &  & 7.27x & 1.53x \\ 
        gemm & 4 & 6 & L & 1.47E+07 & 32.98 &  & 32.98 & 450 & 18 & 7 &  & 2.77 & 2,810 & 188 & 47 & 133 &  & 6.24x & 11.89x \\ 
        gemver & 7 & 13 & M & 7.72E+11 & 0.78 &  & 9.45 & 218 & 21 & 4 &  & 2.99 & 847 & 65 & 5 & 28 &  & 3.89x & 3.16x \\ 
        gemver & 7 & 13 & L & 1.28E+13 & 9.94 &  & 9.94 & 290 & 21 & 7 &  & 0.18 & 1,756 & 221 & 206 & 10 &  & 6.06x & 54.69x \\ 
        gesummv & 2 & 17 & M & 6.12E+02 & 1.97 &  & 1.97 & 220 & 14 & 3 &  & 1.97 & 836 & 80 & 8 & 47 &  & 3.80x & 1.00x \\ 
        gesummv & 2 & 17 & L & 6.33E+03 & 1.82 &  & 2.64 & 236 & 18 & 1 &  & 0.56 & 692 & 94 & 29 & 60 &  & 2.93x & 4.73x \\ 
        gramschmidt & 6 & 34 & M & 1.75E+07 & 1.58 &  & 1.58 & 364 & 7 & 3 &  & 0.44 & 934 & 109 & 92 & 8 &  & 2.57x & 3.56x \\ 
        gramschmidt & 6 & 34 & L & 1.22E+08 & 2.34 &  & 2.34 & 420 & 6 & 4 &  & 0.95 & 819 & 265 & 11 & 239 &  & 1.95x & 2.47x \\ 
        heat-3d & 7 & 42 & M & 3.04E+07 & 0.23 &  & 3.75 & 402 & 17 & 7 &  & 3.75 & 928 & 75 & 33 & 35 &  & 2.31x & 1.00x \\ 
        heat-3d & 7 & 42 & L & 4.37E+07 & 0.13 &  & 0.62 & 520 & 13 & 6 &  & 0.63 & 740 & 109 & 70 & 35 &  & 1.42x & 0.99x \\ 
        jacobi-1d & 3 & 14 & M & 1.48E+03 & 11.43 &  & 11.43 & 55 & 4 & 0 &  & 11.53 & 948 & 126 & 3 & 74 &  & 17.24x & 0.99x \\ 
        jacobi-1d & 3 & 14 & L & 4.00E+04 & 5.95 &  & 5.95 & 386 & 9 & 6 &  & 2.65 & 1,283 & 173 & 21 & 123 &  & 3.32x & 2.25x \\ 
        jacobi-2d & 5 & 22 & M & 8.07E+06 & 0.20 &  & 3.32 & 379 & 12 & 5 &  & 3.32 & 674 & 158 & 26 & 98 &  & 1.78x & 1.00x \\ 
        jacobi-2d & 5 & 22 & L & 1.14E+07 & 0.26 &  & 1.25 & 427 & 9 & 6 &  & 1.25 & 1,106 & 231 & 39 & 171 &  & 2.59x & 1.00x \\ 
        lu & 5 & 16 & M & 2.28E+03 & 0.03 &  & 0.03 & 614 & 19 & 11 &  & 0.04 & 849 & 193 & 1 & 159 &  & 1.38x & 0.98x \\ 
        lu & 5 & 16 & L & 3.99E+03 & 0.03 &  & 0.04 & 335 & 9 & 2 &  & 0.03 & 812 & 258 & 5 & 219 &  & 2.42x & 1.03x \\ 
        mvt & 4 & 6 & M & 1.38E+07 & 7.77 &  & 7.77 & 212 & 17 & 1 &  & 7.77 & 893 & 166 & 6 & 106 &  & 4.21x & 1.00x \\ 
        mvt & 4 & 6 & L & 7.41E+07 & 12.90 &  & 12.90 & 181 & 20 & 3 &  & 1.10 & 1,240 & 249 & 20 & 189 &  & 6.85x & 11.78x \\ 
        seidel-2d & 3 & 27 & M & 4.26E+03 & 0.05 &  & 0.05 & 365 & 5 & 1 &  & 0.05 & 796 & 103 & 27 & 68 &  & 2.18x & 1.01x \\ 
        seidel-2d & 3 & 27 & L & 1.77E+05 & 0.05 &  & 0.05 & 540 & 13 & 7 &  & 0.05 & 880 & 91 & 33 & 48 &  & 1.63x & 1.00x \\ 
        symm & 3 & 33 & M & 2.31E+04 & 0.04 &  & 0.20 & 63 & 5 & 0 &  & 0.20 & 691 & 142 & 35 & 89 &  & 10.97x & 1.00x \\ 
        symm & 3 & 33 & L & 6.64E+04 & 0.21 &  & 0.31 & 540 & 8 & 5 &  & 0.21 & 612 & 731 & 0 & 692 &  & 1.13x & 1.52x \\ 
        syr2k & 4 & 6 & M & 2.32E+04 & 0.07 &  & 1.74 & 224 & 16 & 2 &  & 1.20 & 685 & 230 & 17 & 203 &  & 3.06x & 1.45x \\ 
        syr2k & 4 & 6 & L & 6.67E+04 & 1.30 &  & 1.42 & 420 & 15 & 7 &  & 1.30 & 768 & 293 & 21 & 262 &  & 1.83x & 1.09x \\ 
        syrk & 4 & 6 & M & 2.32E+04 & 0.49 &  & 1.32 & 224 & 16 & 2 &  & 0.61 & 631 & 280 & 4 & 264 &  & 2.82x & 2.15x \\ 
        syrk & 4 & 6 & L & 6.67E+04 & 0.94 &  & 2.07 & 466 & 17 & 7 &  & 0.65 & 643 & 410 & 0 & 398 &  & 1.38x & 3.16x \\ 
        trisolv & 2 & 13 & M & 3.60E+02 & 0.03 &  & 0.03 & 69 & 12 & 0 &  & 0.04 & 694 & 69 & 33 & 23 &  & 10.06x & 0.98x \\ 
        trisolv & 2 & 13 & L & 6.30E+02 & 0.04 &  & 0.04 & 75 & 18 & 0 &  & 0.04 & 651 & 127 & 2 & 98 &  & 8.68x & 0.99x \\ 
        trmm & 3 & 8 & M & 2.31E+04 & 0.01 &  & 0.05 & 20 & 16 & 0 &  & 0.04 & 630 & 401 & 4 & 367 &  & 31.50x & 1.29x \\ 
        trmm & 3 & 8 & L & 6.64E+04 & 0.02 &  & 0.06 & 425 & 17 & 2 &  & 0.03 & 760 & 167 & 159 & 4 &  & 1.79x & 1.79x \\ 
\midrule
% Average &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
% Geo. Mean &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
Average &  &  &  &  & 5.50 &  & 15.44 & 289 &  &  &  & 7.61 & 1,108 &  &  &  &  & 5.93x & 17.57x \\
Geo. Mean &  &  &  &  & 0.54 &  & 1.65 & 232 &  &  &  & 0.69 & 889 &  &  &  &  & 3.82x & 2.40x \\
\bottomrule

\end{tabular}

\caption{Comparison with AutoDSE}

\label{tab:eval}
% \vspace{-0.6cm}
\end{table*}





==> sources/tablev1.tex <==

\begin{table*}[htb]
\centering

% \begin{tabular}{|l rrrr|r|rrrr|rrrrr|rr|}
\begin{tabular}{@{}l rrrrrrrrrrrrrrrrrrr@{}}
\toprule
 &  &  &  &  & FS & & \multicolumn{3}{l}{\textbf{NLP}} & & & \multicolumn{4}{l}{\textbf{AutoDSE}} & &  & \multicolumn{1}{l}{\textbf{SpeedUp}} &  \\
% \cmidrule{6-17}
\cmidrule{6-6}
\cmidrule{8-11}
\cmidrule{13-17}
\cmidrule{19-20}
\textbf{Kernel} & \textbf{NL} & \textbf{ND} & \textbf{S} & \textbf{Space S} & \textbf{GF/s} & &\textbf{GF/s} & \textbf{T} & \textbf{DE} & \textbf{DT} & & \textbf{GF/s} & \textbf{T} & \textbf{DE} & \textbf{DT} & \textbf{ER} & & \textbf{T} & \textbf{GF/s} \\

\midrule



% \input{sources/table2}

% \bottomrule
2mm & 6 & 13 & L & 1.15E+12 & 0.57 &  & 2.17 & 456 & 17 & 3 &  & 0.40 & 1,835 & 291 & 38 & 240 &  & 4.02 & 5.41 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        2mm & 6 & 13 & M & 1.37E+10 & 13.19 &  & 117.48 & 70 & 18 & 0 &  & 0.41 & 1,870 & 101 & 37 & 49 &  & 26.71 & 288.88 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        3mm & 9 & 19 & L & 6.18E+17 & 0.18 &  & 1.01 & 486 & 19 & 3 &  & 0.59 & 968 & 112 & 18 & 81 &  & 1.99 & 1.71 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        3mm & 9 & 19 & M & 1.20E+15 & 13.86 &  & 138.73 & 242 & 18 & 0 &  & 0.39 & 698 & 82 & 15 & 57 &  & 2.88 & 354.12 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        atax & 4 & 12 & L & 1.60E+07 & 0.47 &  & 1.52 & 205 & 11 & 2 &  & 0.44 & 2,325 & 166 & 30 & 106 &  & 11.34 & 3.46 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        atax & 4 & 12 & M & 1.40E+05 & 1.96 &  & 1.96 & 194 & 10 & 1 &  & 1.98 & 1,653 & 175 & 13 & 136 &  & 8.52 & 0.99 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        bicg & 3 & 10 & L & 4.44E+05 & 1.68 &  & 1.68 & 218 & 12 & 1 &  & 0.50 & 3,355 & 236 & 42 & 176 &  & 15.39 & 3.38 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        bicg & 3 & 10 & M & 1.90E+04 & 0.99 &  & 0.99 & 248 & 12 & 1 &  & 0.98 & 729 & 65 & 2 & 28 &  & 2.94 & 1.01 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        covariance & 7 & 34 & L & 1.92E+13 & 0.39 &  & 0.73 & 466 & 21 & 9 &  & 0.62 & 2,849 & 209 & 68 & 118 &  & 6.11 & 1.16 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        covariance & 7 & 34 & M & 1.80E+11 & 0.08 &  & 0.75 & 336 & 21 & 8 &  & 0.28 & 645 & 161 & 15 & 115 &  & 1.92 & 2.64 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        doitgen & 5 & 30 & L & 3.63E+07 & 0.08 &  & 102.62 & 241 & 20 & 1 &  & 110.66 & 1,299 & 222 & 24 & 169 &  & 5.39 & 0.93 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        doitgen & 5 & 30 & M & 8.64E+06 & 19.75 &  & 19.75 & 193 & 13 & 0 &  & 18.95 & 819 & 296 & 14 & 248 &  & 4.24 & 1.04 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        durbin & 4 & 55 & L & 9.00E+00 & 0.12 &  & 0.12 & 212 & 3 & 1 &  & 0.12 & 31 & 7 & 0 & 5 &  & 0.15 & 1.00 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        durbin & 4 & 55 & M & 1.08E+02 & 0.01 &  & 0.20 & 193 & 7 & 4 &  & 0.12 & 134 & 25 & 0 & 23 &  & 0.69 & 1.65 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        fdtd-2d & 8 & 28 & L & 6.47E+11 & 0.88 &  & 0.92 & 630 & 19 & 17 &  & 0.92 & 1,103 & 62 & 20 & 24 &  & 1.75 & 1.00 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        fdtd-2d & 8 & 28 & M & 3.30E+08 & 166.33 &  & 166.33 & 342 & 14 & 2 &  & 162.53 & 1,135 & 81 & 12 & 37 &  & 3.32 & 1.02 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        floyd-warshall & 3 & 21 & L & 3.29E+06 & 0.17 &  & 1.31 & 381 & 20 & 6 &  & 0.10 & 2,728 & 150 & 71 & 77 &  & 7.16 & 13.09 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        floyd-warshall & 3 & 21 & M & 8.65E+04 & 0.17 &  & 0.61 & 246 & 17 & 3 &  & 0.10 & 1,605 & 60 & 22 & 29 &  & 6.52 & 6.15 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        gemm & 4 & 6 & L & 1.47E+07 & 32.98 &  & 32.98 & 450 & 18 & 7 &  & 2.77 & 2,810 & 188 & 47 & 133 &  & 6.24 & 11.89 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        gemm & 4 & 6 & M & 2.30E+06 & 105.18 &  & 105.18 & 185 & 21 & 1 &  & 68.91 & 1,345 & 86 & 27 & 34 &  & 7.27 & 1.53 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        gemver & 7 & 13 & L & 1.28E+13 & 9.94 &  & 9.94 & 290 & 21 & 7 &  & 0.18 & 1,756 & 221 & 206 & 10 &  & 6.06 & 54.69 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        gemver & 7 & 13 & M & 7.72E+11 & 0.78 &  & 9.45 & 218 & 21 & 4 &  & 2.99 & 847 & 65 & 5 & 28 &  & 3.89 & 3.16 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        gesummv & 2 & 17 & L & 6.33E+03 & 1.82 &  & 2.64 & 236 & 18 & 1 &  & 0.56 & 692 & 94 & 29 & 60 &  & 2.93 & 4.73 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        gesummv & 2 & 17 & M & 6.12E+02 & 1.97 &  & 1.97 & 220 & 14 & 3 &  & 1.97 & 836 & 80 & 8 & 47 &  & 3.80 & 1.00 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        gramschmidt & 6 & 34 & L & 1.22E+08 & 2.34 &  & 2.34 & 420 & 6 & 4 &  & 0.95 & 819 & 265 & 11 & 239 &  & 1.95 & 2.47 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        gramschmidt & 6 & 34 & M & 1.75E+07 & 1.58 &  & 1.58 & 364 & 7 & 3 &  & 0.44 & 934 & 109 & 92 & 8 &  & 2.57 & 3.56 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        heat-3d & 7 & 42 & L & 4.37E+07 & 0.13 &  & 0.62 & 520 & 13 & 6 &  & 0.63 & 740 & 109 & 70 & 35 &  & 1.42 & 0.99 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        heat-3d & 7 & 42 & M & 3.04E+07 & 0.23 &  & 3.75 & 402 & 17 & 7 &  & 3.75 & 928 & 75 & 33 & 35 &  & 2.31 & 1.00 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        jacobi-1d & 3 & 14 & L & 4.00E+04 & 5.95 &  & 5.95 & 386 & 9 & 6 &  & 2.65 & 1,283 & 173 & 21 & 123 &  & 3.32 & 2.25 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        jacobi-1d & 3 & 14 & M & 1.48E+03 & 11.43 &  & 11.43 & 55 & 4 & 0 &  & 11.53 & 948 & 126 & 3 & 74 &  & 17.24 & 0.99 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        jacobi-2d & 5 & 22 & L & 1.14E+07 & 0.26 &  & 1.25 & 427 & 9 & 6 &  & 1.25 & 1,106 & 231 & 39 & 171 &  & 2.59 & 1.00 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        jacobi-2d & 5 & 22 & M & 8.07E+06 & 0.20 &  & 3.32 & 379 & 12 & 5 &  & 3.32 & 674 & 158 & 26 & 98 &  & 1.78 & 1.00 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        lu & 5 & 16 & L & 3.99E+03 & 0.03 &  & 0.04 & 335 & 9 & 2 &  & 0.03 & 812 & 258 & 5 & 219 &  & 2.42 & 1.03 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        lu & 5 & 16 & M & 2.28E+03 & 0.03 &  & 0.03 & 614 & 19 & 11 &  & 0.04 & 849 & 193 & 1 & 159 &  & 1.38 & 0.98 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        mvt & 4 & 6 & L & 7.41E+07 & 12.90 &  & 12.90 & 181 & 20 & 3 &  & 1.10 & 1,240 & 249 & 20 & 189 &  & 6.85 & 11.78 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        mvt & 4 & 6 & M & 1.38E+07 & 7.77 &  & 7.77 & 212 & 17 & 1 &  & 7.77 & 893 & 166 & 6 & 106 &  & 4.21 & 1.00 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        seidel-2d & 3 & 27 & L & 1.77E+05 & 0.05 &  & 0.05 & 540 & 13 & 7 &  & 0.05 & 880 & 91 & 33 & 48 &  & 1.63 & 1.00 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        seidel-2d & 3 & 27 & M & 4.26E+03 & 0.05 &  & 0.05 & 365 & 5 & 1 &  & 0.05 & 796 & 103 & 27 & 68 &  & 2.18 & 1.01 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        symm & 3 & 33 & L & 6.64E+04 & 0.21 &  & 0.31 & 540 & 8 & 5 &  & 0.21 & 612 & 731 & 0 & 692 &  & 1.13 & 1.52 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        symm & 3 & 33 & M & 2.31E+04 & 0.04 &  & 0.20 & 63 & 5 & 0 &  & 0.20 & 691 & 142 & 35 & 89 &  & 10.97 & 1.00 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        syr2k & 4 & 6 & L & 6.67E+04 & 1.30 &  & 1.42 & 420 & 15 & 7 &  & 1.30 & 768 & 293 & 21 & 262 &  & 1.83 & 1.09 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        syr2k & 4 & 6 & M & 2.32E+04 & 0.07 &  & 1.74 & 224 & 16 & 2 &  & 1.20 & 685 & 230 & 17 & 203 &  & 3.06 & 1.45 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        syrk & 4 & 6 & L & 6.67E+04 & 0.94 &  & 2.07 & 466 & 17 & 7 &  & 0.65 & 643 & 410 & 0 & 398 &  & 1.38 & 3.16 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        syrk & 4 & 6 & M & 2.32E+04 & 0.49 &  & 1.32 & 224 & 16 & 2 &  & 0.61 & 631 & 280 & 4 & 264 &  & 2.82 & 2.15 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        trisolv & 2 & 13 & L & 6.30E+02 & 0.04 &  & 0.04 & 75 & 18 & 0 &  & 0.04 & 651 & 127 & 2 & 98 &  & 8.68 & 0.99 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        trisolv & 2 & 13 & M & 3.60E+02 & 0.03 &  & 0.03 & 69 & 12 & 0 &  & 0.04 & 694 & 69 & 33 & 23 &  & 10.06 & 0.98 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        trmm & 3 & 8 & L & 6.64E+04 & 0.02 &  & 0.06 & 425 & 17 & 2 &  & 0.03 & 760 & 167 & 159 & 4 &  & 1.79 & 1.79 \\ \cmidrule{6-6} \cmidrule{8-11} \cmidrule{13-17} \cmidrule{19-20} 
        trmm & 3 & 8 & M & 2.31E+04 & 0.01 &  & 0.05 & 20 & 16 & 0 &  & 0.04 & 630 & 401 & 4 & 367 &  & 31.50 & 1.29 \\ 

\bottomrule

\end{tabular}

\caption{Comparison with AutoDSE}
\label{tab:eval}

\end{table*}

% % \vspace{-1cm}
% why there is this probleme to the table ? TODO


==> sources/tablev2_.tex <==
% \newpage
% \newgeometry{left=2cm,top=0.8cm}
% \vspace{-2cm}
\begin{table}[]
% \begin{table*}[]
\footnotesize
\begin{adjustwidth}{-1in}{-1in}
% \begin{adjustheight}
    
\centering
% \begin{spacing}{0.95}
% \begin{tabular}{|l rrrr|r|rrrr|rrrrr|rr|}
\begin{tabular}{@{}l @{\hspace{-0.25cm}}
% rrrr
r
% @{\hspace{-0.05mm}}
r
@{\hspace{-1.6mm}}
rrrrr
@{\hspace{-1.2mm}}
rrrrrrr
@{\hspace{-1.2mm}}
r
r@{}}
\toprule
 &  &   FS & & \multicolumn{3}{l}{\textbf{\framework}} & & & \multicolumn{4}{l}{\textbf{AutoDSE}} & &  & \multicolumn{2}{l}{\textbf{Perf. Improv.}}   \\
% \cmidrule{6-17}
\cmidrule{3-3}
\cmidrule{5-8}
\cmidrule{10-14}
\cmidrule{16-17}
\textbf{Kernel} &  \textbf{NL-ND-S-Space S} & \textbf{GF/s} & &\textbf{GF/s} & \textbf{T} & \textbf{DE} & \textbf{DT} & & \textbf{GF/s} & \textbf{T} & \textbf{DE} & \textbf{DT} & \textbf{ER} & & \textbf{T} & \textbf{GF/s} \\

\midrule

%Data Mining
        cov. & 7-34-M-1.80E+11 & 0.08 &  & 0.75 & 336 & 21 & 8 &  & 0.28 & 645 & 161 & 15 & 115 &  & 1.92x & 2.64x \\ 
        cov. & 7-34-L-1.92E+13 & 0.39 &  & 0.73 & 466 & 21 & 9 &  & 0.62 & 2,849 & 209 & 68 & 118 &  & 6.11x & 1.16x \\ 

\midrule

%LA
        2mm & 6-13-M-1.37E+10 & 13.19 &  & 117.48 & 70 & 18 & 0 &  & 0.41 & 1,870 & 101 & 37 & 49 &  & 26.71x & 288x \\ 
        2mm & 6-13-L-1.15E+12 & 0.57 &  & 2.17 & 456 & 17 & 3 &  & 0.40 & 1,835 & 291 & 38 & 240 &  & 4.02x & 5.41x \\ 
        3mm & 9-19-M-1.20E+15 & 13.86 &  & 138.73 & 242 & 18 & 0 &  & 0.39 & 698 & 82 & 15 & 57 &  & 2.88x & 354x \\ 
        3mm & 9-19-L-6.18E+17 & 0.18 &  & 1.01 & 486 & 19 & 3 &  & 0.59 & 968 & 112 & 18 & 81 &  & 1.99x & 1.71x \\ 
        atAx & 4-12-M-1.40E+05 & 1.96 &  & 1.96 & 194 & 10 & 1 &  & 1.98 & 1,653 & 175 & 13 & 136 &  & 8.52x & 0.99x \\ 
        atAx & 4-12-L-1.60E+07 & 0.47 &  & 1.52 & 205 & 11 & 2 &  & 0.44 & 2,325 & 166 & 30 & 106 &  & 11.34x & 3.46x \\ 
        bicg & 3-10-M-1.90E+04 & 0.99 &  & 0.99 & 248 & 12 & 1 &  & 0.98 & 729 & 65 & 2 & 28 &  & 2.94x & 1.01x \\ 
        bicg & 3-10-L-4.44E+05 & 1.68 &  & 1.68 & 218 & 12 & 1 &  & 0.50 & 3,355 & 236 & 42 & 176 &  & 15.39x & 3.38x \\ 
    cnn & 6-2---6.43E+06 & 0.39 && 97.99 & 213 & 16 & 1 && 97.99 & 1,292 & 28 & 19 & 480 && 6.06x & 1.00x \\

        doitgen & 5-30-M-8.64E+06 & 19.75 &  & 19.75 & 193 & 13 & 0 &  & 18.95 & 819 & 296 & 14 & 248 &  & 4.24x & 1.04x \\ 
        doitgen & 5-30-L-3.63E+07 & 0.08 &  & 102.62 & 241 & 20 & 1 &  & 110.66 & 1,299 & 222 & 24 & 169 &  & 5.39x & 0.93x \\ 
        durbin & 4-55-M-1.08E+02 & 0.01 &  & 0.20 & 193 & 7 & 4 &  & 0.12 & 134 & 25 & 0 & 23 &  & 0.69x & 1.65x \\ 
        durbin & 4-55-L-9.00E+00 & 0.12 &  & 0.12 & 212 & 3 & 1 &  & 0.12 & 31 & 7 & 0 & 5 &  & 0.15x & 1.00x \\ 


        gemm & 4-6-M-2.30E+06 & 105.18 &  & 105.18 & 185 & 21 & 1 &  & 68.91 & 1,345 & 86 & 27 & 34 &  & 7.27x & 1.53x \\ 
        gemm & 4-6-L-1.47E+07 & 32.98 &  & 32.98 & 450 & 18 & 7 &  & 2.77 & 2,810 & 188 & 47 & 133 &  & 6.24x & 11.8x \\ 
        gemver & 7-13-M-7.72E+11 & 0.78 &  & 9.45 & 218 & 21 & 4 &  & 2.99 & 847 & 65 & 5 & 28 &  & 3.89x & 3.16x \\ 
        gemver & 7-13-L-1.28E+13 & 9.94 &  & 9.94 & 290 & 21 & 7 &  & 0.18 & 1,756 & 221 & 206 & 10 &  & 6.06x & 54.6x \\ 
        gesum. & 2-17-M-6.12E+02 & 1.97 &  & 1.97 & 220 & 14 & 3 &  & 1.97 & 836 & 80 & 8 & 47 &  & 3.80x & 1.00x \\ 
        gesum. & 2-17-L-6.33E+03 & 1.82 &  & 2.64 & 236 & 18 & 1 &  & 0.56 & 692 & 94 & 29 & 60 &  & 2.93x & 4.73x \\ 
        gram. & 6-34-M-1.75E+07 & 1.58 &  & 1.58 & 364 & 7 & 3 &  & 0.44 & 934 & 109 & 92 & 8 &  & 2.57x & 3.56x \\ 
        gram. & 6-34-L-1.22E+08 & 2.34 &  & 2.34 & 420 & 6 & 4 &  & 0.95 & 819 & 265 & 11 & 239 &  & 1.95x & 2.47x \\ 

        lu & 5-16-M-2.28E+03 & 0.03 &  & 0.03 & 614 & 19 & 11 &  & 0.04 & 849 & 193 & 1 & 159 &  & 1.38x & 0.98x \\ 
        lu & 5-16-L-3.99E+03 & 0.03 &  & 0.04 & 335 & 9 & 2 &  & 0.03 & 812 & 258 & 5 & 219 &  & 2.42x & 1.03x \\ 
        mvt & 4-6-M-1.38E+07 & 7.77 &  & 7.77 & 212 & 17 & 1 &  & 7.77 & 893 & 166 & 6 & 106 &  & 4.21x & 1.00x \\ 
        mvt & 4-6-L-7.41E+07 & 12.90 &  & 12.90 & 181 & 20 & 3 &  & 1.10 & 1,240 & 249 & 20 & 189 &  & 6.85x & 11.7x \\ 

        symm & 3-33-M-2.31E+04 & 0.04 &  & 0.20 & 63 & 5 & 0 &  & 0.20 & 691 & 142 & 35 & 89 &  & 10.97x & 1.00x \\ 
        symm & 3-33-L-6.64E+04 & 0.21 &  & 0.31 & 540 & 8 & 5 &  & 0.21 & 612 & 731 & 0 & 692 &  & 1.13x & 1.52x \\ 
        syr2k & 4-6-M-2.32E+04 & 0.07 &  & 1.74 & 224 & 16 & 2 &  & 1.20 & 685 & 230 & 17 & 203 &  & 3.06x & 1.45x \\ 
        syr2k & 4-6-L-6.67E+04 & 1.30 &  & 1.42 & 420 & 15 & 7 &  & 1.30 & 768 & 293 & 21 & 262 &  & 1.83x & 1.09x \\ 
        syrk & 4-6-M-2.32E+04 & 0.49 &  & 1.32 & 224 & 16 & 2 &  & 0.61 & 631 & 280 & 4 & 264 &  & 2.82x & 2.15x \\ 
        syrk & 4-6-L-6.67E+04 & 0.94 &  & 2.07 & 466 & 17 & 7 &  & 0.65 & 643 & 410 & 0 & 398 &  & 1.38x & 3.16x \\ 
        trisolv & 2-13-M-3.60E+02 & 0.03 &  & 0.03 & 69 & 12 & 0 &  & 0.04 & 694 & 69 & 33 & 23 &  & 10.06x & 0.98x \\ 
        trisolv & 2-13-L-6.30E+02 & 0.04 &  & 0.04 & 75 & 18 & 0 &  & 0.04 & 651 & 127 & 2 & 98 &  & 8.68x & 0.99x \\ 
        trmm & 3-8-M-2.31E+04 & 0.01 &  & 0.05 & 20 & 16 & 0 &  & 0.04 & 630 & 401 & 4 & 367 &  & 31.50x & 1.29x \\ 
        trmm & 3-8-L-6.64E+04 & 0.02 &  & 0.06 & 425 & 17 & 2 &  & 0.03 & 760 & 167 & 159 & 4 &  & 1.79x & 1.79x \\ 

% Medley
\midrule
        floyd-w & 3-21-M-8.65E+04 & 0.17 &  & 0.61 & 246 & 17 & 3 &  & 0.10 & 1,605 & 60 & 22 & 29 &  & 6.52x & 6.15x \\ 
        floyd-w & 3-21-L-3.29E+06 & 0.17 &  & 1.31 & 381 & 20 & 6 &  & 0.10 & 2,728 & 150 & 71 & 77 &  & 7.16x & 13.1x \\ 
% Stencil
\midrule
            heat-3d & 7-42-M-3.04E+07 & 0.23 &  & 3.75 & 402 & 17 & 7 &  & 3.75 & 928 & 75 & 33 & 35 &  & 2.31x & 1.00x \\ 
        heat-3d & 742-L-4.37E+07 & 0.13 &  & 0.62 & 520 & 13 & 6 &  & 0.63 & 740 & 109 & 70 & 35 &  & 1.42x & 0.99x \\ 
        jacobi-1d & 3-14-M-1.48E+03 & 11.43 &  & 11.43 & 55 & 4 & 0 &  & 11.53 & 948 & 126 & 3 & 74 &  & 17.24x & 0.99x \\ 
        jacobi-1d & 3-14-L-4.00E+04 & 5.95 &  & 5.95 & 386 & 9 & 6 &  & 2.65 & 1,283 & 173 & 21 & 123 &  & 3.32x & 2.25x \\ 
        jacobi-2d & 5-22-M-8.07E+06 & 0.20 &  & 3.32 & 379 & 12 & 5 &  & 3.32 & 674 & 158 & 26 & 98 &  & 1.78x & 1.00x \\ 
        jacobi-2d & 5-22-L-1.14E+07 & 0.26 &  & 1.25 & 427 & 9 & 6 &  & 1.25 & 1,106 & 231 & 39 & 171 &  & 2.59x & 1.00x \\ 
                seidel-2d & 3-27-M-4.26E+03 & 0.05 &  & 0.05 & 365 & 5 & 1 &  & 0.05 & 796 & 103 & 27 & 68 &  & 2.18x & 1.01x \\ 
        seidel-2d & 3-27-L-1.77E+05 & 0.05 &  & 0.05 & 540 & 13 & 7 &  & 0.05 & 880 & 91 & 33 & 48 &  & 1.63x & 1.00x \\ 
\midrule
% Average &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
% Geo. Mean &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
Average &    & 5.38 &  & 15.11 & 296 &  &  &  & 7.44 & 1,123 &  &  &  &  & 5.69x & 17.2x \\
Geo. Mean &    & 0.51 &  & 1.54 & 247 &  &  &  & 0.65 & 916 &  &  &  &  & 3.70x & 2.38x \\
\bottomrule

\end{tabular}
% \end{spacing}
% \vspace{0.4cm}
\end{adjustwidth}
\caption{
Comparison of DSE time and Throughput for \framework, \framework-FS, and AutoDSE across Polybench kernels at different problem sizes: NL, ND, S, and Space S denote the number of loops,  dependencies, problem size (L for Large and M for Medium), and space size, respectively. GF/s indicates throughput, T represents DSE time (min), DE signifies the number of explored designs, and DT denotes timeout designs. Additionally, ET reflects the count of designs early rejected/pruned by AutoDSE
}

\label{tab:eval}
% \vspace{-0.8cm}
% \end{adjustheight}

\end{table}
% \restoregeometry
% % \vspace{-0.4cm}




==> sources/tablev3.tex <==

% Need to remove \renewcommand{\arraystretch}{0.9}

\begin{table*}[htb]
\centering

\begin{tabular}{|l rrrr|r|rrrr|rrrrr|rr|}
% \begin{tabular}{@{}l rrrrrrrrrrrrrrrr@{}}
% \toprule
\hline
 &  &  &  &  & FS  & \multicolumn{3}{l}{\textbf{NLP}} &  & \multicolumn{4}{l}{\textbf{AutoDSE}} &  & \multicolumn{1}{l}{\textbf{SpeedUp}} &  \\
\cline{6-17}

\textbf{Kernel} & \textbf{NL} & \textbf{ND} & \textbf{S} & \textbf{Space S} & \textbf{GF/s}  &\textbf{GF/s} & \textbf{T} & \textbf{DE} & \textbf{DT}  & \textbf{GF/s} & \textbf{T} & \textbf{DE} & \textbf{DT} & \textbf{ER}  & \textbf{T} & \textbf{GF/s} \\
\hline
        2mm & 6 & 13 & L & 1.15E+12 & 0.57 & 2.17 & 456 & 17 & 3 & 0.40 & 1,835 & 291 & 38 & 240 & 4.02 & 5.41 \\ 
        2mm & 6 & 13 & M & 1.37E+10 & 13.19 & 117.48 & 70 & 18 & 0 & 0.41 & 1,870 & 101 & 37 & 49 & 26.71 & 288.88 \\ 
        3mm & 9 & 19 & L & 6.18E+17 & 0.18 & 1.01 & 486 & 19 & 3 & 0.59 & 968 & 112 & 18 & 81 & 1.99 & 1.71 \\ 
        3mm & 9 & 19 & M & 1.20E+15 & 13.86 & 138.73 & 242 & 18 & 0 & 0.39 & 698 & 82 & 15 & 57 & 2.88 & 354.12 \\ 
        atax & 4 & 12 & L & 1.60E+07 & 0.47 & 1.52 & 205 & 11 & 2 & 0.44 & 2,325 & 166 & 30 & 106 & 11.34 & 3.46 \\ 
        atax & 4 & 12 & M & 1.40E+05 & 1.96 & 1.96 & 194 & 10 & 1 & 1.98 & 1,653 & 175 & 13 & 136 & 8.52 & 0.99 \\ 
        bicg & 3 & 10 & L & 4.44E+05 & 1.68 & 1.68 & 218 & 12 & 1 & 0.50 & 3,355 & 236 & 42 & 176 & 15.39 & 3.38 \\ 
        bicg & 3 & 10 & M & 1.90E+04 & 0.99 & 0.99 & 248 & 12 & 1 & 0.98 & 729 & 65 & 2 & 28 & 2.94 & 1.01 \\ 
        covariance & 7 & 34 & L & 1.92E+13 & 0.39 & 0.73 & 466 & 21 & 9 & 0.62 & 2,849 & 209 & 68 & 118 & 6.11 & 1.16 \\ 
        covariance & 7 & 34 & M & 1.80E+11 & 0.08 & 0.75 & 336 & 21 & 8 & 0.28 & 645 & 161 & 15 & 115 & 1.92 & 2.64 \\ 
        doitgen & 5 & 30 & L & 3.63E+07 & 0.08 & 102.62 & 241 & 20 & 1 & 110.66 & 1,299 & 222 & 24 & 169 & 5.39 & 0.93 \\ 
        doitgen & 5 & 30 & M & 8.64E+06 & 19.75 & 19.75 & 193 & 13 & 0 & 18.95 & 819 & 296 & 14 & 248 & 4.24 & 1.04 \\ 
        durbin & 4 & 55 & L & 9.00E+00 & 0.12 & 0.12 & 212 & 3 & 1 & 0.12 & 31 & 7 & 0 & 5 & 0.15 & 1.00 \\ 
        durbin & 4 & 55 & M & 1.08E+02 & 0.01 & 0.20 & 193 & 7 & 4 & 0.12 & 134 & 25 & 0 & 23 & 0.69 & 1.65 \\ 
        fdtd-2d & 8 & 28 & L & 6.47E+11 & 0.88 & 0.92 & 630 & 19 & 17 & 0.92 & 1,103 & 62 & 20 & 24 & 1.75 & 1.00 \\ 
        fdtd-2d & 8 & 28 & M & 3.30E+08 & 166.33 & 166.33 & 342 & 14 & 2 & 162.53 & 1,135 & 81 & 12 & 37 & 3.32 & 1.02 \\ 
        floyd-warshall & 3 & 21 & L & 3.29E+06 & 0.17 & 1.31 & 381 & 20 & 6 & 0.10 & 2,728 & 150 & 71 & 77 & 7.16 & 13.09 \\ 
        floyd-warshall & 3 & 21 & M & 8.65E+04 & 0.17 & 0.61 & 246 & 17 & 3 & 0.10 & 1,605 & 60 & 22 & 29 & 6.52 & 6.15 \\ 
        gemm & 4 & 6 & L & 1.47E+07 & 32.98 & 32.98 & 450 & 18 & 7 & 2.77 & 2,810 & 188 & 47 & 133 & 6.24 & 11.89 \\ 
        gemm & 4 & 6 & M & 2.30E+06 & 105.18 & 105.18 & 185 & 21 & 1 & 68.91 & 1,345 & 86 & 27 & 34 & 7.27 & 1.53 \\ 
        gemver & 7 & 13 & L & 1.28E+13 & 9.94 & 9.94 & 290 & 21 & 7 & 0.18 & 1,756 & 221 & 206 & 10 & 6.06 & 54.69 \\ 
        gemver & 7 & 13 & M & 7.72E+11 & 0.78 & 9.45 & 218 & 21 & 4 & 2.99 & 847 & 65 & 5 & 28 & 3.89 & 3.16 \\ 
        gesummv & 2 & 17 & L & 6.33E+03 & 1.82 & 2.64 & 236 & 18 & 1 & 0.56 & 692 & 94 & 29 & 60 & 2.93 & 4.73 \\ 
        gesummv & 2 & 17 & M & 6.12E+02 & 1.97 & 1.97 & 220 & 14 & 3 & 1.97 & 836 & 80 & 8 & 47 & 3.80 & 1.00 \\ 
        gramschmidt & 6 & 34 & L & 1.22E+08 & 2.34 & 2.34 & 420 & 6 & 4 & 0.95 & 819 & 265 & 11 & 239 & 1.95 & 2.47 \\ 
        gramschmidt & 6 & 34 & M & 1.75E+07 & 1.58 & 1.58 & 364 & 7 & 3 & 0.44 & 934 & 109 & 92 & 8 & 2.57 & 3.56 \\ 
        heat-3d & 7 & 42 & L & 4.37E+07 & 0.13 & 0.62 & 520 & 13 & 6 & 0.63 & 740 & 109 & 70 & 35 & 1.42 & 0.99 \\ 
        heat-3d & 7 & 42 & M & 3.04E+07 & 0.23 & 3.75 & 402 & 17 & 7 & 3.75 & 928 & 75 & 33 & 35 & 2.31 & 1.00 \\ 
        jacobi-1d & 3 & 14 & L & 4.00E+04 & 5.95 & 5.95 & 386 & 9 & 6 & 2.65 & 1,283 & 173 & 21 & 123 & 3.32 & 2.25 \\ 
        jacobi-1d & 3 & 14 & M & 1.48E+03 & 11.43 & 11.43 & 55 & 4 & 0 & 11.53 & 948 & 126 & 3 & 74 & 17.24 & 0.99 \\ 
        jacobi-2d & 5 & 22 & L & 1.14E+07 & 0.26 & 1.25 & 427 & 9 & 6 & 1.25 & 1,106 & 231 & 39 & 171 & 2.59 & 1.00 \\ 
        jacobi-2d & 5 & 22 & M & 8.07E+06 & 0.20 & 3.32 & 379 & 12 & 5 & 3.32 & 674 & 158 & 26 & 98 & 1.78 & 1.00 \\ 
        lu & 5 & 16 & L & 3.99E+03 & 0.03 & 0.04 & 335 & 9 & 2 & 0.03 & 812 & 258 & 5 & 219 & 2.42 & 1.03 \\ 
        lu & 5 & 16 & M & 2.28E+03 & 0.03 & 0.03 & 614 & 19 & 11 & 0.04 & 849 & 193 & 1 & 159 & 1.38 & 0.98 \\ 
        mvt & 4 & 6 & L & 7.41E+07 & 12.90 & 12.90 & 181 & 20 & 3 & 1.10 & 1,240 & 249 & 20 & 189 & 6.85 & 11.78 \\ 
        mvt & 4 & 6 & M & 1.38E+07 & 7.77 & 7.77 & 212 & 17 & 1 & 7.77 & 893 & 166 & 6 & 106 & 4.21 & 1.00 \\ 
        seidel-2d & 3 & 27 & L & 1.77E+05 & 0.05 & 0.05 & 540 & 13 & 7 & 0.05 & 880 & 91 & 33 & 48 & 1.63 & 1.00 \\ 
        seidel-2d & 3 & 27 & M & 4.26E+03 & 0.05 & 0.05 & 365 & 5 & 1 & 0.05 & 796 & 103 & 27 & 68 & 2.18 & 1.01 \\ 
        symm & 3 & 33 & L & 6.64E+04 & 0.21 & 0.31 & 540 & 8 & 5 & 0.21 & 612 & 731 & 0 & 692 & 1.13 & 1.52 \\ 
        symm & 3 & 33 & M & 2.31E+04 & 0.04 & 0.20 & 63 & 5 & 0 & 0.20 & 691 & 142 & 35 & 89 & 10.97 & 1.00 \\ 
        syr2k & 4 & 6 & L & 6.67E+04 & 1.30 & 1.42 & 420 & 15 & 7 & 1.30 & 768 & 293 & 21 & 262 & 1.83 & 1.09 \\ 
        syr2k & 4 & 6 & M & 2.32E+04 & 0.07 & 1.74 & 224 & 16 & 2 & 1.20 & 685 & 230 & 17 & 203 & 3.06 & 1.45 \\ 
        syrk & 4 & 6 & L & 6.67E+04 & 0.94 & 2.07 & 466 & 17 & 7 & 0.65 & 643 & 410 & 0 & 398 & 1.38 & 3.16 \\ 
        syrk & 4 & 6 & M & 2.32E+04 & 0.49 & 1.32 & 224 & 16 & 2 & 0.61 & 631 & 280 & 4 & 264 & 2.82 & 2.15 \\ 
        trisolv & 2 & 13 & L & 6.30E+02 & 0.04 & 0.04 & 75 & 18 & 0 & 0.04 & 651 & 127 & 2 & 98 & 8.68 & 0.99 \\ 
        trisolv & 2 & 13 & M & 3.60E+02 & 0.03 & 0.03 & 69 & 12 & 0 & 0.04 & 694 & 69 & 33 & 23 & 10.06 & 0.98 \\ 
        trmm & 3 & 8 & L & 6.64E+04 & 0.02 & 0.06 & 425 & 17 & 2 & 0.03 & 760 & 167 & 159 & 4 & 1.79 & 1.79 \\ 
        trmm & 3 & 8 & M & 2.31E+04 & 0.01 & 0.05 & 20 & 16 & 0 & 0.04 & 630 & 401 & 4 & 367 & 31.50 & 1.29 \\ 
        \hline

\end{tabular}

\caption{Comparison with AutoDSE}
\label{tab:eval}

\end{table*}


==> sources/th_proof.tex <==
% \section{Analytical Model}

% \label{sec:appendix}
\label{sec:theoretical}


We now outline key elements of our analytical performance model, and the associated proofs this model computes a lower bound on latency under resource constraints. 

% Full proofs cover several pages, and are available in a separate research report: we limit below to summarizing the hypothesis and overall proof approach.

\subsection{Analytical Model Template}
\label{sec:analyticalModelTemplate}


Let $I^{\vec PV_i}_i(X)$ the operators defined as follows:
$$
I^{\vec PV_i}_i(X) = \lfloor II_i * (TC^{avg}_i /uf_i - ispipelined_i)  \rfloor \odot X
$$
where $\odot$ is $+$ if $ispipelined_i = 1$, $*$ otherwise. We also have:

$
C_i^{\vec PV_i}(X_1, X_2, ..., X_n) = max(X_1, X_2, ..., X_n)~~~if~~~inparallel_i %pf_i + uf_i > 2
$

and

$
C_i^{\vec PV_i}(X_1, X_2, \dots, X_n) = \sum_{k=1}^n X_k~~~if~~~insequence_i 
%pf_i + uf_i = 2
$

with $inparallel_i = 1 = 1 - insequence_i$ if $(X_1, X_2, \dots, X_n)$  do not have dependencies (WaR, RaW, WaW) else 0.
Finally, $SL^{\vec PV_i}_i(\vec S_k)$ denotes a region of straight-line code (e.g., an inner-loop body). 
% which is used below in the formal reasoning on the bounds on latency of this template formula. 
Intuitively, $SL$ will represent a lower bound on the latency of a code block such that by composition across all loops as per the template formula, the result remains a lower bound on the full program latency. 

Given the summary AST of the program in constructor form, and the set of $\vec PV_i$ vectors for each loop, we build the analytical formula template as follows: 
\begin{enumerate}
    \item replace the $Loop_i(\vec X)$ operator by $I^{\vec PV_i}_i(\vec X)$ operator;
    \item replace the $\vec X$ list by $C^{\vec PV_i}_i(\vec X)$;
    \item replace statement lists inside loop \texttt{i} $\vec S_x$ by $SL^{\vec PV_i}_i(\vec S_x)$.
\end{enumerate}
That is for our example, we simply rewrite:
$
Loop_i(Loop_{j1}(S1), Loop_{j2}(S2,S3))
$
into

$
I^{\vec PV_i}_i(C^{\vec PV_i}(I^{\vec PV_{j1}}_{j1}(SL^{\vec PV_{j1}}_{j1}(S1)), I^{\vec PV_{j2}}_{j2}(SL^{\vec PV_{j2}}_{j2}(S2,S3))))
$.

2mm on Listing \ref{lst:2mm}  can be represented by: 
$
(Loop_{i_1}(Loop_{j_1}(S_0, Loop_{k_1}(S1))) , Loop_{i_2}(Loop_{j_2}(S_2, Loop_{k_2}(S3))))
$. If we apply the definition of $C^{PV}$ and $I^{PV}$ we have the following equation:

% I^{\vec PV_{i_1}}_{i_1}
$
(
    I^{\vec PV_{i_1}}_{i_1}(
        I^{\vec PV_{j_1}}_{j_1}(
            C_{j_1}^{\vec PV_{j_1}}(
                SL^{\vec PV_{j_1}}_{j_1}(S_0), 
                I^{\vec PV_{k_1}}_{k_1}(
                    SL^{\vec PV_{k_1}}_{k_1}(S1)
                )
            )
        )
    ) , 
    I^{\vec PV_{i_2}}_{i_2}(
        I^{\vec PV_{j_2}}_{j_2}(
            C_{j_1}^{\vec PV_{j_2}}(
                SL^{\vec PV_{j_2}}_{j_2}(S_2), 
                I^{\vec PV_{k_2}}_{k_2}(
                    SL^{\vec PV_{k_2}}_{k_2}(S3)
                )
            )
        )
    )
)
$
.

Upon substituting the definition, we acquire:

$
(
    % I^{\vec PV_{i_1}}_{i_1}(
    \lfloor II_{i_1} * (TC^{avg}_{i_1} /uf_{i_1} - ispipelined_{i_1})  \rfloor \odot 
        % I^{\vec PV_{j_1}}_{j_1}(
        \lfloor II_{j_1} * (TC^{avg}_{j_1} /uf_{j_1} - ispipelined_{j_1})  \rfloor \odot 
            % C_{j_1}^{\vec PV_{j_1}}(
            sum(
                SL^{\vec PV_{j_1}}_{j_1}(S_0), 
                % I^{\vec PV_{k_1}}_{k_1}(
                \lfloor II_{k_1} * (TC^{avg}_{k_1} /uf_{k_1} - ispipelined_{k_1})  \rfloor \odot 
                    SL^{\vec PV_{k_1}}_{k_1}(S1)
                )
            )
        )
    ) , 
    % I^{\vec PV_{i_2}}_{i_2}(
   \lfloor II_{i_2} * (TC^{avg}_{i_2} /uf_{i_2} - ispipelined_{i_2})  \rfloor \odot 
        % I^{\vec PV_{j_2}}_{j_2}(
        \lfloor II_{j_2} * (TC^{avg}_{j_2} /uf_{j_2} - ispipelined_{j_2})  \rfloor \odot 
            % C_{j_1}^{\vec PV_{j_2}}(
            sum(
                SL^{\vec PV_{j_2}}_{j_2}(S_2), 
                % I^{\vec PV_{k_2}}_{k_2}(
                \lfloor II_{k_2} * (TC^{avg}_{k_2} /uf_{k_2} - ispipelined_{k_2})  \rfloor \odot 
                    SL^{\vec PV_{k_2}}_{k_2}(S3)
                )
            )
        )
    )
)
$.





% \subsection{Restrictions and Applicability}

% Our objective is to formulate a lower bound on the latency of a program, after HLS. We therefore put several restrictions:
% \begin{itemize}[leftmargin=*]
%     \item The input program is a pure polyhedral program \cite{girbal06ijpp}, and its analysis (loop trip counts for every loop, all data dependencies \cite{Fea91}) is exact.
%     \item No HLS optimization shall change the number of operations in the computation: strength reduction, common sub-expression elimination, etc. shall either first be performed in the input program before analysis, or not be performed by the HLS toolchain.
%     \item The program does not contain "useless" operations. A typical case is when a value is overwritten before being used, e.g. \texttt{x = 42+51; x = 0;}.
%     \item We only model DSP and BRAM resources for the considered kernel, ignoring all other resources.
%     \item We assume resource (DSP) sharing across different operations executing at the same cycle is not possible.
% \end{itemize}

\subsection{A Formal Model for Latency}

Our objective is to formulate a lower bound on the latency of a program after HLS. We therefore have put several restrictions: we assume the input program is a polyhedral program, that is the control-flow is statically analyzable; all loops can be recognized and their trip count computed; and all array / memory accesses can be exactly modeled at compile-time. No conditional can occur in the program. While our approach may generalize beyond this class, we limit here to these strict assumptions.

To maintain a lower bound on latency by composition, we operate on a representation of (parts of the) program which is both schedule-independent and storage-independent: indeed, a lower bound on this representation is necessarily valid under any schedule and storage eventually implemented. \emph{We however require HLS to not change the count and type of operations}. Furthermore, for lower bounding purposes, we assume unless stated otherwise $\forall i,~inparallel_i = 1$. We will discuss in the next section a more realistic but compiler-dependent approach to set $inparallel_i$, based on dependence analysis.

We assume programs are made of affine loops, that are loops with statically computable control-flow, with loop bounds made only of intersection of affine expressions of surrounding loop iterators and program constants. We now assume loop bodies (i.e., statements surrounded by loops) have been translated to a list of statements, with at most a single operation (e.g., \texttt{+,-,/,*}) per statement. Operations are n-ary, that is they take $n \ge 0$ input scalar values as operand, and produce 0 or 1 output scalar value. A memory location can be loaded from (resp. stored to) an address stored in a scalar variable. This is often referred to as straight-line code
% \cite{some-good-def}
. 
This normalization of the loop body facilitates the computation of live-in/live-out data for the code block, and the extraction of the computation graph. Note the region can be represented in Static Single Assignment 
% \cite{ssa} 
form, to ensure different storage location for every assignment, facilitating the construction of the operation graph.
% 
In addition we require the input program to not contain useless operations which may be removed by the HLS toolchain e.g. by dead code elimination, as illustrated in Listing~\ref{lst:dead-code}.


\begin{lstlisting}[caption={Example of Code Illustrating Dead Code Elimination: As Statement S1 writes to variable x, but the value of x assigned in Statement S0 is never used, the compiler will remove Statement S0.},label={lst:dead-code}]
int example(int y, int z){
    int x;
    S0: x = 12 + y; //  dead-code elimination
    S1: x = y + z;
    return x;
}
\end{lstlisting}
\vspace{0.7cm}


The restriction can be summarized as:

\begin{itemize}[leftmargin=*]
    \item The input program is a pure polyhedral program \cite{girbal06ijpp}, and its analysis (loop trip counts for every loop, all data dependences \cite{Fea92b}) is exact.
    \item No HLS optimization shall change the number of operations in the computation: strength reduction, common sub-expression elimination, etc. shall either first be performed in the input program before analysis, or not be performed by the HLS toolchain. The program also does not contain "useless" operations that may be removed by the compiler.
    \item We only model DSP and BRAM resources for the considered kernel, ignoring all other resources. We do not model LUT and FF resources, because from experience in the loop-based benchmarks we consider DSP and BRAM resources are the most constraining resources. Moreover, the estimation of LUTs and FFs is more tedious.
    \item We assume resource (DSP) sharing across different operations executing at the same cycle is not possible.
\end{itemize}

An important term is $SL$, a latency lower bound for a region of straight-line code. To maintain a lower bound on latency by composition, we operate on a representation of (parts of the) program which is both schedule-independent and storage-independent: the operation graph, or CDAG \cite{elango2015characterizing}. Indeed, a lower bound on this representation is necessarily valid under any schedule and storage eventually implemented and can be used to prove I/O lower bounds on programs \cite{elango2015characterizing} which is the directed acyclic graph with one node per operation in the code region, connecting all producer and consumer operations to build the operation graph. Then, we can easily compute the length of its critical path, which represents the minimal set of operations to execute serially.

% Then, we can build a lower bound on the number of cycles a region $L$ may require to execute, under fixed resources, by simply taking the maximum between the weighted critical path and the work to execute normalized by the resources available.

\begin{definition}[Straight-line code]
\label{def:straightlinecode}
An n-ary operation takes n scalar operands $\vec i$ as input, and produces a single scalar $o$ as output. A statement contains a single n-ary operation, or a load from (resp. store to) a memory location to (resp. from) a scalar. A straight-line code region $L$ is a list of consecutive statements, with a single entry and single exit.
\end{definition}

\begin{definition}[Live-in set] The live-in set $V_I^L$ of region $L$ is the set of scalar values, variables and memory locations that read before being written, under any possible valid execution of $L$.
\end{definition}

\begin{definition}[Live-out set] The live-out set $V_O^L$ of region $L$ is the set of variables and memory locations that written to during any possible valid execution of $L$.
\end{definition}

%%% LNP: I think it's not useful for the reader.
%On the listing \ref{lst:dead-code}, $V_O^L = \{x\}$ and $V_I^L = \{y, z\}$. 
%On the listing \ref{lst:2mm}, let be $L$ the region of the first loop body,
%$V_O^{L} = \{tmp[i_1][j_1], \forall i_1,j_1 \text{ s.t. } 0 \leq i_1 \leq 180 \And 0 \leq j_1 \leq 190  \}$ and $V_I^{L} = \{B[k_1][j_1], \forall k_1,j_1 \text{ s.t. } 0 \leq k_1 \leq 210 \And 0 \leq j_1 \leq 190  \} \cup \{A[i_1][k_1], \forall i_1,k_1 \text{ s.t. } 0 \leq i_1 \leq 180 \And 0 \leq k_1 \leq 210  \} \cup \{alpha\}$. 

We can compute the directed acyclic graph made of all statements (i.e., all n-ary operations), connecting all producer and consumer operations, to build the operation graph: % 
% \cite{someothergoodref}:

\begin{definition}[Operation Graph] 
\label{def:computationgraph}
Given a straight-line code region $R$ made of a list $L$ of statements $S \in L$, the operation graph OG is the directed graph $<\{N,V_I,root,V_O\},E>$ such that $\forall S_i \in L,~N_{S_i} \in N$; and for every operation with output $o$ and inputs $\vec i$ in $L$ $\forall S_i, \forall i_k \in \Vec{i}_{S_i}, e_{i_k, o} \in E$,
$\forall S_i:(o_{S_i},{\vec i}_{S_i}) \in L, S_j:(o_{S_j},{\vec i}_{S_j}) \in L$ with $S_i \ne S_j$ then we have $E_{S_i,S_j} \in E$ iff $o_{Si}\cap{\vec i}_{S_j}\ne \emptyset$. For every input (resp. output) in $S_i$ which is not matched with an output (resp. input) of another $S_j$ in $L$, create a node $V_{val} \in V_I$ (resp. $V_O$) for this input (resp. output) value. If $dim({\vec i}_{S_i}) = 0$ then an edge $e_{root,S_i}$ is added to $E$.
\end{definition}

% \begin{lstlisting}[caption={Example},label={lst:og}]
% A[0] = B[0] + C[0];
% A[1] = B[1] + C[1];
% D[0] = E[0] + A[0];
% D[1] = E[1] + A[1];
% \end{lstlisting}
% \vspace{0.7cm}

% \begin{figure}[htb]
%     \centering
%     \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=1.5cm,semithick]
%     % \begin{tikzpicture}[>=Stealth, auto, shorten >=1pt, semithick, rounded corners]

%         % Nodes
%         \node[draw, circle] (Root) {root};
%         \node[coordinate, below=of Root] (FakeNode) {};
%         \node[draw, circle, left=of FakeNode] (B0) {B[0]};
%         \node[draw, circle, right=of FakeNode] (B1) {B[1]};
%         \node[draw, circle, left=of B0] (C0) {C[0]};
%         \node[draw, circle, right=of B1] (C1) {C[1]};
%         \node[draw, circle, below=of B0] (A0) {A[0]};
%         \node[draw, circle, below=of B1] (A1) {A[1]};
%         \node[draw, circle, below=of A0] (D0) {D[0]};
%         \node[draw, circle, below=of A1] (D1) {D[1]};
%         \node[draw, circle, left=of C0] (E0) {E[0]};
%         \node[draw, circle, right=of C1] (E1) {E[1]};
%         % \node[draw, circle, below=of Root] (A0) {A[0]};
%         % \node[draw, circle, below=of Root] (A1) {A[1]};
%         % \node[draw, circle, below=of Root] (B0) {B[0]};
%         % \node[draw, circle, below=of Root] (B1) {B[1]};
%         % \node[draw, circle, below=of Root] (C0) {C[0]};
%         % \node[draw, circle, below=of Root] (C1) {C[1]};
%         % \node[draw, circle, below=of Root] (D0) {D[0]};
%         % \node[draw, circle, below=of Root] (D1) {D[1]};
%         % \node[draw, circle, below=of Root] (E0) {E[0]};
%         % \node[draw, circle, below=of Root] (E1) {E[1]};



        

%         % Edges
%         \draw[->] (Root) -- (B0);
%         \draw[->] (Root) -- (B1);
%         \draw[->] (Root) -- (C0);
%         \draw[->] (Root) -- (C1);
%         \draw[->] (Root) -- (E0);
%         \draw[->] (Root) -- (E1);

%         \draw[->] (B0) -- (A0);
%         \draw[->] (C0) -- (A0);
%         \draw[->] (B1) -- (A1);
%         \draw[->] (C1) -- (A1);

%         \draw[->] (A0) -- (D0);
%         \draw[->] (E0) -- (D0);
%         \draw[->] (A1) -- (D1);
%         \draw[->] (E1) -- (D1);
        

%     \end{tikzpicture}
%     \caption{Operation Graph Example}
%     \label{fig:operation_graph}
% \end{figure}

% On Figure \ref{fig:operation_graph}, we can see the operation graph of the listing \ref{lst:og}.

From this representation, we can easily define key properties to subsequently estimate the latency and area of this code region, such as its span, or critical path. % \cite{someone}.

\begin{definition}[Operation Graph critical path]
\label{def:ogcriticalpath}
Given $OG^L$ an operation graph for region $L$. Its critical path $OG_{cp}$ is the longest of all the shortest paths between every pairs $(v_i,v_o) \in <\{V_I,root\},V_O>$. 
% Its length, in number of nodes, is noted $\#OG_{cp}^L$.
Its length is noted $\#OG_{cp}^L$.
\end{definition}

% \FIXME{Link with the other operation graph}

On the graph on the Figure \ref{fig:tree_diagram} the critical paths from $A[i]$ to 
$c, \forall i \in$ \([\![0, 7]\!]\), 
have the same length.


\subsubsection{Latency Lower Bound}

We can build a simple a lower bound on the latency of an operation graph:
\begin{theorem}[Lower bound on latency of an Operation Graph]
\label{th:latlbcp}
Given infinite resources, and assuming no operation nor memory movement can take less than one cycle to complete, the latency $LAT_{cp}^L \ge \#OG_{cp}^L$ is a lower bound on the minimal feasible latency to execute $L$.
\end{theorem}

\begin{proof}[Proof Th \ref{th:latlbcp}]
Every operation $S_i$ is associated with at least one edge with a source in $<\{V_I,root\}>$, so there is a path between one of these nodes and every operation by construction in Def.~\ref{def:computationgraph}. For an operation to produce a useful output, there must be a path from its output to a node in $V_O$, otherwise the operation may be removed by dead code elimination. Therefore the shortest path $sp$ between a pair of nodes $(v_i, v_o) \in <\{V_I,root\},V_O>$ is the shortest sequence of operations in dependence that must be executed to produce $v_o$. As any operation takes at least one cycle to complete per Def.~\ref{th:latlbcp}, then this path must take at least $\#sp$ cycles to complete. As we take the largest of the shortest paths between all possible pairs  $(v_i, v_o)$ then $OG_{cp}^L$ is the length of the longest shortest path to produce any output $v_o$ from some input, via a sequence of producer-consumer operations. Therefore it must take at least $\#OG_{cp}^L$ cycles to execute this path.
\end{proof}


%\begin{proof}
%% probably have to show that if it was to take less cycles, then it would have to be because there is an operation taking less than 1 cycle?
%By definition the critical path is the longest path of all the shortest paths between every pairs of node $(v_i,v_o) \in <V_I,V_O>$ through the OG graph and the lower bound of the latency is the minimal number of cycles to perform all operations while respecting the dependencies.
%Suppose the critical path is not the lower bound then there is another path through the graph such that all operations are executed that is shorter than the critical path. Which is false by contradiction.
%Hence, the critical path is the lower bound.
%\end{proof}


We can then build a tighter lower bound on the number of cycles a region $L$ may take to execute, under fixed resources, by simply taking the maximum between the weighted span and the work to execute normalized by the resources available.

\begin{theorem}[Latency Lower Bound under Operation Resource Constraints] 
\label{th:latlbresources}
Given $R_{op}$ a count of available resources of type $op$, for each operation type, and $LO(op)$ the latency function for operation $op$, with $LO(op) \ge 1$. $\#L(op)$ denotes the number of operations of type $op$ in $L$. We define $LO(\#OG_{cp}^L) = \sum_{n \in cp} LO(n)$ the critical path weighted by latency of its operations.
The minimal latency of a region $L$ is bounded by 
$$
Lat_{R_{op}}^L \ge \max(LO(\#OG_{cp}^L),\max_{o \in op} (\lceil \#L(o) \times LO(o) /R_{o}\rceil))
$$
\end{theorem}

\begin{proof}[Proof Th \ref{th:latlbresources}]
Suppose $\forall o \in op,~R_{o} \ge \#L(o) $. Then there is equal or more resources available than work to execute, this is equivalent to the infinite resource hypothesis of Th.~\ref{th:latlbcp}, the minimal latency is $LO(\#OG_{cp}^L)$.

Suppose $\exists o \in op,~R_{o} < \#L(o)  $. Then there exists at least one unit in $R_{o}$ that is executing $\lceil \#L(o) /R_{o} \rceil$ operations. As every operation $op$ take at $L(op) \ge 1$ cycle to complete, this unit will execute in at least  $\lceil \#L(o) \times L_{o}/R_{o} \rceil$ cycles. If $\lceil \#L(o) \times L_{o}/R_{o} \rceil \ge LO(\#OG_{cp}^L)$, the computation cannot execute in less than $\lceil \#L(o) \times L_{o}/R_{o} \rceil$ cycles.
\end{proof}

% \FIXME{May here show an ILP formulation on the CDAG that achieves the lower bound, and reason that all are (over-)approximations of this perfect scheduling+placement solution?}

This theorem provides the building block to our analysis: if reasoning on a straight-line code region, without any loop, then building the operation graph for this region and reasoning on its critical path is sufficient to provide a latency lower bound. 

\begin{lstlisting}[label={lst:reference_bicg},caption={Bicg code: $s=r \times A; q=A \times p$}]
L1: for (i = 0; i < N; i++)  
    S0: s[i] = 0;
L2: for (i = 0; i < M; i++) { 
        S1: q[i] = 0;
    L3: for (j = 0; j < N; j++) {
        S2: s[j]+=r[i]*A[i][j]; 
        S3: q[i]+=A[i][j]*p[j];
    }
}
\end{lstlisting}
\vspace{.5cm}
For example, in Listing~\ref{lst:reference_bicg}, if we consider the sub-loop body composed of loops L3 (fully unrolled) and the statements $S2$ and $S3$ as straight-line code regions, we can calculate the critical paths for $S2$ and $S3$ as follows:
% 
For $S2$, the critical path is given by: $cp_{S2} = \max(L(+) + L(*), N \times (DSP_+ + DSP_*) / R_o)$ with $DSP_{o}$ the number of DSP for the operation $o$.
For $S3$, the critical path is determined by: $cp_{S3} = \max(L(+) \times \log(N) + L(*), N \times (DSP_+ + DSP_*) / R_o)$,  considering the possibility of a tree reduction.
In this context, the critical path for the entire sub-loop body is the maximum of these two individual critical paths, expressed as $\max(cp_{S2}, cp_{S3})$.

We now need to integrate loops and enable the composition of latency bounds.


\subsubsection{Loop Unrolling: full unroll}

% Loop unrolling is an HLS optimization that aims to execute multiple iterations of a loop in parallel. Intuitively, for an unroll factor $UF \ge 1$, $UF$ replications of the loop body will be instantiated. If $TC_l \mod UF_l \ne 0$ then an epilogue code to execute the remaining $TC_l \mod UF_l$ iterations is needed.

% We can bound the latency of a loop nest which has been entirely flatten, that is, all loops have been fully unrolled.

We start by reasoning on the bound for latency of a loop nest which has been fully unrolled, e.g. as a result of \texttt{\#pragma ACCEL parallel} or \texttt{\#pragma HLS unroll}. Full unrolling amounts to fully unroll all $TC$ iterations of a loop, replacing the loop by $TC$ replications of its original loop body, where the loop iterator has been updated with the value it takes, for each replication.

It follows a simple corollary:
\begin{corollary}[Equivalence between fully unrolled and straight-line code]
\label{cor:fullflattenstraightlinecode}
Given a loop nest $l$, if full unrolling is applied to $l$ then the code obtained after full unrolling is a straight-line code as per Def.~\ref{def:straightlinecode}.
\end{corollary}

\begin{proof}[Proof Co \ref{cor:fullflattenstraightlinecode}]
By construction the process of fully unrolling all the loops creates a straight-line code region without loop control, which therefore fits Def.~\ref{def:straightlinecode}.
\end{proof}

Consequently, we can bound the latency of a fully unrolled loop nest:
\begin{theorem}[Minimal latency of a fully unrolled loop nest]
\label{th:minlatflattenednest}
Given a loop nest $l$, which is first rewritten by fully unrolling all loops to create a straight-line code region $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then its minimal latency is bounded by:
$$
Lat_{R_{op}}^l \ge \max(LO(\#OG_{cp}^L),\max_{o \in op} (\lceil \#L(o) \times L_{o}/R_{o} \rceil))
$$
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatflattenednest}]
By Corollary~\ref{cor:fullflattenstraightlinecode}.
\end{proof}

\subsubsection{Loop Unrolling: partial unroll} 

Loop unrolling is an HLS optimization that aims to execute multiple iterations of a loop in parallel. Intuitively, for an unroll factor $UF \ge 1$, $UF$ replications of the loop body will be instantiated. If $TC_l \mod UF_l \ne 0$ then an epilogue code to execute the remaining $TC_l \mod UF_l$ iterations is needed.

% \FIXME{NOTE: write here some comment on what happens if you unroll non-rectangular loops, loops where UF does not divide TC, etc. from the Merlin/Vitis implementation point of view.}

% Partial unrolling can be viewed as a two-step transformation: first strip-mine the loop by the unroll factor, then consider the inner loop obtained is fully-unrolled. The latency of the resulting sub-program is determined by how the outer-loop generated will be implemented. We assume without additional explicit information this outer loop will execute in a non-pipelined, non-parallel fashion, to provide the following bound:

Unrolling can be viewed as a two-step transformation: first strip-mine the loop by the unroll factor, then consider the inner loop obtained to be fully-unrolled. The latency of the resulting sub-program is determined by how the outer-loop generated will be implemented. 
We assume without additional explicit information this unrolled loop will execute in a non-pipelined, non-parallel fashion.
Note this bound requires to build the operation graph for the whole loop body. This is straightforward for inner loops and/or fully unrolled loop nests, but impractical if the loop body contains other loops. We therefore define a weaker, but more practical, bound \emph{that enables composition}:

\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF]
\label{th:minlatunrolled1}
Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^{'}$ the loop body obtained by replicating $UF$ times the original loop body $L$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^{L^{'}}
$$    
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatunrolled1}]
By construction and Theorem~\ref{th:latlbresources}, $Lat_{R_{op}}^{L^{'}}$ is a lower bound on the latency of $L^{'}$, that is the sub-program made of $UF$ iterations of the loop. $\lfloor TC/UF \rfloor \le TC_l/UF$ is a lower bound on the number of iterations of the loop. As we assume a non-pipelined execution for the resulting outer loop, every iteration shall start after the completion of the preceding one, that is its iteration latency, itself bounded by $Lat_{R_{op}}^{L^{'}}$.
\end{proof}

% (*@\colorbox{green}{\textcolor{black}{}}@*)
\begin{lstlisting}[label={lst:partial_before_unroll},caption=Example before partial unrolling,escapechar=!]
#pragma ACCEL parallel UF=4
L1: for (i = 0; i < 8; i++)  {
    S0: a[i] = b[i] * c[i];
}
\end{lstlisting}
% \vspace{-0.5cm}

% \begin{tikzpicture}[remember picture,overlay]
% \draw[black,rounded corners]
%   ([shift={(-3pt,2ex)}]pic cs:w) 
%     rectangle 
%   ([shift={(3pt,-0.65ex)}]pic cs:q);
% \end{tikzpicture}

% \begin{tikzpicture}[remember picture,overlay]
% \draw[black,rounded corners]
%   ([shift={(-3pt,2ex)}]pic cs:n) 
%     rectangle 
%   ([shift={(3pt,-0.65ex)}]pic cs:t);
% \end{tikzpicture}

\begin{lstlisting}[label={lst:partial_after_unroll},caption=Example after partial unrolling,escapechar=!]
// explicitly unroll with UF=4
L1: for (i = 0; i < 8; i+=4)  {
    S0: a[i] = b[i] * c[i];
    S1: a[i+1] = b[i+1] * c[i+1];
    S2: a[i+2] = b[i+2] * c[i+2];
    S3: a[i+3] = b[i+3] * c[i+3];
}
\end{lstlisting}
\vspace{.4cm}

% \begin{tikzpicture}[remember picture,overlay]
% \draw[black,rounded corners]
%   ([shift={(-3pt,2ex)}]pic cs:n) 
%     rectangle 
%   ([shift={(3pt,-0.65ex)}]pic cs:t);
% \end{tikzpicture}

% \begin{tikzpicture}[remember picture,overlay]
% \draw[black,rounded corners]
%   ([shift={(-3pt,2ex)}]pic cs:n) 
%     rectangle 
%   ([shift={(3pt,-0.65ex)}]current page.east|-{pic cs:t});
% \end{tikzpicture}

% On the Listing \ref{lst:partial_before_unroll}, $L$ represent the green part which is unroll by a factor 4 and is explicitly unrolled on the listing \ref{lst:partial_after_unroll}, hence the purple code represent the loop body $L^{'}$.


In Listing \ref{lst:partial_before_unroll}, the loop body denoted by $L$ is depicted in the rectangle. The loop L1 is subjected to a partial unrolling with a factor of 4, as specified by the directive \textit{#pragma ACCEL parallel UF=4} hence S0 have to be expanded and replicated four times.
% 
The explicit unrolling of the loop is illustrated in Listing \ref{lst:partial_after_unroll}, where S0, S1, S2 and S3 represent the loop body $L^{'}$ of the Theorem \ref{th:minlatunrolled1}.
% 
The latency of the program in Listing \ref{lst:partial_before_unroll} and \ref{lst:partial_after_unroll} (which are equivalent) is greater or equal to $\lfloor \frac{TC}{UF} \rfloor$, in this case 2, multiply by the latency of the loop body $L^{'}$.

Note this bound requires to build the operation graph for the whole loop body. This is straightforward for inner loops and/or fully unrolled loop nests, but impractical if the loop body contains other loops. We therefore define a weaker, but more practical, bound:

%\FIXME{Need to precise that we use DSA. And cite Feautrier papier for transformation Affine -> DSA}

\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF and complex loop bodies]
\label{th:minlatunrolled2}
Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor * Lat_{R_{op}}^L
$$    
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatunrolled2}]

% Key argument to prove: style of: lat(S1,forloop) >= max(lat(S1),lat(forloop) that is by adding a new instruction we dont reduce the cp length. A counter example is
% \{for i:  a = a+b\};a = 43


% if we consider a CDAG, adding the edge a = 43 gives a shorter path to a than any of the i iteration in the fully unrolled cdag. So we must add conditions such as writes to the same location have to be all executed, in the order of the original code (sensible condition in presence of data dependencies WAW).

% Proof flow:
% 1) Given $OG^{i}$ and $OG^j$ two CDAGs, for a pair of distinct iterations $i,j$ of loop $L$. If $V_O^i \cap V_O^j = \emptyset$, then the graph $OG^{i,j}$ made of the two iterations $i,j$ cannot have a smaller critical path length than $OG^{i}$ and $OG^j$: there is no edge crossing $OG^{i}$ and $OG^j$ in $OG^{i,j}$ since outputs are distincts, therfore $Lat(OG^{i,j} \ge \max(Lat(OG^i),Lat(OG^j))$.

% 2) Suppose now  $V_O^i \cap V_O^j \ne \emptyset$. Then iterations $i$ and $j$ produce at least one output in common. IDEA: DSA. If the program is in dynamic single assignent form, this is a contradiction (DSA: only 1 write per location). Need to adjust defs at start to be in DSA form? Mention automatic conversion from affine to DSA exists (Feautrier, 90s).


Given $OG^i$ and $OG^j$ two CDAGs, for a pair of distinct iterations $i,j$ of loop $l$. 

If $V_O^i \cap V_O^j = \emptyset$, then the graph $OG^{i,j}$ made of the two iterations $i,j$ cannot have a smaller critical path length than $OG^i$ and $OG^j$: there is no edge crossing $OG^i$ and $OG^j$ in $OG^{i,j}$ since outputs are distinct, therefore $Lat(OG^{i,j}) \ge \max(Lat(OG^i),Lat(OG^j))$.

If $V_O^i \cap V_O^j \ne \emptyset$. Then iterations $i$ and $j$ produce at least one output in common. As there is no useless operation, the graph $OG^{i,j}$ made of the two iterations $i,j$ can not be smaller than $OG^i$ or $OG^j$ and hence $Lat(OG^{i,j}) \ge \max(Lat(OG^i),Lat(OG^j))$.

\end{proof}

Consider the scenario of loop $L0$ within Listing \ref{lst:reference_bicg}, which has been unrolled by a factor denoted as $UF \leq TC_{L0}$ where $TC_{L0}$ is the trip count of $L0$. The latency for one iteration of $S0$ is denoted as $Lat^{S0}_{R_{o}} > 0$.
In the absence of pipelining, the lower bound of the latency of this sub-loop body is: $\lfloor TC_{L0} / UF \rfloor \times Lat^{S0}_{R_{o}}$.

% \FIXME{The above theorem covers the composition case of C operator, with children made of loops with a bound and statements. Perhaps worth rewriting the theorem (or a corrollary) to show this composition of children is valid? That would conclude the formulas with the pipelining below.}

Vitis allows to do a reduction with a tree reduction in logarithmic time with the option ``unsafe-math''. 

% \textcolor{red}{TODO: Should we decompose red and // operation ?}

\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF for reduction loop with tree reduction]
\label{th:minlatunrolled3}
Given a reduction loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$, if executed in a non-pipelined fashion and the tree reduction is legal is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^L \times \lfloor \log_2(UF)  \rfloor
$$    
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatunrolled3}]
    
    By definition a reduction loop is a loop with a dependency distance of 1. Hence, at each iteration the same memory cell is read and write. 
Because of the dependency distance of 1, only one element can be added to the same memory cell.
However each data can be adding independently two by two and the result of this independent addition can also be adding two by two until we obtained one value. Hence the reduction can be done in $\log_2(UF)$ iterations with a tree reduction.
As the depth of the tree is $\log_2(UF)$ and each node at the same depth can be executed independently in $Lat_{R_{op}}^L$ cycles, the straight line code has a latency greater or equal to $Lat_{R_{op}}^L \times \lfloor \log_2(UF)  \rfloor$. And then similarly to Th. \ref{th:minlatunrolled2} and \ref{th:minlatunrolled3} the sequential execution of the loops without pragma repeat this process $\lfloor TC/UF \rfloor$ times.
    
\end{proof}

\begin{lstlisting}[label={lst:tree_red},caption={
Example of code demonstrating a reduction, where a tree reduction technique can be applied, as depicted in Figure \ref{fig:tree_diagram}.}]
L1: for (i = 0; i < 8; i++)  {
    c += a[i];
}
\end{lstlisting}
\vspace{.5cm}


\begin{figure}
    \centering
    \rotatebox{180}{%
\begin{forest}
[\rotatebox{180}{c}, for tree={circle, draw, minimum size=2em, edge={<-}}
  [+, for tree={circle, draw, minimum size=2em, edge={<-}}
    [+, for tree={circle, draw, minimum size=2em, edge={<-}}
        [+, for tree={circle, draw, minimum size=2em, edge={<-}}
            [{\rotatebox{180}{$A[7]$}}]
            [{\rotatebox{180}{$A[6]$}}]
        ]
        [+, for tree={circle, draw, minimum size=2em, edge={<-}}
            [{\rotatebox{180}{$A[5]$}}]
            [{\rotatebox{180}{$A[4]$}}]
        ]
    ]
    [+, for tree={circle, draw, minimum size=2em, edge={<-}}
        [+, for tree={circle, draw, minimum size=2em, edge={<-}}
            [{\rotatebox{180}{$A[3]$}}]
            [{\rotatebox{180}{$A[2]$}}]
        ]
        [+, for tree={circle, draw, minimum size=2em, edge={<-}}
            [{\rotatebox{180}{$A[1]$}}]
            [{\rotatebox{180}{$A[0]$}}]
        ]
    ]
  ]
]
% [\rotatebox{180}{c}, for tree={circle, draw, minimum size=2em, edge={<-}}
%   [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%     [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%       [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[7]]
%               [B[7]]
%               [,phantom]
%               [tmp7, name=tmp7]
%             ]
%         ]
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[1]]
%               [B[1]]
%             ]
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[0]]
%               [B[0]]
%             ]
%         ]
%       ]
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[7]]
%               [B[7]]
%               [,phantom]
%               [tmp7, name=tmp7]
%             ]
%         ]
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[1]]
%               [B[1]]
%             ]
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[0]]
%               [B[0]]
%             ]
%         ]
      
%     ]
%   ]
% ]
  % \node[above=1cm, align=center, font=\bfseries] at (!r.north) {Computation Tree};
  % \draw[->, dashed] (tmp) -- (C);
  % \draw[->, dashed] (tmp) -- (C);
  % \draw[->, dashed] (tmp) -- (C);
\end{forest}
}

    \caption{Illustrating the concurrent execution depicted in Listing \ref{lst:tree_red} through a tree reduction method, accomplished within logarithmic time.}
    \label{fig:tree_diagram}
\end{figure}


Figure \ref{fig:tree_diagram} represent the tree reduction of the Listing \ref{lst:tree_red}. Due to the reduction, we use a tree reduction in order to increase the parallelism of the reduction, and execute a loop of trip count $n=8$ in $\log_2(n)=3$ iterations.

% \begin{forest}
%   % [*, for tree={circle, draw, minimum size=2em, edge={->}}
%   %   [a[0]]
%   %   [b[0]]
%   % ]
%   [ , for tree={}
%     [*, for tree={circle, draw, minimum size=2em, edge={->}}
%       [a[0]]
%       [b[0]]
%     ]
%     [+, for tree={circle, draw, minimum size=2em, edge={->}}
%       [*, for tree={circle, draw, minimum size=2em, edge={->}}
%         [a[1]]
%         [b[1]]
%       ]
%       [+, for tree={circle, draw, minimum size=2em, edge={->}}
%         [$\ldots$]
%         [+, for tree={circle, draw, minimum size=2em, edge={->}}
%           [a[7]]
%           [b[7]]
%         ]
%       ]
%     ]
%   ]

% \end{forest}

\subsubsection{Loop pipelining} 

% Loop pipelining amounts to overlapping multiple iterations of the loop, so that the next iteration can start prior to the completion of the preceding one. The initiation interval (II) measures in cycles the delay between the start of two consecutive iterations. 

Loop pipelining amounts to overlapping multiple iterations of the loop, so that the next iteration can start prior to the completion of the preceding one. The initiation interval (II) measures in cycles the delay between the start of two consecutive iterations. It is easy to prove our formula template accurately integrates the latency of pipelined loops with the $I$ operator.
% 
We compute the minimal II in function of the dependencies of the pipelined loop and the iteration latency of the operations of the statements during the NLP generation. 
Let $RecMII$ and $ResMII$ be the recurrence constraints and the resource constraints of the pipelined loop, respectively. We have $II \geq \max{(ResMII, RecMII)}$. 
% 
$RecMII = \max_i \lceil \frac{ delay(c_i)}{ distance(c_i)} \rceil$ with $delay(c_i)$ the total latency in dependency cycle $c_i$ and $distance(c_i)$ the total distance in dependency cycle $c_i$.
% As we cannot compute accurately $ResMII$ as we don't know how the resource will be used by the compiler 
We suppose that $ResMII=1$, as we do not know how the resource will be used by the compiler.
% 
Hence, if the loop is a reduction loop then the $II \geq \frac{IL_{reduction}}{1}$ with $IL_{reduction}$ the iteration latency of the operation of reduction. For a kernel like the Listing \ref{lst:ex_II}
% $for (j = 0; j < N; j++) y[j] = y[j-2] + 3;$ 
the $II \geq \lceil \frac{IL_+}{2} \rceil$.

\begin{lstlisting}[label={lst:ex_II},caption={Demonstration of a code snippet showcasing a scenario where a loop pipelined with a dependency of distance 2 results in an initiation interval ($II$) that satisfies $II \geq \lceil \frac{IL_+}{2} \rceil$. }]
for (j = 0; j < N; j++) 
    y[j] = y[j-2] + 3;
\end{lstlisting}
\vspace{1cm}

It follows a bound on the minimal latency of a pipelined loop:
\begin{theorem}[Minimal latency of a pipelined loop with known II]
\label{th:minlatpipeline}
Given a loop $l$ with trip count $TC_l$ and loop body $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$ if executed in a pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,P} \ge Lat_{R_{op}}^L + II *( TC_l - 1)
$$    
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatpipeline}]
$Lat_{R_{op}}^L$ is the minimal latency to complete one iteration of $l$ by Theorem~\ref{th:latlbresources}. The initiation interval measures the number of elapsed cycles before the next iteration can start, it takes therefore at least $TC_l * II - 1$ to start $TC_l - 1$ iterations, irrespective of their completion time. Therefore the latency of the loop is at least the latency of one iteration to complete, and for all iterations to be started.
\end{proof}



\subsubsection{Loop pipelining and unrolling}

A loop $l$ with trip count $TC_l$ can be pipelined and partially unrolled with $UF < TC_l$, in this case there is loop splitting where the trip count of the innermost loop equal to the unroll factor and the trip count of the outermost loop equal to $\frac{TC_l}{UF}$.



\begin{theorem}[Minimal latency of a pipelined loop with known II and partially unrolled]
\label{th:minlatpipeline_unrolled}
Given a loop $l$ with trip count $TC_l$, partially unrolled by an unroll factor $UF < TC_l$ and a loop body $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^{'}$ the loop body obtained by replicating UF times the original loop body $L$.
Then the minimal latency of $l$ if executed in a pipelined fashion is bounded by:

$$
Lat_{R_{op}}^{l,P} \ge Lat_{R_{op}}^{L^{'}} 
+ II * ( \frac{TC_l}{UF} - 1)
$$    
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatpipeline_unrolled}]

By construction and Theorem \ref{th:minlatflattenednest} the latency $Lat_{R_{op}}^{L^{'}}$ is a lower bound of $L^{'}$. As the loop was split due to the partial unrolling, the trip count of the pipelined loop is $\frac{TC_l}{UF}$. Theorem \ref{th:minlatpipeline} gives us the lower bound of the latency for a loop with a trip count equal to $\frac{TC_l}{UF}$.

\end{proof}

\subsubsection{Non-Parallel, Non-Pipelined Loops}

We continue with a trivial case: if the loop is not optimized by any directive (including any automatically inserted by the compilers), i.e., not parallelized nor pipelined, then every next iteration of the loop starts only after the end of the prior iteration.

\begin{definition}[Lower bound on latency of a non-parallel, non-pipelined loop under resources constraints]
\label{def:loopIteratedSequentially}
Given a loop $l$ with trip count $TC_l$ which is neither pipelined nor parallelized, that is, iteration $i+1$ starts after the full completion of iteration $i$, for all iterations. Given $Lat_{R_{op}}^L$ the minimal latency of its loop body. Then
$$
Lat_{R_{op}}^l \ge TC_l * Lat_{R_{op}}^L
$$

\end{definition}

\subsubsection{Coarse-Grained parallelization}

Coarse-grained parallelization is a performance enhancement technique involving the unrolling of a loop which iterates a loop body not fully unrolled i.e., containing at least a pipelined loop or a loop executed sequentially. It is therefore impossible to do a coarse-grained parallelization with a reduction loop because the $n$ sub loop body are dependent on each other.


It follows a bound on the minimal latency of a coarse-grained unrolled loop:
\begin{theorem}[Minimal latency of coarse-grained unrolled loop]
\label{th:coarse_grained}

Given a loop $l$, which is not a reduction loop, with trip count $TC_l$, an unroll factor $UF \le TC_l$ and  $L$ the loop body iterated by the loop $l$ with a latency lower bound $Lat^{L}_{R_{op}}$. 
Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^{'}$ the loop body obtained by replicating $UF$ times the original loop body $L$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^{L^{'}}
$$
\end{theorem}

\begin{proof}[Proof Th \ref{th:coarse_grained}]


By construction, Definition \ref{def:loopIteratedSequentially}, Theorem \ref{th:minlatpipeline} and definition of the loop body $L$, $Lat^{L}_{R_{op}}$ is a lower bound of the loop body $L$. As the loop is not a reduction loop there is no dependency between the loop bodies of $L$ for different iteration of $l$ and then the loop bodies can be executed in parallel. 
If $UF < TC_l$, then $\lfloor TC_l/UF \rfloor \leq TC_l / UF $ is a lower bound on the number of iterations of the loop. As we assume a non-pipelined execution for the resulting outer loop, every iteration shall start after the
completion of the preceding one, that is its iteration latency, itself bounded by 
$ Lat_{R_{op}}^{L^{'}} $.

\end{proof}

% \paragraph*{Latency under resource constraint} 

% \FIXME{Statement not define for the following th}

% \begin{theorem}[Minimal resource consumption]
% \label{th:minresource}
% Given a loop body $L$, available resources $R_{op}$ and configuration of pragma $C$. 

% On the condition that the resources are only used by the operations of the different statements
% the minimal number of resource (DSPs) consumed by $L$ for the configuration $C$ is:
% % $$
% % R_{op} < \sum_{op} \max_{t}( \#L_{op}^t) \times DSP_{op} 
% % $$    

% $$
% R_{op} < \sum_{op} \max_{S \in \mathcal{S}_{par}}( \min(1,\#L_{op}^{S}) \times DSP_{op} \times UF^{S})
% $$    

% % with $\#L_{op}^t$ the number of operation $op$ in parallel at time $t$ and $DSP_{op}$ the number of resource (DSPs) used for the operation $op$.

% with $\#L_{op}^t$ the number of operation $op$ in parallel for the statements $S$ which are under the same loop unrolled, $DSP_{op}$ the number of resource (DSPs) used for the operation $op$ and $\mathcal{S}_{par}$ the set of set statements which are under the same unrolled loop.

% \end{theorem}

% \begin{proof}
    
% Here we suppose a perfect reuse intra and inter statement, which means if a computational unit is not used at time $t$, it can be reuse.

% Suppose the formula is wrong, i.e. at time $t$, we can use less resource and hence globally consume less resource. 

% % In this case, we can reuse a computational unit
% 1. If at time $t$ no resource has been used until now, we are oblige to used the number of computational unit necessary for the operations in parallel.

% 2. If at time $t$ we can reuse all the resource, then the number of resource used at time $t$ are less or equal to the resource already used

% 3. If at time $t$ the number of computational unit necessary for the computation is greater than the number of available resource already used and available. Then we reuse the maximum of resource unused plus the difference of new resource needed to do the computation. We can differentiate three possible cases:
%     3.1 If two statements are under the same unrolled loop then we only count one computation unit per operation for all the statements under the loop(s) unrolled.
%     3.2 If two statements are not under the same unrolled loop, then when the second statement will be run all resource consumed by the first statement will be free and hence can be reused.
%     3.3 If a loop is pipelined and the II is not as expected we still have the minimum of DSP used because of reuse intra-statement i.e. the minimal number of DSP will be independant of the II.

% In all case, the number of DSP is minimal.




% % Plus complique que ca il faut dire que y'a un reuse intra statement
% %  mais qu'on suppose qu'il est utilisé que 1 fois par chaque statement
% % du coup faut reecrire la formule
% % 
% % 
    
% \end{proof}

% \begin{theorem}[Maximal resource consumption]
% \label{th:maxresource}
% Given a loop body $L$, available resources $R_{op}$ and configuration $C$. 
% On the condition that the resources are only used by the operations of the different statements
% the maximum number of resource (DSPs) consumed by $L$ is:
% $$
% R_{op} \ge \sum_{S \in \mathcal{S}} \sum_{op}\max_{t}( \#L_{op}^{S,t}) \times DSP_{op} 
% $$    
% with $\#L_{op}^t$ the number of operation $op$ in parallel at time $t$ and $\mathcal{S}$ the set of statements.

% \end{theorem}

% \begin{proof}
% % est ce que c'est pas se compliquer la vie ?

% Here we suppose we don't have reuse inter and intra-statement. Hence, if one statement need to do two additions, the two additions will used different computational unit and these computational units will not be used for other statement.

% As we sum all the resource used per operation per statement we have to prove that 1. The same operation for the same statement can't used more resource than $DSP_{op}$. And we have as hypothesis than the operation $op$ used $DSP_{op}$.

% 2. If more parallelism the number of DSP will be greater. However, we know the configuration as input and hence know the parallelism of the kernel.



% % Problem if UF does not divide TC  => False Problem because if Merlin transform we know the code

    
% \end{proof}

% \begin{theorem}[Latency under resource constraint]
% \label{th:minlatpipeline}
% Given a loop body $L$, available resources $R_{op}$, lower bound without constraint $lb$ and configuration $C$. 

% The lower bound $lb$ can not be achieve under resource constraint if 
% $$
% R_{op} < \sum_{op} \max_{S \in \mathcal{S}_{par}}( \min(1,\#L_{op}^{S}) \times DSP_{op} \times UF^{S})
% $$    
% with $\#L_{op}^t$ the number of operation $op$ in parallel for the statements $S$ which are under the same loop unrolled, $DSP_{op}$ the number of resource (DSPs) used for the operation $op$ and $\mathcal{S}_{par}$ the set of set statements which are under the same unrolled loop.

% The lower bound $lb$ can be achieve under resource constraint if 
% $$
% R_{op} \ge \sum_{S \in \mathcal{S}} \sum_{op}\max_{t}( \#L_{op}^{S,t}) \times DSP_{op} 
% $$    
% with $\mathcal{S}$ the set of statements.
% \end{theorem}

% \begin{proof}
% We compute the resource used for two cases:

% \begin{itemize}
%     \item Perfect Reuse, which is intra and inter statement. If a resource is not use at time $t$, then it can be reuse for the same operation.
%     \item No reuse, i.e. each statement use different resource.
% \end{itemize}


% In the first case (perfect reuse), it is impossible to consume less resource, as proof in Theorem \ref{th:minresource}. In the second case, it is impossible to consume more resource, as proof in Theorem \ref{th:maxresource}. Hence, if a loop body $L$ 
% has a minimum of resource comsumption greater than resource available
% the loop body can not be synthesized and run on this board. Hence the lower bound can not be achieve.

% In other way if a loop body $L$, has a maximal amount of resource lesser than resource available the design can be synthetized and run on this board. The lower bound can be achieve.

% If in practice at least one pragma is not applied as expected, then we have an other configuration with it is own lower bound.

% % If the hypothesis of reuse is wrong hence the resource consumed is greater than the one computed and the resource used are greater than resource available.
% \end{proof}

\subsubsection{Program latency lower bound under resource constraints} 

We now focus on the latency lower bound of a program, under resource constraints. This bound takes into account the limitations imposed by available resources, which can significantly affect the achievable performance.
% 
We assume here that the resources consumed are only consumed by the computing units and resource use by the computational unit of one operation can not be reused by the computational unit of another operation executing at the same time. We also assume that the compilers have implemented the pragma configuration given as input.


For DSPs we suppose we have a perfect reuse i.e., that the computation units for the same operation can be reused as soon as the computation unit is not in use. Under-estimating the resources used is fundamental to proving the latency lower bound, as otherwise another design that consumes less resources than predicted may be feasible, itself possibly leading to a better latency. 


% \begin{theorem}
% \label{th:minres}
%     Given a loop body $L$,  the set of statements $\mathcal{S}$,
% $\#L_{op}^s$ the number of operations $op$  for the statements $s$, $DSP_{op}$ the number of resources (DSPs) used for the operation $op$, $MCU_{op}^s$ the maximal number of computational units the statement $s$ can use in parallel at any given time,  and  the configuration of pragma $\vec{PV_i}$ for each loop.
% The minimal number of resource (DSPs) consumed, $R_{used}^{min}$, by $L$ for the pragma configuration  is the sum, for each operation, of the maximum number of DSPs used in parallel by a statement.
% This corresponds to:
% $$R^{min}_{used} =  \sum_{op} \max_{s \in \mathcal{S}}(
% \#L_{op}^s
% \times DSP_{op} 
% \times MCU_{op}^{s})$$
% \end{theorem}

% \begin{proof}[Proof Th \ref{th:minres}]
%     Considering perfect resource reuse, where all unused computational units can be reused, and assuming that the compilers have implemented the pragma configuration provided as input. 
% For each statement $s$, the maximum number of computational units used in parallel is determined. This means that each statement $s$ requires at least $\#L_{op}^s \times DSP_{op} \times MCU_{op}^s$ DSPs. By considering the maximum across all statements, we can guarantee that at least one statement will require $\max_{s \in \mathcal{S}}(\#L_{op} \times DSP_{op} \times MCU_{op}^s)$ DSPs.
% Since there is no possibility of resource reuse between different operations, the summation of the resource consumed for each operation remains the minimum consumption of resources. In other words, the sum of the individual resource consumption for each operation represents the minimum amount of resources required.
% \end{proof}

\begin{theorem}
\label{th:minres}
    Given a loop body $L$,  the set of set of  statements $\mathcal{S}_{seq}$ non executed in parallel, 
$\#L_{op}^s$ the number of operations $op$  for the statements $s$, $DSP_{op}$ the number of resources (DSPs) used for the operation $op$, $MCU_{op}^s$ the maximal number of computational units the statement $s$ can use in parallel at any given time,  and  the configuration of pragma $\vec{PV_i}$ for each loop.
The minimal number of resource (DSPs) consumed, $R_{used}^{min}$, by $L$ for the pragma configuration  is the sum, for each operation, of the maximum number of DSPs used in parallel by a statement.
This corresponds to:
$$R^{min}_{used} =  \sum_{op} \max_{\mathcal{S} \in \mathcal{S}_{seq}}( \sum_{s \in \mathcal{S}}
\#L_{op}^s
\times DSP_{op} 
\times MCU_{op}^{s})$$
\end{theorem}

\begin{proof}[Proof Th \ref{th:minres}]
    Considering perfect resource reuse, where all unused computational units can be reused, and assuming that the compilers have implemented the pragma configuration provided as input. 
For each statement $s$, the maximum number of computational units used in parallel is determined. This means that each statement $s$ requires at least $\#L_{op}^s \times DSP_{op} \times MCU_{op}^s$ DSPs. 
If a set of statements $\mathcal{S}$ are executed in parallel they cannot share the resource so the execution in parallel of the statement $s \in \mathcal{S}$ will require $( \sum_{s \in \mathcal{S}}
\#L_{op}^s
\times DSP_{op} 
\times MCU_{op}^{s})$ DSPs.
% 
By considering the maximum across all statements, we can guarantee that at least one set of statement executed in parallel will require $\max_{s \in \mathcal{S}_{seq}}(\sum_{s \in \mathcal{S}} \#L_{op} \times DSP_{op} \times MCU_{op}^s)$ DSPs.
Since there is no possibility of resource reuse between different operations, the summation of the resource consumed for each operation remains the minimum consumption of resources. In other words, the sum of the individual resource consumption for each operation represents the minimum amount of resources required.
\end{proof}


Given a program and the available resource of DSP $DSP_{avail}$, if $R^{min}_{used} < DSP_{avail}$ the lower bound is valid and the program does not over-utilize the resources. 

%%% LNP: I cannot parse this sentence.
%The latency lower bound of a kernel is therefore the latency lower bound of the configuration such that the minimal resource consumption is less than or equal to the resource available.

% \begin{theorem}[Latency Lower bound of a program]
% \label{th:minlatpipelineunderresourceconstraint}
% % Given a kernel, available resource $R_{op}$, the set of statements $\mathcal{S}$ and all the configuration of pragmas which are constitute of  the vectors $\Vec{PV_i}$ for each loop.
% Given a loop body $L$,  the set of statements $\mathcal{S}$,
% $\#L_{op}^s$ the number of operation $op$  for the statements $s$, $DSP_{op}$ the number of resources (DSPs) used for the operation $op$, $MCU_{op}^{s}$ the maximal number of computational unit the statement $s$ can use in parallel, and  the configuration of pragma  $\Vec{PV_i}$ for each loop.

% The configuration of pragma, which has the minimal lower bound and which respect $R_{used}^{min} = \sum_{op} \max_{s \in \mathcal{S}}(
% \#L_{op}^s
% \times DSP_{op} 
% \times MCU_{op}^{s}) \leq R_{op}$, is the lower bound of the kernel.


% \end{theorem}


% \begin{proof}[Proof Th \ref{th:minlatpipelineunderresourceconstraint}]

%     According to Theorem \ref{th:minres}, $R_{used}^{min}$ is the minimal number of DSP a configuration can use. Hence, all configuration which does not respect the constraint $R_{used}^{min}\leq R_{op}$ have a over-utilization of the resource and hence are invalid.

%     Hence, the minimal lower bound of each configuration of pragma is the lower bound of the kernel.
    
% \end{proof}

%   

\subsubsection{Memory transfer}

AMD/Xilinx Merlin manages automatically the memory transfer. The memory transfer and computation are not overlap (no dataflow) hence the latency is the sum of the latency of computation and communication. We assume that for each array the contents of the array are in the same DRAM bank.

\begin{theorem}[Lower bound of the memory transfer latency for an array]
\label{th:memlatonearray}

Given a loop body $L$,  the set of array $\mathcal{A}$,  an array $a \in \mathcal{A}$, and $LAT^{mem}_a$ the latency to transfer the array $a$ from off-chip to on-chip (inputs) and from on-chip to off-chip (outputs).
$\forall a \in \mathcal{A}, LAT^{mem}_a \geq 
(\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$.
With $\mathds{1}_{cond} = 1$ if $cond$ = true else 0.

\end{theorem}

\begin{proof}[Proof Th \ref{th:memlatonearray}]
    In order to transfer all the elements of the array $a$ we can use packing with a maximum packing allowed by the target device of $max\_burst\_size$, which means in practice the real burst size will be equal or less than $max\_burst\_size$.
    As all the elements of the array $a$ are in the same bank, the transfer is sequential. And as we as suppose all operation including memory transfers are done in at least one cycle, the minimum latency is $footprint_a / max\_burst\_size$ to transfer once the array $a$. As an array can be input, output or both we need to add the transfer from off-chip to on-chip for inputs i.e., $a \in V_I^L$ and from on-chip to off-chip for the outputs i.e., $a \in V_O^L$.
    
\end{proof}

%%%%%%% TODO: figure with footprint, 512 bits, off-chip and on-chip mem

% \begin{figure}
%     \centering
% \begin{tikzpicture}[
%     node distance=2cm,
%     block/.style={draw, rectangle, align=center, minimum height=1.5cm, minimum width=2.5cm},
%     arrow/.style={-Stealth, thick},
% ]

% % Off-chip memory
% \node[block, fill=blue!20] (offchip) {Off-chip\\Memory};
% \draw[<->, thick] ([yshift=-0.5cm]offchip.south west) -- ([yshift=-0.5cm]offchip.south east) node[midway, below] {512 bits};

% % On-chip memory
% \node[block, right=of offchip, fill=green!20] (onchip) {On-chip\\Memory};

% % Arrow indicating data transfer
% \draw[arrow] (offchip.east) -- (onchip.west) node[midway, above] {Transfer};

% % Footprint of off-chip memory
% \draw[dashed, thick, draw=red] ([xshift=-0.5cm]offchip.north west) rectangle ([xshift=0.5cm]offchip.south east) node[midway, right=1cm] {Footprint};

% \end{tikzpicture}
% \caption{Memeory transfer from off-chip to on-chip}
%     \label{fig:mem_trans}
% \end{figure}


\begin{theorem}[Lower bound of the memory transfer latency]
\label{th:memlat}

Given a loop body $L$,  the set of array $\mathcal{A}$, the number of cycles to transfer  the array $a$ is bounded by $\max_{a \in \mathcal{A}} (\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$.

\end{theorem}

\begin{proof}[Proof Th \ref{th:memlat}]
According to Th. \ref{th:memlatonearray} the lower bound to transfer one array $a$ is $(\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$. As the array can be on different DRAM banks the transfer from off-chip to on-chip can be done in parallel but at least one array has a latency greater or equal to $(\mathds{1}_{a \in V_O^L} + \mathbb{\in V_I^L}) \times footprint_a / max\_burst\_size$ and hence the memory latency is equal to $\max_{a \in \mathcal{A}} (\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L})  \times footprint_a / burst\_size$. 
\end{proof}

% \begin{theorem}[Lower bound of the memory latency under resource constraint]
% \label{th:memlat_resource}

% TODO mem on chip

% Given a loop body $L$,  the set of array $\mathcal{A}$, the number of cycle to transfer  the array $a$ is bounded by $\max_{a \in \mathcal{A}} (\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$.

% \end{theorem}

% \begin{proof}[Proof Th \ref{th:memlat_resource}]
% According to Th. \ref{th:memlatonearray} the lower bound to transfer one array $a$ is $(\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$. As the array can be on different DRAM banks the transfer from off-chip to on-chip can be done in parallel but at least one array have a latency greater or equal to $(\mathds{1}_{a \in V_O^L} + \mathbb{\in V_I^L}) \times footprint_a / max\_burst\_size$ and hence the memory latency is equal to $\max_{a \in \mathcal{A}} (\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L})  \times footprint_a / burst\_size$. 
% \end{proof}





\subsection{Summary}



By composing all the theorems, this allows us to end up with the final latency lower bound of the program which is presented in theorems \ref{th:comp_lb} for the computation and \ref{th:global_lb} for the computation and communication.




\begin{theorem}[Computation Latency Lower bound of a Program]
\label{th:comp_lb}

Given available resource $DSP_{avail}$ and a program which contains a loop body $L$ which contains by composition a set of loops $\mathcal{L}^{non \; reduction}_{L}$ potentially coarse-grained unrolled with $\forall l \in \mathcal{L}_{L}, UF_l$ and a set of reduction loops executed sequentially $\mathcal{L}^{reduction}_{L}$ which iterates a loop body $L_{pip}$. The loop body $L_{pip}$ contains a pipelined loop $l_{pip}$ which iterate a loop body $L_{fg}$ fully unrolled. The loop body $L_{fg}$ contains operations which can be done in parallel with a latency $Lat_{L_{par}}$ 
and operations which are reduction originally iterated by the loops $\mathcal{L}^{reduction}_{L_{fg}}$ with a latency $Lat_{L_{seq}}$.

The computation latency lower bound of $L$, which respected $DSP^{min}_{ued} \leq DSP_{avail}$, executed with tree reduction is:

$$
Lat_{L} = \prod_{l\in \mathcal{L}^{par}_{L}} \frac{TC_l}{UF_l} \times 
\prod_{l\in \mathcal{L}^{reduction}_{L}} TC_l \times Lat_{L_{pip}}
$$

with 

$Lat_{L_{pip}} = (Lat_{L_{fg}} + II\times (\frac{TC_{l_{pip}}}{l_{pip}\_UF}-1) )$
and 
$Lat_{L_{fg}} = Lat_{L_{par}} +
Lat_{L_{seq}} \times \prod_{l\in \mathcal{L}^{reduction}_{L_{fg}}} \frac{TC_l}{UF_l} \times \log_2(UF_l)   $.

\end{theorem}


\begin{proof}[Proof Th \ref{th:comp_lb}]

% By composition and Theorems \ref{th:minlatunrolled1} and \ref{th:minlatunrolled2}, $Lat_{L_{fg}}$ is a lower bound of the fully unrolled sub-loop body of $L$, $L_{fg}$.

% By composition and Theorems \ref{th:minlatpipeline} and \ref{th:minlatpipeline_unrolled}, $Lat_{L_{pip}}$ is a lower bound of $L_{pip}$.

% By composition, Theorem \ref{th:coarse_grained} and Definition \ref{def:loopIteratedSequentially}, $Lat_{L}$ is a lower bound of $L$.

Through composition and the application of Theorems \ref{th:minlatunrolled1} and \ref{th:minlatunrolled2}, $Lat_{L_{fg}}$ serves as a computation latency lower bound for the fully unrolled sub-loop body of $L$, denoted as $L_{fg}$.

By employing composition alongside Theorems \ref{th:minlatpipeline} and \ref{th:minlatpipeline_unrolled}, $Lat_{L_{pip}}$ stands as a computation latency lower bound for $L_{pip}$.

Utilizing composition, Theorem \ref{th:coarse_grained}, and Definition \ref{def:loopIteratedSequentially}, $Lat_{L}$ emerges as a computation latency lower bound for $L$.

\end{proof}



\begin{theorem}[Latency lower bound of a program optimized with Merlin pragmas]
\label{th:global_lb}

Given available resource $DSP_{avail}$ and a program which contains a loop body $L$ with a computation latency $Lat_{L}^{computation}$ and a communication latency $Lat_{L}^{communication}$.

The lower bound for $L$ which respected $DSP^{min}_{ued} \leq DSP_{avail}$ and where the computation and communication can not be overlap is:

$$
Lat_{L} = Lat_{L}^{computation} + Lat_{L}^{communication}
$$

\end{theorem}


\begin{proof}[Proof Th \ref{th:global_lb}]
The AMD/Xilinx Merlin compiler does not overlap computation and communication. Hence the computation and communication is a sum of the latency of computation and latency of communication.
By composition and Theorems \ref{th:comp_lb} and \ref{th:memlat}.

\end{proof}




==> sources/th_proof_complete.tex <==
\section{Theoretical Latency and Resource Modeling}

% \label{sec:appendix}
\label{appendix:theoretical}



We now outline key elements of our analytical performance model, and the associated proofs this model computes a lower bound on latency under resource constraints. 

% Full proofs cover several pages, and are available in a separate research report: we limit below to summarizing the hypothesis and overall proof approach.




\subsection{Analytical Model Template}
\label{sec:analyticalModelTemplate}


Consider the expression $I^{\vec PV_i}_i(X)$ for the loop $i$, where $X$ denotes a subpart of the program, and the operators are defined as follows:

\[
I^{\vec{PV}_i}_i(X) = \begin{cases} 
      \left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor + X & \text{if loop } i \text{ is pipelined}  \\
      & (\text{ispip}_i = 1) \\ \\
      \left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor \cdot X & \text{otherwise } (\text{ispip}_i = 0)
   \end{cases}
\]

For simplicity, we will represent the operation as $\odot$ to differentiate between the two different cases. 

Let $C_i^{\vec PV_i}(X_1, X_2, \dots, X_n)$ which compose the different sub part of a program under the loop $i$.

\[
C_i^{\vec PV_i}(X_1, X_2, \dots, X_n) = \begin{cases} 
      max(X_1, X_2, \dots, X_n) & \text{ if } (X_1, \dots, X_n) \text{ do not have dependencies (WaR, RaW, WaW)} \\
      % \\
      % & \text{inparallel}_i = 1 = 1 - \text{insequence}_i \\ \\
      \sum_{k=1}^n X_k & \text{otherwise}
   \end{cases}
\]

\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[label={lst:example_dep},caption={Example of code where two statements have dependencies}]
S0: x1 += y;
S1: x2 += x1 + z;
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[label={lst:example_nodep},caption={Example of code where two statements do not have dependency}]
S0: x1 += y;
S1: x2 += z;
\end{lstlisting}
\end{minipage}
\vspace{0.6cm}

% \begin{lstlisting}[label={lst:example_dep},caption={Example of code where two statements have dependencies} ]
% S0:x1 += y;
% S1:x2 += x1 + z;
% \end{lstlisting}
% \vspace{0.5cm}

% \begin{lstlisting}[label={lst:example_nodep},caption={Example of code where two statements do not have dependency} ]
% S0:x1 += y;
% S1:x2 += z;
% \end{lstlisting}
% \vspace{0.5cm}


In List~\ref{lst:example_dep}, statements $S0$ and $S1$ exhibit dependencies, resulting in a program latency equal to the sum of their latencies, corresponding to $issequence=1$. Conversely, the statements in List~\ref{lst:example_nodep} lack dependencies, allowing $S0$ and $S1$ to be executed concurrently. Therefore, the latency is determined by the maximum of $S0$ and $S1$ latencies, representing the case $inparallel=1$.

Finally, $SL^{\vec PV_i}_i(\vec S_k)$ denotes a region of straight-line code (e.g., an inner-loop body). 
% which is used below in the formal reasoning on the bounds on latency of this template formula. 
Intuitively, $SL$ will represent a lower bound on the latency of a code block such that by composition across all loops as per the template formula, the result remains a lower bound on the full program latency. 

Given the summary AST of the program in constructor form, and the set of $\vec PV_i$ vectors for each loop, we build the analytical formula template as follows: 
\begin{enumerate}
    \item replace the $Loop_i(\vec X)$ operator by $I^{\vec PV_i}_i(\vec X)$ operator;
    \item replace the $\vec X$ list by $C^{\vec PV_i}_i(\vec X)$;
    \item replace statement lists inside loop \texttt{i} $\vec S_x$ by $SL^{\vec PV_i}_i(\vec S_x)$.
\end{enumerate}
For our example, we can rewrite the expression:
\[
Loop_i(Loop_{j1}(S1), Loop_{j2}(S2,S3))
\]

as

\[
I^{\vec PV_i}_i(C^{\vec PV_i}(I^{\vec PV_{j1}}_{j1}(SL^{\vec PV_{j1}}_{j1}(S1)), I^{\vec PV_{j2}}_{j2}(SL^{\vec PV_{j2}}_{j2}(S2,S3))))
\]

Upon substituting the definitions and assuming that the statements are independent, we obtain:

\[
% I^{\vec PV_i}_i(
\left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor \odot
    % C^{\vec PV_i}(
    \max \left(
        % I^{\vec PV_{j1}}_{j1}(
        \left\lfloor II_{j1} \cdot \left(\frac{TC^{avg}_{j1}}{uf_{j1}} - \text{ispip}_{j1}\right) \right\rfloor \odot
            SL^{\vec PV_{j1}}_{j1}(S1)
        % ), 
        ,
        % I^{\vec PV_{j2}}_{j2}(
        \left\lfloor II_{j2} \cdot \left(\frac{TC^{avg}_{j2}}{uf_{j2}} - \text{ispip}_{j2}\right) \right\rfloor  \odot
            SL^{\vec PV_{j2}}_{j2}(
                S2,
                S3
            )
        \right)
%     )
% )
\]

% \FIXME{I let you judge but I think it is unreadable for 2mm}

% 2mm on Listing \ref{lst:2mm}  can be represented by: 
% $
% (Loop_{i_1}(Loop_{j_1}(S_0, Loop_{k_1}(S1))) , Loop_{i_2}(Loop_{j_2}(S_2, Loop_{k_2}(S3))))
% $. If we apply the definition of $C^{PV}$ and $I^{PV}$ we have the following equation:

% % I^{\vec PV_{i_1}}_{i_1}
% $
% (
%     I^{\vec PV_{i_1}}_{i_1}(
%         I^{\vec PV_{j_1}}_{j_1}(
%             C_{j_1}^{\vec PV_{j_1}}(
%                 SL^{\vec PV_{j_1}}_{j_1}(S_0), 
%                 I^{\vec PV_{k_1}}_{k_1}(
%                     SL^{\vec PV_{k_1}}_{k_1}(S1)
%                 )
%             )
%         )
%     ) , 
%     I^{\vec PV_{i_2}}_{i_2}(
%         I^{\vec PV_{j_2}}_{j_2}(
%             C_{j_1}^{\vec PV_{j_2}}(
%                 SL^{\vec PV_{j_2}}_{j_2}(S_2), 
%                 I^{\vec PV_{k_2}}_{k_2}(
%                     SL^{\vec PV_{k_2}}_{k_2}(S3)
%                 )
%             )
%         )
%     )
% )
% $
% .

% Upon substituting the definition, we acquire:

% $
% (
%     % I^{\vec PV_{i_1}}_{i_1}(
%     \lfloor II_{i_1} * (TC^{avg}_{i_1} /uf_{i_1} - ispip_{i_1})  \rfloor \odot 
%         % I^{\vec PV_{j_1}}_{j_1}(
%         \lfloor II_{j_1} * (TC^{avg}_{j_1} /uf_{j_1} - ispip_{j_1})  \rfloor \odot 
%             % C_{j_1}^{\vec PV_{j_1}}(
%             sum(
%                 SL^{\vec PV_{j_1}}_{j_1}(S_0), 
%                 % I^{\vec PV_{k_1}}_{k_1}(
%                 \lfloor II_{k_1} * (TC^{avg}_{k_1} /uf_{k_1} - ispip_{k_1})  \rfloor \odot 
%                     SL^{\vec PV_{k_1}}_{k_1}(S1)
%                 )
%             )
%         )
%     ) , 
%     % I^{\vec PV_{i_2}}_{i_2}(
%    \lfloor II_{i_2} * (TC^{avg}_{i_2} /uf_{i_2} - ispip_{i_2})  \rfloor \odot 
%         % I^{\vec PV_{j_2}}_{j_2}(
%         \lfloor II_{j_2} * (TC^{avg}_{j_2} /uf_{j_2} - ispip_{j_2})  \rfloor \odot 
%             % C_{j_1}^{\vec PV_{j_2}}(
%             sum(
%                 SL^{\vec PV_{j_2}}_{j_2}(S_2), 
%                 % I^{\vec PV_{k_2}}_{k_2}(
%                 \lfloor II_{k_2} * (TC^{avg}_{k_2} /uf_{k_2} - ispip_{k_2})  \rfloor \odot 
%                     SL^{\vec PV_{k_2}}_{k_2}(S3)
%                 )
%             )
%         )
%     )
% )
% $.




\subsection{A Formal Model for Latency}

Our objective is to formulate a lower bound on the latency of a program after HLS. We therefore have put several restrictions: we assume the input program is a polyhedral program, that is the control-flow is statically analyzable; all loops can be recognized and their trip count computed; and all array / memory accesses can be exactly modeled at compile-time. No conditional can occur in the program. While our approach may generalize beyond this class, we limit here to these strict assumptions.

To maintain a lower bound on latency by composition, we operate on a representation of (parts of the) program which is both schedule-independent and storage-independent: indeed, a lower bound on this representation is necessarily valid under any schedule and storage eventually implemented. \emph{We however require HLS to not change the count and type of operations}. Furthermore, for lower bounding purposes, we assume unless stated otherwise $\forall i,~inparallel_i = 1$. We will discuss in the next section a more realistic but compiler-dependent approach to set $inparallel_i$, based on dependence analysis.

We assume programs are made of affine loops, that are loops with statically computable control-flow, with loop bounds made only of intersection of affine expressions of surrounding loop iterators and program constants. We now assume loop bodies (i.e., statements surrounded by loops) have been translated to a list of statements, with at most a single operation (e.g., \texttt{+,-,/,*}) per statement. Operations are n-ary, that is they take $n \ge 0$ input scalar values as operand, and produce 0 or 1 output scalar value. A memory location can be loaded from (resp. stored to) an address stored in a scalar variable. This is often referred to as straight-line code
% \cite{some-good-def}
. 
This normalization of the loop body facilitates the computation of live-in/live-out data for the code block, and the extraction of the computation graph. Note the region can be represented in Static Single Assignment 
% \cite{ssa} 
form, to ensure different storage location for every assignment, facilitating the construction of the operation graph.
% 
In addition we require the input program to not contain useless operations which may be removed by the HLS toolchain e.g. by dead code elimination, as illustrated in Listing~\ref{lst:dead-code}.


\begin{lstlisting}[caption={Example of Code Illustrating Dead Code Elimination: As Statement S1 writes to variable x, but the value of x assigned in Statement S0 is never used, the compiler will remove Statement S0.},label={lst:dead-code}]
int example(int y, int z){
    int x;
    S0: x = 12 + y; //  dead-code elimination
    S1: x = y + z;
    return x;
}
\end{lstlisting}
\vspace{0.7cm}


The restriction can be summarized as:

\begin{itemize}[leftmargin=*]
    \item The input program is a pure polyhedral program \cite{girbal06ijpp}, and its analysis (loop trip counts for every loop, all data dependences \cite{Fea92b}) is exact.
    \item No HLS optimization shall change the number of operations in the computation: strength reduction, common sub-expression elimination, etc. shall either first be performed in the input program before analysis, or not be performed by the HLS toolchain. The program also does not contain "useless" operations that may be removed by the compiler.
    \item We only model DSP and BRAM resources for the considered kernel, ignoring all other resources. We do not model LUT and FF resources, because from experience in the loop-based benchmarks we consider DSP and BRAM resources are the most constraining resources. Moreover, the estimation of LUTs and FFs is more tedious.
    \item We assume resource (DSP) sharing across different operations executing at the same cycle is not possible.
\end{itemize}

An important term is $SL$, a latency lower bound for a region of straight-line code. To maintain a lower bound on latency by composition, we operate on a representation of (parts of the) program which is both schedule-independent and storage-independent: the operation graph, or CDAG \cite{elango2015characterizing}. Indeed, a lower bound on this representation is necessarily valid under any schedule and storage eventually implemented and can be used to prove I/O lower bounds on programs \cite{elango2015characterizing} which is the directed acyclic graph with one node per operation in the code region, connecting all producer and consumer operations to build the operation graph. Then, we can easily compute the length of its critical path, which represents the minimal set of operations to execute serially.

% Then, we can build a lower bound on the number of cycles a region $L$ may require to execute, under fixed resources, by simply taking the maximum between the weighted critical path and the work to execute normalized by the resources available.

\begin{definition}[Straight-line code]
\label{def:straightlinecode}
An n-ary operation takes n scalar operands $\vec i$ as input, and produces a single scalar $o$ as output. A statement contains a single n-ary operation, or a load from (resp. store to) a memory location to (resp. from) a scalar. A straight-line code region $L$ is a list of consecutive statements, with a single entry and single exit.
\end{definition}

\begin{definition}[Live-in set] The live-in set $V_I^L$ of region $L$ is the set of scalar values, variables and memory locations that read before being written, under any possible valid execution of $L$.
\end{definition}

\begin{definition}[Live-out set] The live-out set $V_O^L$ of region $L$ is the set of variables and memory locations that written to during any possible valid execution of $L$.
\end{definition}

%%% LNP: I think it's not useful for the reader.
%On the listing \ref{lst:dead-code}, $V_O^L = \{x\}$ and $V_I^L = \{y, z\}$. 
%On the listing \ref{lst:2mm}, let be $L$ the region of the first loop body,
%$V_O^{L} = \{tmp[i_1][j_1], \forall i_1,j_1 \text{ s.t. } 0 \leq i_1 \leq 180 \And 0 \leq j_1 \leq 190  \}$ and $V_I^{L} = \{B[k_1][j_1], \forall k_1,j_1 \text{ s.t. } 0 \leq k_1 \leq 210 \And 0 \leq j_1 \leq 190  \} \cup \{A[i_1][k_1], \forall i_1,k_1 \text{ s.t. } 0 \leq i_1 \leq 180 \And 0 \leq k_1 \leq 210  \} \cup \{alpha\}$. 

We can compute the directed acyclic graph made of all statements (i.e., all n-ary operations), connecting all producer and consumer operations, to build the operation graph: % 
% \cite{someothergoodref}:

\begin{definition}[Operation Graph] 
\label{def:computationgraph}
Given a straight-line code region $R$ made of a list $L$ of statements $S \in L$, the operation graph OG is the directed graph $<\{N,V_I,root,V_O\},E>$ such that $\forall S_i \in L,~N_{S_i} \in N$; and for every operation with output $o$ and inputs $\vec i$ in $L$ $\forall S_i, \forall i_k \in \Vec{i}_{S_i}, e_{i_k, o} \in E$,
$\forall S_i:(o_{S_i},{\vec i}_{S_i}) \in L, S_j:(o_{S_j},{\vec i}_{S_j}) \in L$ with $S_i \ne S_j$ then we have $E_{S_i,S_j} \in E$ iff $o_{Si}\cap{\vec i}_{S_j}\ne \emptyset$. For every input (resp. output) in $S_i$ which is not matched with an output (resp. input) of another $S_j$ in $L$, create a node $V_{val} \in V_I$ (resp. $V_O$) for this input (resp. output) value. If $dim({\vec i}_{S_i}) = 0$ then an edge $e_{root,S_i}$ is added to $E$.
\end{definition}

% \begin{lstlisting}[caption={Example},label={lst:og}]
% A[0] = B[0] + C[0];
% A[1] = B[1] + C[1];
% D[0] = E[0] + A[0];
% D[1] = E[1] + A[1];
% \end{lstlisting}
% \vspace{0.7cm}

% \begin{figure}[htb]
%     \centering
%     \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=1.5cm,semithick]
%     % \begin{tikzpicture}[>=Stealth, auto, shorten >=1pt, semithick, rounded corners]

%         % Nodes
%         \node[draw, circle] (Root) {root};
%         \node[coordinate, below=of Root] (FakeNode) {};
%         \node[draw, circle, left=of FakeNode] (B0) {B[0]};
%         \node[draw, circle, right=of FakeNode] (B1) {B[1]};
%         \node[draw, circle, left=of B0] (C0) {C[0]};
%         \node[draw, circle, right=of B1] (C1) {C[1]};
%         \node[draw, circle, below=of B0] (A0) {A[0]};
%         \node[draw, circle, below=of B1] (A1) {A[1]};
%         \node[draw, circle, below=of A0] (D0) {D[0]};
%         \node[draw, circle, below=of A1] (D1) {D[1]};
%         \node[draw, circle, left=of C0] (E0) {E[0]};
%         \node[draw, circle, right=of C1] (E1) {E[1]};
%         % \node[draw, circle, below=of Root] (A0) {A[0]};
%         % \node[draw, circle, below=of Root] (A1) {A[1]};
%         % \node[draw, circle, below=of Root] (B0) {B[0]};
%         % \node[draw, circle, below=of Root] (B1) {B[1]};
%         % \node[draw, circle, below=of Root] (C0) {C[0]};
%         % \node[draw, circle, below=of Root] (C1) {C[1]};
%         % \node[draw, circle, below=of Root] (D0) {D[0]};
%         % \node[draw, circle, below=of Root] (D1) {D[1]};
%         % \node[draw, circle, below=of Root] (E0) {E[0]};
%         % \node[draw, circle, below=of Root] (E1) {E[1]};



        

%         % Edges
%         \draw[->] (Root) -- (B0);
%         \draw[->] (Root) -- (B1);
%         \draw[->] (Root) -- (C0);
%         \draw[->] (Root) -- (C1);
%         \draw[->] (Root) -- (E0);
%         \draw[->] (Root) -- (E1);

%         \draw[->] (B0) -- (A0);
%         \draw[->] (C0) -- (A0);
%         \draw[->] (B1) -- (A1);
%         \draw[->] (C1) -- (A1);

%         \draw[->] (A0) -- (D0);
%         \draw[->] (E0) -- (D0);
%         \draw[->] (A1) -- (D1);
%         \draw[->] (E1) -- (D1);
        

%     \end{tikzpicture}
%     \caption{Operation Graph Example}
%     \label{fig:operation_graph}
% \end{figure}

% On Figure \ref{fig:operation_graph}, we can see the operation graph of the listing \ref{lst:og}.

From this representation, we can easily define key properties to subsequently estimate the latency and area of this code region, such as its span, or critical path. % \cite{someone}.

\begin{definition}[Operation Graph critical path]
\label{def:ogcriticalpath}
Given $OG^L$ an operation graph for region $L$. Its critical path $OG_{cp}$ is the longest of all the shortest paths between every pairs $(v_i,v_o) \in <\{V_I,root\},V_O>$. 
% Its length, in number of nodes, is noted $\#OG_{cp}^L$.
Its length is noted $\#OG_{cp}^L$.
\end{definition}

% \FIXME{Link with the other operation graph}

On the graph on the Figure \ref{fig:tree_diagram} the critical paths from $A[i]$ to 
$c, \forall i \in$ \([\![0, 7]\!]\), 
have the same length.


\subsubsection{Latency Lower Bound}

We can build a simple a lower bound on the latency of an operation graph:
\begin{theorem}[Lower bound on latency of an Operation Graph]
\label{th:latlbcp}
Given infinite resources, and assuming no operation nor memory movement can take less than one cycle to complete, the latency $LAT_{cp}^L \ge \#OG_{cp}^L$ is a lower bound on the minimal feasible latency to execute $L$.
\end{theorem}

\begin{proof}[Proof Th \ref{th:latlbcp}]
Every operation $S_i$ is associated with at least one edge with a source in $<\{V_I,root\}>$, so there is a path between one of these nodes and every operation by construction in Def.~\ref{def:computationgraph}. For an operation to produce a useful output, there must be a path from its output to a node in $V_O$, otherwise the operation may be removed by dead code elimination. Therefore the shortest path $sp$ between a pair of nodes $(v_i, v_o) \in <\{V_I,root\},V_O>$ is the shortest sequence of operations in dependence that must be executed to produce $v_o$. As any operation takes at least one cycle to complete per Def.~\ref{th:latlbcp}, then this path must take at least $\#sp$ cycles to complete. As we take the largest of the shortest paths between all possible pairs  $(v_i, v_o)$ then $OG_{cp}^L$ is the length of the longest shortest path to produce any output $v_o$ from some input, via a sequence of producer-consumer operations. Therefore it must take at least $\#OG_{cp}^L$ cycles to execute this path.
\end{proof}


%\begin{proof}
%% probably have to show that if it was to take less cycles, then it would have to be because there is an operation taking less than 1 cycle?
%By definition the critical path is the longest path of all the shortest paths between every pairs of node $(v_i,v_o) \in <V_I,V_O>$ through the OG graph and the lower bound of the latency is the minimal number of cycles to perform all operations while respecting the dependencies.
%Suppose the critical path is not the lower bound then there is another path through the graph such that all operations are executed that is shorter than the critical path. Which is false by contradiction.
%Hence, the critical path is the lower bound.
%\end{proof}


We can then build a tighter lower bound on the number of cycles a region $L$ may take to execute, under fixed resources, by simply taking the maximum between the weighted span and the work to execute normalized by the resources available.

\begin{theorem}[Latency Lower Bound under Operation Resource Constraints] 
\label{th:latlbresources}
Given $R_{op}$ a count of available resources of type $op$, for each operation type, and $LO(op)$ the latency function for operation $op$, with $LO(op) \ge 1$. $\#L(op)$ denotes the number of operations of type $op$ in $L$. We define $LO(\#OG_{cp}^L) = \sum_{n \in cp} LO(n)$ the critical path weighted by latency of its operations.
The minimal latency of a region $L$ is bounded by 
$$
Lat_{R_{op}}^L \ge \max(LO(\#OG_{cp}^L),\max_{o \in op} (\lceil \#L(o) \times LO(o) /R_{o}\rceil))
$$
\end{theorem}

\begin{proof}[Proof Th \ref{th:latlbresources}]
Suppose $\forall o \in op,~R_{o} \ge \#L(o) $. Then there is equal or more resources available than work to execute, this is equivalent to the infinite resource hypothesis of Th.~\ref{th:latlbcp}, the minimal latency is $LO(\#OG_{cp}^L)$.

Suppose $\exists o \in op,~R_{o} < \#L(o)  $. Then there exists at least one unit in $R_{o}$ that is executing $\lceil \#L(o) /R_{o} \rceil$ operations. As every operation $op$ take at $L(op) \ge 1$ cycle to complete, this unit will execute in at least  $\lceil \#L(o) \times L_{o}/R_{o} \rceil$ cycles. If $\lceil \#L(o) \times L_{o}/R_{o} \rceil \ge LO(\#OG_{cp}^L)$, the computation cannot execute in less than $\lceil \#L(o) \times L_{o}/R_{o} \rceil$ cycles.
\end{proof}

% \FIXME{May here show an ILP formulation on the CDAG that achieves the lower bound, and reason that all are (over-)approximations of this perfect scheduling+placement solution?}

This theorem provides the building block to our analysis: if reasoning on a straight-line code region, without any loop, then building the operation graph for this region and reasoning on its critical path is sufficient to provide a latency lower bound. 

\begin{lstlisting}[label={lst:reference_bicg},caption={Bicg code: $s=r \times A; q=A \times p$}]
L1: for (i = 0; i < N; i++)  
    S0: s[i] = 0;
L2: for (i = 0; i < M; i++) { 
        S1: q[i] = 0;
    L3: for (j = 0; j < N; j++) {
        S2: s[j]+=r[i]*A[i][j]; 
        S3: q[i]+=A[i][j]*p[j];
    }
}
\end{lstlisting}
\vspace{.5cm}
For example, in Listing~\ref{lst:reference_bicg}, if we consider the sub-loop body composed of loops L3 (fully unrolled) and the statements $S2$ and $S3$ as straight-line code regions, we can calculate the critical paths for $S2$ and $S3$ as follows:
% 
For $S2$, the critical path is given by: $cp_{S2} = \max(L(+) + L(*), N \times (DSP_+ + DSP_*) / R_o)$ with $DSP_{o}$ the number of DSP for the operation $o$.
For $S3$, the critical path is determined by: $cp_{S3} = \max(L(+) \times \log(N) + L(*), N \times (DSP_+ + DSP_*) / R_o)$,  considering the possibility of a tree reduction.
In this context, the critical path for the entire sub-loop body is the maximum of these two individual critical paths, expressed as $\max(cp_{S2}, cp_{S3})$.

We now need to integrate loops and enable the composition of latency bounds.


\subsubsection{Loop Unrolling: full unroll}

% Loop unrolling is an HLS optimization that aims to execute multiple iterations of a loop in parallel. Intuitively, for an unroll factor $UF \ge 1$, $UF$ replications of the loop body will be instantiated. If $TC_l \mod UF_l \ne 0$ then an epilogue code to execute the remaining $TC_l \mod UF_l$ iterations is needed.

% We can bound the latency of a loop nest which has been entirely flatten, that is, all loops have been fully unrolled.

We start by reasoning on the bound for latency of a loop nest which has been fully unrolled, e.g. as a result of \texttt{\#pragma ACCEL parallel} or \texttt{\#pragma HLS unroll}. Full unrolling amounts to fully unroll all $TC$ iterations of a loop, replacing the loop by $TC$ replications of its original loop body, where the loop iterator has been updated with the value it takes, for each replication.

It follows a simple corollary:
\begin{corollary}[Equivalence between fully unrolled and straight-line code]
\label{cor:fullflattenstraightlinecode}
Given a loop nest $l$, if full unrolling is applied to $l$ then the code obtained after full unrolling is a straight-line code as per Def.~\ref{def:straightlinecode}.
\end{corollary}

\begin{proof}[Proof Co \ref{cor:fullflattenstraightlinecode}]
By construction the process of fully unrolling all the loops creates a straight-line code region without loop control, which therefore fits Def.~\ref{def:straightlinecode}.
\end{proof}

Consequently, we can bound the latency of a fully unrolled loop nest:
\begin{theorem}[Minimal latency of a fully unrolled loop nest]
\label{th:minlatflattenednest}
Given a loop nest $l$, which is first rewritten by fully unrolling all loops to create a straight-line code region $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then its minimal latency is bounded by:
$$
Lat_{R_{op}}^l \ge \max(LO(\#OG_{cp}^L),\max_{o \in op} (\lceil \#L(o) \times L_{o}/R_{o} \rceil))
$$
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatflattenednest}]
By Corollary~\ref{cor:fullflattenstraightlinecode}.
\end{proof}

\subsubsection{Loop Unrolling: partial unroll} 

Loop unrolling is an HLS optimization that aims to execute multiple iterations of a loop in parallel. Intuitively, for an unroll factor $UF \ge 1$, $UF$ replications of the loop body will be instantiated. If $TC_l \mod UF_l \ne 0$ then an epilogue code to execute the remaining $TC_l \mod UF_l$ iterations is needed.

% \FIXME{NOTE: write here some comment on what happens if you unroll non-rectangular loops, loops where UF does not divide TC, etc. from the Merlin/Vitis implementation point of view.}

% Partial unrolling can be viewed as a two-step transformation: first strip-mine the loop by the unroll factor, then consider the inner loop obtained is fully-unrolled. The latency of the resulting sub-program is determined by how the outer-loop generated will be implemented. We assume without additional explicit information this outer loop will execute in a non-pipelined, non-parallel fashion, to provide the following bound:

Unrolling can be viewed as a two-step transformation: first strip-mine the loop by the unroll factor, then consider the inner loop obtained to be fully-unrolled. The latency of the resulting sub-program is determined by how the outer-loop generated will be implemented. 
We assume without additional explicit information this unrolled loop will execute in a non-pipelined, non-parallel fashion.
Note this bound requires to build the operation graph for the whole loop body. This is straightforward for inner loops and/or fully unrolled loop nests, but impractical if the loop body contains other loops. We therefore define a weaker, but more practical, bound \emph{that enables composition}:

\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF]
\label{th:minlatunrolled1}
Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^{'}$ the loop body obtained by replicating $UF$ times the original loop body $L$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^{L^{'}}
$$    
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatunrolled1}]
By construction and Theorem~\ref{th:latlbresources}, $Lat_{R_{op}}^{L^{'}}$ is a lower bound on the latency of $L^{'}$, that is the sub-program made of $UF$ iterations of the loop. $\lfloor TC/UF \rfloor \le TC_l/UF$ is a lower bound on the number of iterations of the loop. As we assume a non-pipelined execution for the resulting outer loop, every iteration shall start after the completion of the preceding one, that is its iteration latency, itself bounded by $Lat_{R_{op}}^{L^{'}}$.
\end{proof}

% (*@\colorbox{green}{\textcolor{black}{}}@*)
\begin{lstlisting}[label={lst:partial_before_unroll},caption=Example before partial unrolling,escapechar=!]
#pragma ACCEL parallel UF=4
L1: for (i = 0; i < 8; i++)  {
    S0: a[i] = b[i] * c[i];
}
\end{lstlisting}
% \vspace{-0.5cm}

% \begin{tikzpicture}[remember picture,overlay]
% \draw[black,rounded corners]
%   ([shift={(-3pt,2ex)}]pic cs:w) 
%     rectangle 
%   ([shift={(3pt,-0.65ex)}]pic cs:q);
% \end{tikzpicture}

% \begin{tikzpicture}[remember picture,overlay]
% \draw[black,rounded corners]
%   ([shift={(-3pt,2ex)}]pic cs:n) 
%     rectangle 
%   ([shift={(3pt,-0.65ex)}]pic cs:t);
% \end{tikzpicture}

\begin{lstlisting}[label={lst:partial_after_unroll},caption=Example after partial unrolling,escapechar=!]
// explicitly unroll with UF=4
L1: for (i = 0; i < 8; i+=4)  {
    S0: a[i] = b[i] * c[i];
    S1: a[i+1] = b[i+1] * c[i+1];
    S2: a[i+2] = b[i+2] * c[i+2];
    S3: a[i+3] = b[i+3] * c[i+3];
}
\end{lstlisting}
\vspace{.4cm}

% \begin{tikzpicture}[remember picture,overlay]
% \draw[black,rounded corners]
%   ([shift={(-3pt,2ex)}]pic cs:n) 
%     rectangle 
%   ([shift={(3pt,-0.65ex)}]pic cs:t);
% \end{tikzpicture}

% \begin{tikzpicture}[remember picture,overlay]
% \draw[black,rounded corners]
%   ([shift={(-3pt,2ex)}]pic cs:n) 
%     rectangle 
%   ([shift={(3pt,-0.65ex)}]current page.east|-{pic cs:t});
% \end{tikzpicture}

% On the Listing \ref{lst:partial_before_unroll}, $L$ represent the green part which is unroll by a factor 4 and is explicitly unrolled on the listing \ref{lst:partial_after_unroll}, hence the purple code represent the loop body $L^{'}$.


In Listing \ref{lst:partial_before_unroll}, the loop body denoted by $L$ is depicted in the rectangle. The loop L1 is subjected to a partial unrolling with a factor of 4, as specified by the directive \textit{#pragma ACCEL parallel UF=4} hence S0 have to be expanded and replicated four times.
% 
The explicit unrolling of the loop is illustrated in Listing \ref{lst:partial_after_unroll}, where S0, S1, S2 and S3 represent the loop body $L^{'}$ of the Theorem \ref{th:minlatunrolled1}.
% 
The latency of the program in Listing \ref{lst:partial_before_unroll} and \ref{lst:partial_after_unroll} (which are equivalent) is greater or equal to $\lfloor \frac{TC}{UF} \rfloor$, in this case 2, multiply by the latency of the loop body $L^{'}$.

Note this bound requires to build the operation graph for the whole loop body. This is straightforward for inner loops and/or fully unrolled loop nests, but impractical if the loop body contains other loops. We therefore define a weaker, but more practical, bound:

%\FIXME{Need to precise that we use DSA. And cite Feautrier papier for transformation Affine -> DSA}

\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF and complex loop bodies]
\label{th:minlatunrolled2}
Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor * Lat_{R_{op}}^L
$$    
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatunrolled2}]

% Key argument to prove: style of: lat(S1,forloop) >= max(lat(S1),lat(forloop) that is by adding a new instruction we dont reduce the cp length. A counter example is
% \{for i:  a = a+b\};a = 43


% if we consider a CDAG, adding the edge a = 43 gives a shorter path to a than any of the i iteration in the fully unrolled cdag. So we must add conditions such as writes to the same location have to be all executed, in the order of the original code (sensible condition in presence of data dependencies WAW).

% Proof flow:
% 1) Given $OG^{i}$ and $OG^j$ two CDAGs, for a pair of distinct iterations $i,j$ of loop $L$. If $V_O^i \cap V_O^j = \emptyset$, then the graph $OG^{i,j}$ made of the two iterations $i,j$ cannot have a smaller critical path length than $OG^{i}$ and $OG^j$: there is no edge crossing $OG^{i}$ and $OG^j$ in $OG^{i,j}$ since outputs are distincts, therfore $Lat(OG^{i,j} \ge \max(Lat(OG^i),Lat(OG^j))$.

% 2) Suppose now  $V_O^i \cap V_O^j \ne \emptyset$. Then iterations $i$ and $j$ produce at least one output in common. IDEA: DSA. If the program is in dynamic single assignent form, this is a contradiction (DSA: only 1 write per location). Need to adjust defs at start to be in DSA form? Mention automatic conversion from affine to DSA exists (Feautrier, 90s).


Given $OG^i$ and $OG^j$ two CDAGs, for a pair of distinct iterations $i,j$ of loop $l$. 

If $V_O^i \cap V_O^j = \emptyset$, then the graph $OG^{i,j}$ made of the two iterations $i,j$ cannot have a smaller critical path length than $OG^i$ and $OG^j$: there is no edge crossing $OG^i$ and $OG^j$ in $OG^{i,j}$ since outputs are distinct, therefore $Lat(OG^{i,j}) \ge \max(Lat(OG^i),Lat(OG^j))$.

If $V_O^i \cap V_O^j \ne \emptyset$. Then iterations $i$ and $j$ produce at least one output in common. As there is no useless operation, the graph $OG^{i,j}$ made of the two iterations $i,j$ can not be smaller than $OG^i$ or $OG^j$ and hence $Lat(OG^{i,j}) \ge \max(Lat(OG^i),Lat(OG^j))$.

\end{proof}

Consider the scenario of loop $L0$ within Listing \ref{lst:reference_bicg}, which has been unrolled by a factor denoted as $UF \leq TC_{L0}$ where $TC_{L0}$ is the trip count of $L0$. The latency for one iteration of $S0$ is denoted as $Lat^{S0}_{R_{o}} > 0$.
In the absence of pipelining, the lower bound of the latency of this sub-loop body is: $\lfloor TC_{L0} / UF \rfloor \times Lat^{S0}_{R_{o}}$.

% \FIXME{The above theorem covers the composition case of C operator, with children made of loops with a bound and statements. Perhaps worth rewriting the theorem (or a corrollary) to show this composition of children is valid? That would conclude the formulas with the pipelining below.}

Vitis allows to do a reduction with a tree reduction in logarithmic time with the option ``unsafe-math''. 

% \textcolor{red}{TODO: Should we decompose red and // operation ?}

\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF for reduction loop with tree reduction]
\label{th:minlatunrolled3}
Given a reduction loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$, if executed in a non-pipelined fashion and the tree reduction is legal is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^L \times \lfloor \log_2(UF)  \rfloor
$$    
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatunrolled3}]
    
    By definition a reduction loop is a loop with a dependency distance of 1. Hence, at each iteration the same memory cell is read and write. 
Because of the dependency distance of 1, only one element can be added to the same memory cell.
However each data can be adding independently two by two and the result of this independent addition can also be adding two by two until we obtained one value. Hence the reduction can be done in $\log_2(UF)$ iterations with a tree reduction.
As the depth of the tree is $\log_2(UF)$ and each node at the same depth can be executed independently in $Lat_{R_{op}}^L$ cycles, the straight line code has a latency greater or equal to $Lat_{R_{op}}^L \times \lfloor \log_2(UF)  \rfloor$. And then similarly to Th. \ref{th:minlatunrolled2} and \ref{th:minlatunrolled3} the sequential execution of the loops without pragma repeat this process $\lfloor TC/UF \rfloor$ times.
    
\end{proof}

\begin{lstlisting}[label={lst:tree_red},caption={
Example of code demonstrating a reduction, where a tree reduction technique can be applied, as depicted in Figure \ref{fig:tree_diagram}.}]
L1: for (i = 0; i < 8; i++)  {
    c += a[i];
}
\end{lstlisting}
\vspace{.5cm}


\begin{figure}
    \centering
    \rotatebox{180}{%
\begin{forest}
[\rotatebox{180}{c}, for tree={circle, draw, minimum size=2em, edge={<-}}
  [+, for tree={circle, draw, minimum size=2em, edge={<-}}
    [+, for tree={circle, draw, minimum size=2em, edge={<-}}
        [+, for tree={circle, draw, minimum size=2em, edge={<-}}
            [{\rotatebox{180}{$A[7]$}}]
            [{\rotatebox{180}{$A[6]$}}]
        ]
        [+, for tree={circle, draw, minimum size=2em, edge={<-}}
            [{\rotatebox{180}{$A[5]$}}]
            [{\rotatebox{180}{$A[4]$}}]
        ]
    ]
    [+, for tree={circle, draw, minimum size=2em, edge={<-}}
        [+, for tree={circle, draw, minimum size=2em, edge={<-}}
            [{\rotatebox{180}{$A[3]$}}]
            [{\rotatebox{180}{$A[2]$}}]
        ]
        [+, for tree={circle, draw, minimum size=2em, edge={<-}}
            [{\rotatebox{180}{$A[1]$}}]
            [{\rotatebox{180}{$A[0]$}}]
        ]
    ]
  ]
]
% [\rotatebox{180}{c}, for tree={circle, draw, minimum size=2em, edge={<-}}
%   [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%     [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%       [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[7]]
%               [B[7]]
%               [,phantom]
%               [tmp7, name=tmp7]
%             ]
%         ]
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[1]]
%               [B[1]]
%             ]
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[0]]
%               [B[0]]
%             ]
%         ]
%       ]
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[7]]
%               [B[7]]
%               [,phantom]
%               [tmp7, name=tmp7]
%             ]
%         ]
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[1]]
%               [B[1]]
%             ]
%             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
%               [A[0]]
%               [B[0]]
%             ]
%         ]
      
%     ]
%   ]
% ]
  % \node[above=1cm, align=center, font=\bfseries] at (!r.north) {Computation Tree};
  % \draw[->, dashed] (tmp) -- (C);
  % \draw[->, dashed] (tmp) -- (C);
  % \draw[->, dashed] (tmp) -- (C);
\end{forest}
}

    \caption{Illustrating the concurrent execution depicted in Listing \ref{lst:tree_red} through a tree reduction method, accomplished within logarithmic time.}
    \label{fig:tree_diagram}
\end{figure}


Figure \ref{fig:tree_diagram} represent the tree reduction of the Listing \ref{lst:tree_red}. Due to the reduction, we use a tree reduction in order to increase the parallelism of the reduction, and execute a loop of trip count $n=8$ in $\log_2(n)=3$ iterations.

% \begin{forest}
%   % [*, for tree={circle, draw, minimum size=2em, edge={->}}
%   %   [a[0]]
%   %   [b[0]]
%   % ]
%   [ , for tree={}
%     [*, for tree={circle, draw, minimum size=2em, edge={->}}
%       [a[0]]
%       [b[0]]
%     ]
%     [+, for tree={circle, draw, minimum size=2em, edge={->}}
%       [*, for tree={circle, draw, minimum size=2em, edge={->}}
%         [a[1]]
%         [b[1]]
%       ]
%       [+, for tree={circle, draw, minimum size=2em, edge={->}}
%         [$\ldots$]
%         [+, for tree={circle, draw, minimum size=2em, edge={->}}
%           [a[7]]
%           [b[7]]
%         ]
%       ]
%     ]
%   ]

% \end{forest}

\subsubsection{Loop pipelining} 

% Loop pipelining amounts to overlapping multiple iterations of the loop, so that the next iteration can start prior to the completion of the preceding one. The initiation interval (II) measures in cycles the delay between the start of two consecutive iterations. 

Loop pipelining amounts to overlapping multiple iterations of the loop, so that the next iteration can start prior to the completion of the preceding one. The initiation interval (II) measures in cycles the delay between the start of two consecutive iterations. It is easy to prove our formula template accurately integrates the latency of pipelined loops with the $I$ operator.
% 
We compute the minimal II in function of the dependencies of the pipelined loop and the iteration latency of the operations of the statements during the NLP generation. 
Let $RecMII$ and $ResMII$ be the recurrence constraints and the resource constraints of the pipelined loop, respectively. We have $II \geq \max{(ResMII, RecMII)}$. 
% 
$RecMII = \max_i \lceil \frac{ delay(c_i)}{ distance(c_i)} \rceil$ with $delay(c_i)$ the total latency in dependency cycle $c_i$ and $distance(c_i)$ the total distance in dependency cycle $c_i$.
% As we cannot compute accurately $ResMII$ as we don't know how the resource will be used by the compiler 
We suppose that $ResMII=1$, as we do not know how the resource will be used by the compiler.
% 
Hence, if the loop is a reduction loop then the $II \geq \frac{IL_{reduction}}{1}$ with $IL_{reduction}$ the iteration latency of the operation of reduction. For a kernel like the Listing \ref{lst:ex_II}
% $for (j = 0; j < N; j++) y[j] = y[j-2] + 3;$ 
the $II \geq \lceil \frac{IL_+}{2} \rceil$.

\begin{lstlisting}[label={lst:ex_II},caption={Demonstration of a code snippet showcasing a scenario where a loop pipelined with a dependency of distance 2 results in an initiation interval ($II$) that satisfies $II \geq \lceil \frac{IL_+}{2} \rceil$. }]
for (j = 0; j < N; j++) 
    y[j] = y[j-2] + 3;
\end{lstlisting}
\vspace{1cm}

It follows a bound on the minimal latency of a pipelined loop:
\begin{theorem}[Minimal latency of a pipelined loop with known II]
\label{th:minlatpipeline}
Given a loop $l$ with trip count $TC_l$ and loop body $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$ if executed in a pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,P} \ge Lat_{R_{op}}^L + II *( TC_l - 1)
$$    
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatpipeline}]
$Lat_{R_{op}}^L$ is the minimal latency to complete one iteration of $l$ by Theorem~\ref{th:latlbresources}. The initiation interval measures the number of elapsed cycles before the next iteration can start, it takes therefore at least $TC_l * II - 1$ to start $TC_l - 1$ iterations, irrespective of their completion time. Therefore the latency of the loop is at least the latency of one iteration to complete, and for all iterations to be started.
\end{proof}



\subsubsection{Loop pipelining and unrolling}

A loop $l$ with trip count $TC_l$ can be pipelined and partially unrolled with $UF < TC_l$, in this case there is loop splitting where the trip count of the innermost loop equal to the unroll factor and the trip count of the outermost loop equal to $\frac{TC_l}{UF}$.



\begin{theorem}[Minimal latency of a pipelined loop with known II and partially unrolled]
\label{th:minlatpipeline_unrolled}
Given a loop $l$ with trip count $TC_l$, partially unrolled by an unroll factor $UF < TC_l$ and a loop body $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^{'}$ the loop body obtained by replicating UF times the original loop body $L$.
Then the minimal latency of $l$ if executed in a pipelined fashion is bounded by:

$$
Lat_{R_{op}}^{l,P} \ge Lat_{R_{op}}^{L^{'}} 
+ II * ( \frac{TC_l}{UF} - 1)
$$    
\end{theorem}

\begin{proof}[Proof Th \ref{th:minlatpipeline_unrolled}]

By construction and Theorem \ref{th:minlatflattenednest} the latency $Lat_{R_{op}}^{L^{'}}$ is a lower bound of $L^{'}$. As the loop was split due to the partial unrolling, the trip count of the pipelined loop is $\frac{TC_l}{UF}$. Theorem \ref{th:minlatpipeline} gives us the lower bound of the latency for a loop with a trip count equal to $\frac{TC_l}{UF}$.

\end{proof}

\subsubsection{Non-Parallel, Non-Pipelined Loops}

We continue with a trivial case: if the loop is not optimized by any directive (including any automatically inserted by the compilers), i.e., not parallelized nor pipelined, then every next iteration of the loop starts only after the end of the prior iteration.

\begin{definition}[Lower bound on latency of a non-parallel, non-pipelined loop under resources constraints]
\label{def:loopIteratedSequentially}
Given a loop $l$ with trip count $TC_l$ which is neither pipelined nor parallelized, that is, iteration $i+1$ starts after the full completion of iteration $i$, for all iterations. Given $Lat_{R_{op}}^L$ the minimal latency of its loop body. Then
$$
Lat_{R_{op}}^l \ge TC_l * Lat_{R_{op}}^L
$$

\end{definition}

\subsubsection{Coarse-Grained parallelization}

Coarse-grained parallelization is a performance enhancement technique involving the unrolling of a loop which iterates a loop body not fully unrolled i.e., containing at least a pipelined loop or a loop executed sequentially. It is therefore impossible to do a coarse-grained parallelization with a reduction loop because the $n$ sub loop body are dependent on each other.


It follows a bound on the minimal latency of a coarse-grained unrolled loop:
\begin{theorem}[Minimal latency of coarse-grained unrolled loop]
\label{th:coarse_grained}

Given a loop $l$, which is not a reduction loop, with trip count $TC_l$, an unroll factor $UF \le TC_l$ and  $L$ the loop body iterated by the loop $l$ with a latency lower bound $Lat^{L}_{R_{op}}$. 
Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^{'}$ the loop body obtained by replicating $UF$ times the original loop body $L$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^{L^{'}}
$$
\end{theorem}

\begin{proof}[Proof Th \ref{th:coarse_grained}]


By construction, Definition \ref{def:loopIteratedSequentially}, Theorem \ref{th:minlatpipeline} and definition of the loop body $L$, $Lat^{L}_{R_{op}}$ is a lower bound of the loop body $L$. As the loop is not a reduction loop there is no dependency between the loop bodies of $L$ for different iteration of $l$ and then the loop bodies can be executed in parallel. 
If $UF < TC_l$, then $\lfloor TC_l/UF \rfloor \leq TC_l / UF $ is a lower bound on the number of iterations of the loop. As we assume a non-pipelined execution for the resulting outer loop, every iteration shall start after the
completion of the preceding one, that is its iteration latency, itself bounded by 
$ Lat_{R_{op}}^{L^{'}} $.

\end{proof}

% \paragraph*{Latency under resource constraint} 

% \FIXME{Statement not define for the following th}

% \begin{theorem}[Minimal resource consumption]
% \label{th:minresource}
% Given a loop body $L$, available resources $R_{op}$ and configuration of pragma $C$. 

% On the condition that the resources are only used by the operations of the different statements
% the minimal number of resource (DSPs) consumed by $L$ for the configuration $C$ is:
% % $$
% % R_{op} < \sum_{op} \max_{t}( \#L_{op}^t) \times DSP_{op} 
% % $$    

% $$
% R_{op} < \sum_{op} \max_{S \in \mathcal{S}_{par}}( \min(1,\#L_{op}^{S}) \times DSP_{op} \times UF^{S})
% $$    

% % with $\#L_{op}^t$ the number of operation $op$ in parallel at time $t$ and $DSP_{op}$ the number of resource (DSPs) used for the operation $op$.

% with $\#L_{op}^t$ the number of operation $op$ in parallel for the statements $S$ which are under the same loop unrolled, $DSP_{op}$ the number of resource (DSPs) used for the operation $op$ and $\mathcal{S}_{par}$ the set of set statements which are under the same unrolled loop.

% \end{theorem}

% \begin{proof}
    
% Here we suppose a perfect reuse intra and inter statement, which means if a computational unit is not used at time $t$, it can be reuse.

% Suppose the formula is wrong, i.e. at time $t$, we can use less resource and hence globally consume less resource. 

% % In this case, we can reuse a computational unit
% 1. If at time $t$ no resource has been used until now, we are oblige to used the number of computational unit necessary for the operations in parallel.

% 2. If at time $t$ we can reuse all the resource, then the number of resource used at time $t$ are less or equal to the resource already used

% 3. If at time $t$ the number of computational unit necessary for the computation is greater than the number of available resource already used and available. Then we reuse the maximum of resource unused plus the difference of new resource needed to do the computation. We can differentiate three possible cases:
%     3.1 If two statements are under the same unrolled loop then we only count one computation unit per operation for all the statements under the loop(s) unrolled.
%     3.2 If two statements are not under the same unrolled loop, then when the second statement will be run all resource consumed by the first statement will be free and hence can be reused.
%     3.3 If a loop is pipelined and the II is not as expected we still have the minimum of DSP used because of reuse intra-statement i.e. the minimal number of DSP will be independant of the II.

% In all case, the number of DSP is minimal.




% % Plus complique que ca il faut dire que y'a un reuse intra statement
% %  mais qu'on suppose qu'il est utilisé que 1 fois par chaque statement
% % du coup faut reecrire la formule
% % 
% % 
    
% \end{proof}

% \begin{theorem}[Maximal resource consumption]
% \label{th:maxresource}
% Given a loop body $L$, available resources $R_{op}$ and configuration $C$. 
% On the condition that the resources are only used by the operations of the different statements
% the maximum number of resource (DSPs) consumed by $L$ is:
% $$
% R_{op} \ge \sum_{S \in \mathcal{S}} \sum_{op}\max_{t}( \#L_{op}^{S,t}) \times DSP_{op} 
% $$    
% with $\#L_{op}^t$ the number of operation $op$ in parallel at time $t$ and $\mathcal{S}$ the set of statements.

% \end{theorem}

% \begin{proof}
% % est ce que c'est pas se compliquer la vie ?

% Here we suppose we don't have reuse inter and intra-statement. Hence, if one statement need to do two additions, the two additions will used different computational unit and these computational units will not be used for other statement.

% As we sum all the resource used per operation per statement we have to prove that 1. The same operation for the same statement can't used more resource than $DSP_{op}$. And we have as hypothesis than the operation $op$ used $DSP_{op}$.

% 2. If more parallelism the number of DSP will be greater. However, we know the configuration as input and hence know the parallelism of the kernel.



% % Problem if UF does not divide TC  => False Problem because if Merlin transform we know the code

    
% \end{proof}

% \begin{theorem}[Latency under resource constraint]
% \label{th:minlatpipeline}
% Given a loop body $L$, available resources $R_{op}$, lower bound without constraint $lb$ and configuration $C$. 

% The lower bound $lb$ can not be achieve under resource constraint if 
% $$
% R_{op} < \sum_{op} \max_{S \in \mathcal{S}_{par}}( \min(1,\#L_{op}^{S}) \times DSP_{op} \times UF^{S})
% $$    
% with $\#L_{op}^t$ the number of operation $op$ in parallel for the statements $S$ which are under the same loop unrolled, $DSP_{op}$ the number of resource (DSPs) used for the operation $op$ and $\mathcal{S}_{par}$ the set of set statements which are under the same unrolled loop.

% The lower bound $lb$ can be achieve under resource constraint if 
% $$
% R_{op} \ge \sum_{S \in \mathcal{S}} \sum_{op}\max_{t}( \#L_{op}^{S,t}) \times DSP_{op} 
% $$    
% with $\mathcal{S}$ the set of statements.
% \end{theorem}

% \begin{proof}
% We compute the resource used for two cases:

% \begin{itemize}
%     \item Perfect Reuse, which is intra and inter statement. If a resource is not use at time $t$, then it can be reuse for the same operation.
%     \item No reuse, i.e. each statement use different resource.
% \end{itemize}


% In the first case (perfect reuse), it is impossible to consume less resource, as proof in Theorem \ref{th:minresource}. In the second case, it is impossible to consume more resource, as proof in Theorem \ref{th:maxresource}. Hence, if a loop body $L$ 
% has a minimum of resource comsumption greater than resource available
% the loop body can not be synthesized and run on this board. Hence the lower bound can not be achieve.

% In other way if a loop body $L$, has a maximal amount of resource lesser than resource available the design can be synthetized and run on this board. The lower bound can be achieve.

% If in practice at least one pragma is not applied as expected, then we have an other configuration with it is own lower bound.

% % If the hypothesis of reuse is wrong hence the resource consumed is greater than the one computed and the resource used are greater than resource available.
% \end{proof}

\subsubsection{Program latency lower bound under resource constraints} 

We now focus on the latency lower bound of a program, under resource constraints. This bound takes into account the limitations imposed by available resources, which can significantly affect the achievable performance.
% 
We assume here that the resources consumed are only consumed by the computing units and resource use by the computational unit of one operation can not be reused by the computational unit of another operation executing at the same time. We also assume that the compilers have implemented the pragma configuration given as input.


For DSPs we suppose we have a perfect reuse i.e., that the computation units for the same operation can be reused as soon as the computation unit is not in use. Under-estimating the resources used is fundamental to proving the latency lower bound, as otherwise another design that consumes less resources than predicted may be feasible, itself possibly leading to a better latency. 


\begin{theorem}
\label{th:minres}
    Given a loop body $L$,  the set of set of  statements $\mathcal{S}_{seq}$ non executed in parallel, 
$\#L_{op}^s$ the number of operations $op$  for the statements $s$, $DSP_{op}$ the number of resources (DSPs) used for the operation $op$, $MCU_{op}^s$ the maximal number of computational units the statement $s$ can use in parallel at any given time,  and  the configuration of pragma $\vec{PV_i}$ for each loop.
The minimal number of resource (DSPs) consumed, $R_{used}^{min}$, by $L$ for the pragma configuration  is the sum, for each operation, of the maximum number of DSPs used in parallel by a statement.
This corresponds to:
$$R^{min}_{used} =  \sum_{op} \max_{\mathcal{S} \in \mathcal{S}_{seq}}( \sum_{s \in \mathcal{S}}
\#L_{op}^s
\times DSP_{op} 
\times MCU_{op}^{s})$$
\end{theorem}

\begin{proof}[Proof Th \ref{th:minres}]
    Considering perfect resource reuse, where all unused computational units can be reused, and assuming that the compilers have implemented the pragma configuration provided as input. 
For each statement $s$, the maximum number of computational units used in parallel is determined. This means that each statement $s$ requires at least $\#L_{op}^s \times DSP_{op} \times MCU_{op}^s$ DSPs. 
If a set of statements $\mathcal{S}$ are executed in parallel they cannot share the resource so the execution in parallel of the statement $s \in \mathcal{S}$ will require $( \sum_{s \in \mathcal{S}}
\#L_{op}^s
\times DSP_{op} 
\times MCU_{op}^{s})$ DSPs.
% 
By considering the maximum across all statements, we can guarantee that at least one set of statement executed in parallel will require $\max_{s \in \mathcal{S}_{seq}}(\sum_{s \in \mathcal{S}} \#L_{op} \times DSP_{op} \times MCU_{op}^s)$ DSPs.
Since there is no possibility of resource reuse between different operations, the summation of the resource consumed for each operation remains the minimum consumption of resources. In other words, the sum of the individual resource consumption for each operation represents the minimum amount of resources required.
\end{proof}


Given a program and the available resource of DSP $DSP_{avail}$, if $R^{min}_{used} < DSP_{avail}$ the lower bound is valid and the program does not over-utilize the resources. 

%%% LNP: I cannot parse this sentence.
%The latency lower bound of a kernel is therefore the latency lower bound of the configuration such that the minimal resource consumption is less than or equal to the resource available.

% \begin{theorem}[Latency Lower bound of a program]
% \label{th:minlatpipelineunderresourceconstraint}
% % Given a kernel, available resource $R_{op}$, the set of statements $\mathcal{S}$ and all the configuration of pragmas which are constitute of  the vectors $\Vec{PV_i}$ for each loop.
% Given a loop body $L$,  the set of statements $\mathcal{S}$,
% $\#L_{op}^s$ the number of operation $op$  for the statements $s$, $DSP_{op}$ the number of resources (DSPs) used for the operation $op$, $MCU_{op}^{s}$ the maximal number of computational unit the statement $s$ can use in parallel, and  the configuration of pragma  $\Vec{PV_i}$ for each loop.

% The configuration of pragma, which has the minimal lower bound and which respect $R_{used}^{min} = \sum_{op} \max_{s \in \mathcal{S}}(
% \#L_{op}^s
% \times DSP_{op} 
% \times MCU_{op}^{s}) \leq R_{op}$, is the lower bound of the kernel.


% \end{theorem}


% \begin{proof}[Proof Th \ref{th:minlatpipelineunderresourceconstraint}]

%     According to Theorem \ref{th:minres}, $R_{used}^{min}$ is the minimal number of DSP a configuration can use. Hence, all configuration which does not respect the constraint $R_{used}^{min}\leq R_{op}$ have a over-utilization of the resource and hence are invalid.

%     Hence, the minimal lower bound of each configuration of pragma is the lower bound of the kernel.
    
% \end{proof}

%   

\subsubsection{Memory transfer}

AMD/Xilinx Merlin manages automatically the memory transfer. The memory transfer and computation are not overlap (no dataflow) hence the latency is the sum of the latency of computation and communication. We assume that for each array the contents of the array are in the same DRAM bank.

\begin{theorem}[Lower bound of the memory transfer latency for an array]
\label{th:memlatonearray}

Given a loop body $L$,  the set of array $\mathcal{A}$,  an array $a \in \mathcal{A}$, and $LAT^{mem}_a$ the latency to transfer the array $a$ from off-chip to on-chip (inputs) and from on-chip to off-chip (outputs).
$\forall a \in \mathcal{A}, LAT^{mem}_a \geq 
(\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$.
With $\mathds{1}_{cond} = 1$ if $cond$ = true else 0.

\end{theorem}

\begin{proof}[Proof Th \ref{th:memlatonearray}]
    In order to transfer all the elements of the array $a$ we can use packing with a maximum packing allowed by the target device of $max\_burst\_size$, which means in practice the real burst size will be equal or less than $max\_burst\_size$.
    As all the elements of the array $a$ are in the same bank, the transfer is sequential. And as we as suppose all operation including memory transfers are done in at least one cycle, the minimum latency is $footprint_a / max\_burst\_size$ to transfer once the array $a$. As an array can be input, output or both we need to add the transfer from off-chip to on-chip for inputs i.e., $a \in V_I^L$ and from on-chip to off-chip for the outputs i.e., $a \in V_O^L$.
    
\end{proof}

%%%%%%% TODO: figure with footprint, 512 bits, off-chip and on-chip mem

% \begin{figure}
%     \centering
% \begin{tikzpicture}[
%     node distance=2cm,
%     block/.style={draw, rectangle, align=center, minimum height=1.5cm, minimum width=2.5cm},
%     arrow/.style={-Stealth, thick},
% ]

% % Off-chip memory
% \node[block, fill=blue!20] (offchip) {Off-chip\\Memory};
% \draw[<->, thick] ([yshift=-0.5cm]offchip.south west) -- ([yshift=-0.5cm]offchip.south east) node[midway, below] {512 bits};

% % On-chip memory
% \node[block, right=of offchip, fill=green!20] (onchip) {On-chip\\Memory};

% % Arrow indicating data transfer
% \draw[arrow] (offchip.east) -- (onchip.west) node[midway, above] {Transfer};

% % Footprint of off-chip memory
% \draw[dashed, thick, draw=red] ([xshift=-0.5cm]offchip.north west) rectangle ([xshift=0.5cm]offchip.south east) node[midway, right=1cm] {Footprint};

% \end{tikzpicture}
% \caption{Memeory transfer from off-chip to on-chip}
%     \label{fig:mem_trans}
% \end{figure}


\begin{theorem}[Lower bound of the memory transfer latency]
\label{th:memlat}

Given a loop body $L$,  the set of array $\mathcal{A}$, the number of cycles to transfer  the array $a$ is bounded by $\max_{a \in \mathcal{A}} (\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$.

\end{theorem}

\begin{proof}[Proof Th \ref{th:memlat}]
According to Th. \ref{th:memlatonearray} the lower bound to transfer one array $a$ is $(\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$. As the array can be on different DRAM banks the transfer from off-chip to on-chip can be done in parallel but at least one array has a latency greater or equal to $(\mathds{1}_{a \in V_O^L} + \mathbb{\in V_I^L}) \times footprint_a / max\_burst\_size$ and hence the memory latency is equal to $\max_{a \in \mathcal{A}} (\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L})  \times footprint_a / burst\_size$. 
\end{proof}

% \begin{theorem}[Lower bound of the memory latency under resource constraint]
% \label{th:memlat_resource}

% TODO mem on chip

% Given a loop body $L$,  the set of array $\mathcal{A}$, the number of cycle to transfer  the array $a$ is bounded by $\max_{a \in \mathcal{A}} (\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$.

% \end{theorem}

% \begin{proof}[Proof Th \ref{th:memlat_resource}]
% According to Th. \ref{th:memlatonearray} the lower bound to transfer one array $a$ is $(\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$. As the array can be on different DRAM banks the transfer from off-chip to on-chip can be done in parallel but at least one array have a latency greater or equal to $(\mathds{1}_{a \in V_O^L} + \mathbb{\in V_I^L}) \times footprint_a / max\_burst\_size$ and hence the memory latency is equal to $\max_{a \in \mathcal{A}} (\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L})  \times footprint_a / burst\_size$. 
% \end{proof}





\subsection{Summary}



By composing all the theorems, this allows us to end up with the final latency lower bound of the program which is presented in theorems \ref{th:comp_lb} for the computation and \ref{th:global_lb} for the computation and communication.




\begin{theorem}[Computation Latency Lower bound of a Program]
\label{th:comp_lb}

Given available resource $DSP_{avail}$, the properties vector $\Vec{PV}_i$ for each loop and a program which contains a loop body $L$.
The properties vector allows to give all the information concerning the trip counts and the II of the pipelined loops and to decompose the loop body $L$ with a set of loops $\mathcal{L}^{non \; reduction}_{L}$ potentially coarse-grained unrolled with $\forall l \in \mathcal{L}_{L}, UF_l$ and a set of reduction loops executed sequentially $\mathcal{L}^{reduction}_{L}$ which iterates a loop body $L_{pip}$. 
% 
By recursion the loop body $L_{pip}$ contains a pipelined loop $l_{pip}$ which iterate a loop body $L_{fg}$ fully unrolled. The loop body $L_{fg}$ contains operations which can be done in parallel with a latency $Lat^{L_{par}}_{R_{op}}$ 
and operations which are reduction originally iterated by the loops $\mathcal{L}^{reduction}_{L_{fg}}$ with a latency $Lat_{L_{seq}}$. 

The computation latency lower bound of $L$, which respected $DSP^{min}_{ued} \leq DSP_{avail}$, executed with tree reduction is:

$$
Lat^{L}_{R_{op}} \geq \prod_{l\in \mathcal{L}^{par}_{L}} \frac{TC_l}{UF_l} \times 
\prod_{l\in \mathcal{L}^{reduction}_{L}} TC_l \times Lat^{L_{pip}}_{R_{op}}
$$

with 

$Lat^{L_{pip}}_{R_{op}} = (Lat^{L_{fg}}_{R_{op}} + II\times (\frac{TC_{l_{pip}}}{l_{pip}\_UF}-1) )$
and 
$Lat^{L_{fg}}_{R_{op}} = Lat_{L_{par}} +
Lat_{L_{seq}} \times \prod_{l\in \mathcal{L}^{reduction}_{L_{fg}}} \frac{TC_l}{UF_l} \times \log_2(UF_l)   $.

\end{theorem}


\begin{proof}[Proof Th \ref{th:comp_lb}]

% By composition and Theorems \ref{th:minlatunrolled1} and \ref{th:minlatunrolled2}, $Lat_{L_{fg}}$ is a lower bound of the fully unrolled sub-loop body of $L$, $L_{fg}$.

% By composition and Theorems \ref{th:minlatpipeline} and \ref{th:minlatpipeline_unrolled}, $Lat_{L_{pip}}$ is a lower bound of $L_{pip}$.

% By composition, Theorem \ref{th:coarse_grained} and Definition \ref{def:loopIteratedSequentially}, $Lat_{L}$ is a lower bound of $L$.

Through composition and the application of Theorems \ref{th:minlatflattenednest}, \ref{th:minlatunrolled1} and  \ref{th:minlatunrolled2}, $Lat^{L_{fg}}_{R_{op}}$ serves as a computation latency lower bound for the fully unrolled sub-loop body of $L$, denoted as $L_{fg}$, where $Lat_{L_{par}} +
Lat_{L_{seq}} \times \prod_{l\in \mathcal{L}^{reduction}_{L_{fg}}} \frac{TC_l}{UF_l} \times \log_2(UF_l)$ represent the critical path of $Lat^{L_{fg}}_{R_{op}}$.

By employing composition alongside Theorems \ref{th:minlatpipeline} and \ref{th:minlatpipeline_unrolled}, $Lat^{L_{pip}}_{R_{op}}$ stands as a computation latency lower bound for $L_{pip}$.

Utilizing composition, Theorem \ref{th:coarse_grained}, and Definition \ref{def:loopIteratedSequentially}, $Lat^{L}_{R_{op}}$ emerges as a computation latency lower bound for $L$.

\end{proof}



\begin{theorem}[Latency lower bound of a program optimized with Merlin pragmas]
\label{th:global_lb}

Given available resource $DSP_{avail}$ and a program which contains a loop body $L$ with a computation latency $Lat_{L}^{computation}$ and a communication latency $Lat_{L}^{communication}$.

The lower bound for $L$ which respected $DSP^{min}_{ued} \leq DSP_{avail}$ and where the computation and communication can not be overlap is:

$$
Lat_{L} = Lat_{L}^{computation} + Lat_{L}^{communication}
$$

\end{theorem}


\begin{proof}[Proof Th \ref{th:global_lb}]
The AMD/Xilinx Merlin compiler does not overlap computation and communication. Hence the computation and communication is a sum of the latency of computation and latency of communication.
By composition and Theorems \ref{th:comp_lb} and \ref{th:memlat}.

\end{proof}




==> sources/th_proof_model_template.tex <==
\subsection{Analytical Model Template}
\label{sec:analyticalModelTemplate}

To build the analytical formula for a program, we start from its summary AST in constructor notation and  the set of $\vec PV_i$ vectors for each loop, and rewrite it using the following operators, each detailed below:
\begin{enumerate}
    \item replace the $Loop_i(\vec X)$ operator by the loop information operator $I^{\vec PV_i}_i(\vec X)$;
    \item replace a list of children $\vec X$, which can be made of statements and loops, by the dependence-aware composition operator $C^{\vec PV_i}_i(\vec X)$ for this list;
    \item replace the list of consecutive statements $\vec S_x$ by the straight-line operator $SL^{\vec PV_i}_i(\vec S_x)$, which captures the profile of a straight-line code block.
\end{enumerate}

\paragraph{Loop information operator}
We define $I^{\vec PV_i}_i(X)$, the operator for loop $i$ associated with the property vector $PV_i$, where $X$ represents the cost associated with its loop body, as follows:

\[
I^{\vec{PV}_i}_i(X) = \begin{cases} 
      \left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor + X & \text{if loop } i \text{ is pipelined}  \\
      & (\text{ispip}_i = 1) \\ \\
      \left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor \cdot X & \text{otherwise } (\text{ispip}_i = 0)
   \end{cases}
\]

That is, if the loop is pipelined, we approximate its latency as the sum of the latency of the loop body with a function of the number of loop iterations \cite{comba}, otherwise as the product of the number of iterations and latency of the loop body. This can be encoded in a non-linear program as:

$$
I^{\vec{PV}_i}_i(X) =  
      \left(\left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor + X\right) \cdot \text{ispip}_i + 
      \left(\left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor \cdot X) \cdot (1 - \text{ispip}_i)\right)
$$

%For simplicity, we will represent the operation as $\odot$ to differentiate between the two different cases. 

\paragraph{Composition of siblings AST nodes}

We define $C_i^{\vec PV_i}(X_1, X_2)$, which composes the latency of $X_1$ and $X_2$ as follows:

\[
C_i^{\vec PV_i}(X_1, X_2) = \begin{cases} 
      max(X_1, X_2) & \text{ if } (X_1, X_2) \text{ do not have dependencies (WaR, RaW, WaW)} \\
      % \\
      % & \text{inparallel}_i = 1 = 1 - \text{insequence}_i \\ \\
      X_1 + X_2 & \text{otherwise}
   \end{cases}
\]


Indeed, if there is no dependence between two blocks (be they statements, loops, or a mix of both) then in the best case they may execute fully in parallel, and their latency is the maximum between them. If there exists a dependence between them, then they must execute in sequence and their latencies are summed. We perform fine-grain polyhedral data dependence analysis to determine the exact and minimal set of data dependences between loop iterations and statements, as discussed in Sec.~\ref{sec:formulation}.


\begin{comment}
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[label={lst:example_dep},caption={Example of code where two statements have dependencies}]
S0: x1 += y;
S1: x2 += x1 + z;
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[label={lst:example_nodep},caption={Example of code where two statements do not have dependency}]
S0: x1 += y;
S1: x2 += z;
\end{lstlisting}
\end{minipage}
\vspace{0.6cm}
\end{comment}

% \begin{lstlisting}[label={lst:example_dep},caption={Example of code where two statements have dependencies} ]
% S0:x1 += y;
% S1:x2 += x1 + z;
% \end{lstlisting}
% \vspace{0.5cm}

% \begin{lstlisting}[label={lst:example_nodep},caption={Example of code where two statements do not have dependency} ]
% S0:x1 += y;
% S1:x2 += z;
% \end{lstlisting}
% \vspace{0.5cm}


\begin{comment}
In List~\ref{lst:example_dep}, statements $S0$ and $S1$ exhibit dependencies, resulting in a program latency equal to the sum of their latencies, corresponding to $issequence=1$. Conversely, the statements in List~\ref{lst:example_nodep} lack dependencies, allowing $S0$ and $S1$ to be executed concurrently. Therefore, the latency is determined by the maximum of $S0$ and $S1$ latencies, representing the case $inparallel=1$.
\end{comment}

\paragraph{Modeling straight-line code regions}

Finally, $SL^{\vec PV_i}_i(\vec S_k)$ denotes a region of straight-line code (e.g., an inner-loop body), made of 1 or more statements $\vec S_k$. 
% which is used below in the formal reasoning on the bounds on latency of this template formula. 
Intuitively, $SL$ will represent a lower bound on the latency of a code block such that by composition across all loops as per the template formula, the result remains a lower bound on the full program latency. 


\paragraph{Example}

Returning to the example in Sec.~\ref{sec:modeling}, we can rewrite the summary AST expression:
\[
Loop_i(Loop_{j1}(S1), Loop_{j2}(S2,S3))
\]

into

\[
I^{\vec PV_i}_i(C^{\vec PV_i}(I^{\vec PV_{j1}}_{j1}(SL^{\vec PV_{j1}}_{j1}(S1)), I^{\vec PV_{j2}}_{j2}(SL^{\vec PV_{j2}}_{j2}(S2,S3))))
\]

By applying the simple rewrite described above. Upon substituting the definitions, and assuming here that the statements are independent, we obtain:

{
\small
\[
% I^{\vec PV_i}_i(
\left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor \odot_{\text{ispip}_i}
    % C^{\vec PV_i}(
    \max \left(
        % I^{\vec PV_{j1}}_{j1}(
        \left\lfloor II_{j1} \cdot \left(\frac{TC^{avg}_{j1}}{uf_{j1}} - \text{ispip}_{j1}\right) \right\rfloor \odot_{\text{ispip}_{j1}}
            SL^{\vec PV_{j1}}_{j1}(S1)
        % ), 
        ,
        % I^{\vec PV_{j2}}_{j2}(
        \left\lfloor II_{j2} \cdot \left(\frac{TC^{avg}_{j2}}{uf_{j2}} - \text{ispip}_{j2}\right) \right\rfloor  \odot_{\text{ispip}_{j2}}
            SL^{\vec PV_{j2}}_{j2}(
                S2,
                S3
            )
        \right)
%     )
% )
\]
}

\noindent where for brevity of the notation, we write $\odot_{\text{ispip}_i} X$ to represent $\cdot X$ or $+ X$ in the $I$ operators.


==> sources/th_proof_summary.tex <==
% \section{Analytical Model}

% \label{sec:appendix}
\label{sec:theoretical}



We present the foundational components of our analytical performance model and demonstrate how this model computes a lower bound on latency while adhering to resource constraints. The theorems and their accompanying proofs can be found in Appendix \ref{appendix:theoretical}.

\subsection{Analytical Model Template}
\label{sec:analyticalModelTemplate}


Consider the expression $I^{\vec PV_i}_i(X)$ for the loop $i$, where $X$ denotes a subpart of the program, and the operators are defined as follows:

\[
I^{\vec{PV}_i}_i(X) = \begin{cases} 
      \left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor + X & \text{if loop } i \text{ is pipelined}  \\
      & (\text{ispip}_i = 1) \\ \\
      \left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor \cdot X & \text{otherwise } (\text{ispip}_i = 0)
   \end{cases}
\]

For simplicity, we will represent the operation as $\odot$ to differentiate between the two different cases. 

Let $C_i^{\vec PV_i}(X_1, X_2, \dots, X_n)$ which compose the different sub part of a program under the loop $i$.

\[
C_i^{\vec PV_i}(X_1, X_2, \dots, X_n) = \begin{cases} 
      max(X_1, X_2, \dots, X_n) & \text{ if } (X_1, \dots, X_n) \text{ do not have dependencies (WaR, RaW, WaW)} \\
      % \\
      % & \text{inparallel}_i = 1 = 1 - \text{insequence}_i \\ \\
      \sum_{k=1}^n X_k & \text{otherwise}
   \end{cases}
\]

\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[label={lst:example_dep},caption={Example of code where two statements have dependencies}]
S0: x1 += y;
S1: x2 += x1 + z;
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[label={lst:example_nodep},caption={Example of code where two statements do not have dependency}]
S0: x1 += y;
S1: x2 += z;
\end{lstlisting}
\end{minipage}
\vspace{0.6cm}

% \begin{lstlisting}[label={lst:example_dep},caption={Example of code where two statements have dependencies} ]
% S0:x1 += y;
% S1:x2 += x1 + z;
% \end{lstlisting}
% \vspace{0.5cm}

% \begin{lstlisting}[label={lst:example_nodep},caption={Example of code where two statements do not have dependency} ]
% S0:x1 += y;
% S1:x2 += z;
% \end{lstlisting}
% \vspace{0.5cm}


In List~\ref{lst:example_dep}, statements $S0$ and $S1$ exhibit dependencies, resulting in a program latency equal to the sum of their latencies, corresponding to $issequence=1$. Conversely, the statements in List~\ref{lst:example_nodep} lack dependencies, allowing $S0$ and $S1$ to be executed concurrently. Therefore, the latency is determined by the maximum of $S0$ and $S1$ latencies, representing the case $inparallel=1$.

Finally, $SL^{\vec PV_i}_i(\vec S_k)$ denotes a region of straight-line code (e.g., an inner-loop body). 
% which is used below in the formal reasoning on the bounds on latency of this template formula. 
Intuitively, $SL$ will represent a lower bound on the latency of a code block such that by composition across all loops as per the template formula, the result remains a lower bound on the full program latency. 

Given the summary AST of the program in constructor form, and the set of $\vec PV_i$ vectors for each loop, we build the analytical formula template as follows: 
\begin{enumerate}
    \item replace the $Loop_i(\vec X)$ operator by $I^{\vec PV_i}_i(\vec X)$ operator;
    \item replace the $\vec X$ list by $C^{\vec PV_i}_i(\vec X)$;
    \item replace statement lists inside loop \texttt{i} $\vec S_x$ by $SL^{\vec PV_i}_i(\vec S_x)$.
\end{enumerate}
For our example, we can rewrite the expression:
\[
Loop_i(Loop_{j1}(S1), Loop_{j2}(S2,S3))
\]

as

\[
I^{\vec PV_i}_i(C^{\vec PV_i}(I^{\vec PV_{j1}}_{j1}(SL^{\vec PV_{j1}}_{j1}(S1)), I^{\vec PV_{j2}}_{j2}(SL^{\vec PV_{j2}}_{j2}(S2,S3))))
\]

Upon substituting the definitions and assuming that the statements are independent, we obtain:

\[
% I^{\vec PV_i}_i(
\left\lfloor II_i \cdot \left(\frac{TC^{avg}_i}{uf_i} - \text{ispip}_i\right) \right\rfloor \odot
    % C^{\vec PV_i}(
    \max \left(
        % I^{\vec PV_{j1}}_{j1}(
        \left\lfloor II_{j1} \cdot \left(\frac{TC^{avg}_{j1}}{uf_{j1}} - \text{ispip}_{j1}\right) \right\rfloor \odot
            SL^{\vec PV_{j1}}_{j1}(S1)
        % ), 
        ,
        % I^{\vec PV_{j2}}_{j2}(
        \left\lfloor II_{j2} \cdot \left(\frac{TC^{avg}_{j2}}{uf_{j2}} - \text{ispip}_{j2}\right) \right\rfloor  \odot
            SL^{\vec PV_{j2}}_{j2}(
                S2,
                S3
            )
        \right)
%     )
% )
\]

% \FIXME{I let you judge but I think it is unreadable for 2mm}

% 2mm on Listing \ref{lst:2mm}  can be represented by: 
% $
% (Loop_{i_1}(Loop_{j_1}(S_0, Loop_{k_1}(S1))) , Loop_{i_2}(Loop_{j_2}(S_2, Loop_{k_2}(S3))))
% $. If we apply the definition of $C^{PV}$ and $I^{PV}$ we have the following equation:

% % I^{\vec PV_{i_1}}_{i_1}
% $
% (
%     I^{\vec PV_{i_1}}_{i_1}(
%         I^{\vec PV_{j_1}}_{j_1}(
%             C_{j_1}^{\vec PV_{j_1}}(
%                 SL^{\vec PV_{j_1}}_{j_1}(S_0), 
%                 I^{\vec PV_{k_1}}_{k_1}(
%                     SL^{\vec PV_{k_1}}_{k_1}(S1)
%                 )
%             )
%         )
%     ) , 
%     I^{\vec PV_{i_2}}_{i_2}(
%         I^{\vec PV_{j_2}}_{j_2}(
%             C_{j_1}^{\vec PV_{j_2}}(
%                 SL^{\vec PV_{j_2}}_{j_2}(S_2), 
%                 I^{\vec PV_{k_2}}_{k_2}(
%                     SL^{\vec PV_{k_2}}_{k_2}(S3)
%                 )
%             )
%         )
%     )
% )
% $
% .

% Upon substituting the definition, we acquire:

% $
% (
%     % I^{\vec PV_{i_1}}_{i_1}(
%     \lfloor II_{i_1} * (TC^{avg}_{i_1} /uf_{i_1} - ispip_{i_1})  \rfloor \odot 
%         % I^{\vec PV_{j_1}}_{j_1}(
%         \lfloor II_{j_1} * (TC^{avg}_{j_1} /uf_{j_1} - ispip_{j_1})  \rfloor \odot 
%             % C_{j_1}^{\vec PV_{j_1}}(
%             sum(
%                 SL^{\vec PV_{j_1}}_{j_1}(S_0), 
%                 % I^{\vec PV_{k_1}}_{k_1}(
%                 \lfloor II_{k_1} * (TC^{avg}_{k_1} /uf_{k_1} - ispip_{k_1})  \rfloor \odot 
%                     SL^{\vec PV_{k_1}}_{k_1}(S1)
%                 )
%             )
%         )
%     ) , 
%     % I^{\vec PV_{i_2}}_{i_2}(
%    \lfloor II_{i_2} * (TC^{avg}_{i_2} /uf_{i_2} - ispip_{i_2})  \rfloor \odot 
%         % I^{\vec PV_{j_2}}_{j_2}(
%         \lfloor II_{j_2} * (TC^{avg}_{j_2} /uf_{j_2} - ispip_{j_2})  \rfloor \odot 
%             % C_{j_1}^{\vec PV_{j_2}}(
%             sum(
%                 SL^{\vec PV_{j_2}}_{j_2}(S_2), 
%                 % I^{\vec PV_{k_2}}_{k_2}(
%                 \lfloor II_{k_2} * (TC^{avg}_{k_2} /uf_{k_2} - ispip_{k_2})  \rfloor \odot 
%                     SL^{\vec PV_{k_2}}_{k_2}(S3)
%                 )
%             )
%         )
%     )
% )
% $.



\subsection{A Formal Model for Latency}

Our objective is to formulate a lower bound on the latency of a program after HLS. We therefore have put several restrictions: we assume the input program is a polyhedral program, that is the control-flow is statically analyzable; all loops can be recognized and their trip count computed; and all array / memory accesses can be exactly modeled at compile-time. No conditional can occur in the program. While our approach may generalize beyond this class, we limit here to these strict assumptions.

To maintain a lower bound on latency by composition, we operate on a representation of (parts of the) program which is both schedule-independent and storage-independent: indeed, a lower bound on this representation is necessarily valid under any schedule and storage eventually implemented. \emph{We however require HLS to not change the count and type of operations}. Furthermore, for lower bounding purposes, we assume unless stated otherwise $\forall i,~inparallel_i = 1$. We will discuss in the next section a more realistic but compiler-dependent approach to set $inparallel_i$, based on dependence analysis.

We assume programs are made of affine loops, that are loops with statically computable control-flow, with loop bounds made only of intersection of affine expressions of surrounding loop iterators and program constants. We now assume loop bodies (i.e., statements surrounded by loops) have been translated to a list of statements, with at most a single operation (e.g., \texttt{+,-,/,*}) per statement. Operations are n-ary, that is they take $n \ge 0$ input scalar values as operand, and produce 0 or 1 output scalar value. A memory location can be loaded from (resp. stored to) an address stored in a scalar variable. This is often referred to as straight-line code
% \cite{some-good-def}
. 
This normalization of the loop body facilitates the computation of live-in/live-out data for the code block, and the extraction of the computation graph. Note the region can be represented in Static Single Assignment 
% \cite{ssa} 
form, to ensure different storage location for every assignment, facilitating the construction of the operation graph.
% 
In addition we require the input program to not contain useless operations which may be removed by the HLS toolchain e.g. by dead code elimination, as illustrated in Listing~\ref{lst:dead-code}.


\begin{lstlisting}[caption={Example of Code Illustrating Dead Code Elimination: As Statement S1 writes to variable x, but the value of x assigned in Statement S0 is never used, the compiler will remove Statement S0.},label={lst:dead-code}]
int example(int y, int z){
    int x;
    S0: x = 12 + y; //  dead-code elimination
    S1: x = y + z;
    return x;
}
\end{lstlisting}
\vspace{0.7cm}


The restriction can be summarized as:

\begin{itemize}[leftmargin=*]
    \item The input program is a pure polyhedral program \cite{girbal06ijpp}, and its analysis (loop trip counts for every loop, all data dependences \cite{Fea92b}) is exact.
    \item No HLS optimization shall change the number of operations in the computation: strength reduction, common sub-expression elimination, etc. shall either first be performed in the input program before analysis, or not be performed by the HLS toolchain. The program also does not contain "useless" operations that may be removed by the compiler.
    \item We only model DSP and BRAM resources for the considered kernel, ignoring all other resources. We do not model LUT and FF resources, because from experience in the loop-based benchmarks we consider DSP and BRAM resources are the most constraining resources. Moreover, the estimation of LUTs and FFs is more tedious.
    \item We assume resource (DSP) sharing across different operations executing at the same cycle is not possible.
\end{itemize}

An important term is $SL$, a latency lower bound for a region of straight-line code. To maintain a lower bound on latency by composition, we operate on a representation of (parts of the) program which is both schedule-independent and storage-independent: the operation graph, or CDAG \cite{elango2015characterizing}. Indeed, a lower bound on this representation is necessarily valid under any schedule and storage eventually implemented and can be used to prove I/O lower bounds on programs \cite{elango2015characterizing} which is the directed acyclic graph with one node per operation in the code region, connecting all producer and consumer operations to build the operation graph. Then, we can easily compute the length of its critical path, which represents the minimal set of operations to execute serially.




We can compute the directed acyclic graph made of all statements (i.e., all n-ary operations), connecting all producer and consumer operations, to build the operation graph: % 
% \cite{someothergoodref}:

\begin{definition}[Operation Graph] 
\label{def:computationgraph}
Given a straight-line code region $R$ made of a list $L$ of statements $S \in L$, the operation graph OG is the directed graph $<\{N,V_I,root,V_O\},E>$ such that $\forall S_i \in L,~N_{S_i} \in N$; and for every operation with output $o$ and inputs $\vec i$ in $L$ $\forall S_i, \forall i_k \in \Vec{i}_{S_i}, e_{i_k, o} \in E$,
$\forall S_i:(o_{S_i},{\vec i}_{S_i}) \in L, S_j:(o_{S_j},{\vec i}_{S_j}) \in L$ with $S_i \ne S_j$ then we have $E_{S_i,S_j} \in E$ iff $o_{Si}\cap{\vec i}_{S_j}\ne \emptyset$. For every input (resp. output) in $S_i$ which is not matched with an output (resp. input) of another $S_j$ in $L$, create a node $V_{val} \in V_I$ (resp. $V_O$) for this input (resp. output) value. If $dim({\vec i}_{S_i}) = 0$ then an edge $e_{root,S_i}$ is added to $E$.
\end{definition}



From this representation, we can easily define key properties to subsequently estimate the latency and area of this code region, such as its span, or critical path. % \cite{someone}.

\begin{definition}[Operation Graph critical path]
\label{def:ogcriticalpath}
Given $OG^L$ an operation graph for region $L$. Its critical path $OG_{cp}$ is the longest of all the shortest paths between every pairs $(v_i,v_o) \in <\{V_I,root\},V_O>$. 
% Its length, in number of nodes, is noted $\#OG_{cp}^L$.
Its length is noted $\#OG_{cp}^L$.
\end{definition}


On the graph on the Figure \ref{fig:tree_diagram} the critical paths from $A[i]$ to 
$c, \forall i \in$ \([\![0, 7]\!]\), 
have the same length.


\subsubsection{Latency Lower Bound}

We can build a simple a lower bound on the latency of an operation graph:
\begin{theorem}[Lower bound on latency of an Operation Graph]
\label{th:latlbcp}
Given infinite resources, and assuming no operation nor memory movement can take less than one cycle to complete, the latency $LAT_{cp}^L \ge \#OG_{cp}^L$ is a lower bound on the minimal feasible latency to execute $L$.
\end{theorem}



We can then build a tighter lower bound on the number of cycles a region $L$ may take to execute, under fixed resources, by simply taking the maximum between the weighted span and the work to execute normalized by the resources available.

\begin{theorem}[Latency Lower Bound under Operation Resource Constraints] 
\label{th:latlbresources}
Given $R_{op}$ a count of available resources of type $op$, for each operation type, and $LO(op)$ the latency function for operation $op$, with $LO(op) \ge 1$. $\#L(op)$ denotes the number of operations of type $op$ in $L$. We define $LO(\#OG_{cp}^L) = \sum_{n \in cp} LO(n)$ the critical path weighted by latency of its operations.
The minimal latency of a region $L$ is bounded by 
$$
Lat_{R_{op}}^L \ge \max(LO(\#OG_{cp}^L),\max_{o \in op} (\lceil \#L(o) \times LO(o) /R_{o}\rceil))
$$
\end{theorem}




This theorem provides the building block to our analysis: if reasoning on a straight-line code region, without any loop, then building the operation graph for this region and reasoning on its critical path is sufficient to provide a latency lower bound. 

\begin{lstlisting}[label={lst:reference_bicg},caption={Bicg code: $s=r \times A; q=A \times p$}]
\#pragma ACCEL unroll factor=uf
L0: for (i = 0; i < N; i++)  
    S0: s[i] = 0;
\#pragma ACCEL pipeline
L1: for (i = 0; i < M; i++) { 
        S1: q[i] = 0;
\#pragma ACCEL unroll
    L2: for (j = 0; j < N; j++) {
        S2: s[j]+=r[i]*A[i][j]; 
        S3: q[i]+=A[i][j]*p[j];
    }
}
\end{lstlisting}
\vspace{.5cm}
For example, in Listing~\ref{lst:reference_bicg}, if we consider the sub-loop body composed of loops L2 (fully unrolled) and the statements $S2$ and $S3$ as straight-line code regions, we can calculate the critical paths for $S2$ and $S3$ as follows:
% 
For $S2$, the critical path is given by: $cp_{S2} = \max(L(+) + L(*), N \times (DSP_+ + DSP_*) / R_o)$ with $DSP_{o}$ the number of DSP for the operation $o$.
For $S3$, the critical path is determined by: $cp_{S3} = \max(L(+) \times \log(N) + L(*), N \times (DSP_+ + DSP_*) / R_o)$,  considering the possibility of a tree reduction.
In this context, the critical path for the entire sub-loop body is the maximum of these two individual critical paths, expressed as $\max(cp_{S2}, cp_{S3})$.

We now need to integrate loops and enable the composition of latency bounds.


\subsubsection{Loop Unrolling: partial unroll} 

Loop unrolling is an HLS optimization that aims to execute multiple iterations of a loop in parallel. Intuitively, for an unroll factor $UF \ge 1$, $UF$ replications of the loop body will be instantiated. If $TC_l \mod UF_l \ne 0$ then an epilogue code to execute the remaining $TC_l \mod UF_l$ iterations is needed.


Unrolling can be viewed as a two-step transformation: first strip-mine the loop by the unroll factor, then consider the inner loop obtained to be fully-unrolled. The latency of the resulting sub-program is determined by how the outer-loop generated will be implemented. 
We assume without additional explicit information this unrolled loop will execute in a non-pipelined, non-parallel fashion.
Note this bound requires to build the operation graph for the whole loop body. This is straightforward for inner loops and/or fully unrolled loop nests, but impractical if the loop body contains other loops. We therefore define a weaker, but more practical, bound \emph{that enables composition}:

\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF]
\label{th:minlatunrolled1}
Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^{'}$ the loop body obtained by replicating $UF$ times the original loop body $L$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^{L^{'}}
$$    
\end{theorem}


\begin{lstlisting}[label={lst:partial_before_unroll},caption=Example before partial unrolling,escapechar=!]
\#pragma ACCEL parallel UF=4
L1: for (i = 0; i < 8; i++)  {
    S0: a[i] = b[i] * c[i];
}
\end{lstlisting}
% \vspace{-0.5cm}


\begin{lstlisting}[label={lst:partial_after_unroll},caption=Example after partial unrolling,escapechar=!]
// explicitly unroll with UF=4
L1: for (i = 0; i < 8; i+=4)  {
    S0: a[i] = b[i] * c[i];
    S1: a[i+1] = b[i+1] * c[i+1];
    S2: a[i+2] = b[i+2] * c[i+2];
    S3: a[i+3] = b[i+3] * c[i+3];
}
\end{lstlisting}
\vspace{.4cm}




In Listing \ref{lst:partial_before_unroll}, the loop body denoted by $L$ is depicted in the rectangle. The loop L1 is subjected to a partial unrolling with a factor of 4, as specified by the directive \textit{\#pragma ACCEL parallel UF=4} hence S0 have to be expanded and replicated four times.
% 
The explicit unrolling of the loop is illustrated in Listing \ref{lst:partial_after_unroll}, where S0, S1, S2 and S3 represent the loop body $L^{'}$ of the Theorem \ref{th:minlatunrolled1}.
% 
The latency of the program in Listing \ref{lst:partial_before_unroll} and \ref{lst:partial_after_unroll} (which are equivalent) is greater or equal to $\lfloor \frac{TC}{UF} \rfloor$, in this case 2, multiply by the latency of the loop body $L^{'}$. 
In this context, $L^{'}$ comprises statements S0, S1, S2, and S3. These four statements are independent of each other and can be executed concurrently. Therefore, the lower bound on latency for $L^{'}$ is equivalent to the latency of the multiplication operation.

Note this bound requires to build the operation graph for the whole loop body. This is straightforward for inner loops and/or fully unrolled loop nests, but impractical if the loop body contains other loops. We therefore define a weaker, but more practical, bound:


\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF and complex loop bodies]
\label{th:minlatunrolled2}
Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor * Lat_{R_{op}}^L
$$    
\end{theorem}

Consider the scenario of loop $L0$ within Listing \ref{lst:reference_bicg}, which has been unrolled by a factor denoted as $UF \leq TC_{L0}$ where $TC_{L0}$ is the trip count of $L0$. The latency for one iteration of $S0$ is denoted as $Lat^{S0}_{R_{o}} > 0$.
In the absence of pipelining, the lower bound of the latency of this sub-loop body is: $\lfloor TC_{L0} / UF \rfloor \times Lat^{S0}_{R_{o}}$.



Vitis allows to do a reduction with a tree reduction in logarithmic time with the option ``unsafe-math''. 


\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF for reduction loop with tree reduction]
\label{th:minlatunrolled3}
Given a reduction loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$, if executed in a non-pipelined fashion and the tree reduction is legal is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^L \times \lfloor \log_2(UF)  \rfloor
$$    
\end{theorem}


\begin{lstlisting}[label={lst:tree_red},caption={
Example of code demonstrating a reduction, where a tree reduction technique can be applied, as depicted in Figure \ref{fig:tree_diagram}.}]
L1: for (i = 0; i < 8; i++)  {
    c += a[i];
}
\end{lstlisting}
\vspace{.5cm}


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/tree.png}
%     \rotatebox{180}{%
% \begin{forest}
% [\rotatebox{180}{c}, for tree={circle, draw, minimum size=2em, edge={<-}}
%   [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%     [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [{\rotatebox{180}{$A[7]$}}]
%             [{\rotatebox{180}{$A[6]$}}]
%         ]
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [{\rotatebox{180}{$A[5]$}}]
%             [{\rotatebox{180}{$A[4]$}}]
%         ]
%     ]
%     [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [{\rotatebox{180}{$A[3]$}}]
%             [{\rotatebox{180}{$A[2]$}}]
%         ]
%         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
%             [{\rotatebox{180}{$A[1]$}}]
%             [{\rotatebox{180}{$A[0]$}}]
%         ]
%     ]
%   ]
% ]
% % [\rotatebox{180}{c}, for tree={circle, draw, minimum size=2em, edge={<-}}
% %   [+, for tree={circle, draw, minimum size=2em, edge={<-}}
% %     [+, for tree={circle, draw, minimum size=2em, edge={<-}}
% %       [+, for tree={circle, draw, minimum size=2em, edge={<-}}
% %         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
% %             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
% %               [A[7]]
% %               [B[7]]
% %               [,phantom]
% %               [tmp7, name=tmp7]
% %             ]
% %         ]
% %         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
% %             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
% %               [A[1]]
% %               [B[1]]
% %             ]
% %             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
% %               [A[0]]
% %               [B[0]]
% %             ]
% %         ]
% %       ]
% %         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
% %             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
% %               [A[7]]
% %               [B[7]]
% %               [,phantom]
% %               [tmp7, name=tmp7]
% %             ]
% %         ]
% %         [+, for tree={circle, draw, minimum size=2em, edge={<-}}
% %             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
% %               [A[1]]
% %               [B[1]]
% %             ]
% %             [*, for tree={circle, draw, minimum size=2em, edge={<-}}
% %               [A[0]]
% %               [B[0]]
% %             ]
% %         ]
      
% %     ]
% %   ]
% % ]
%   % \node[above=1cm, align=center, font=\bfseries] at (!r.north) {Computation Tree};
%   % \draw[->, dashed] (tmp) -- (C);
%   % \draw[->, dashed] (tmp) -- (C);
%   % \draw[->, dashed] (tmp) -- (C);
% \end{forest}
% }

    \caption{Illustrating the concurrent execution depicted in Listing \ref{lst:tree_red} through a tree reduction method, accomplished within logarithmic time.}
    \label{fig:tree_diagram}
\end{figure}


Figure \ref{fig:tree_diagram} represent the tree reduction of the Listing \ref{lst:tree_red}. Due to the reduction, we use a tree reduction in order to increase the parallelism of the reduction, and execute a loop of trip count $n=8$ in $\log_2(n)=3$ iterations.


\subsubsection{Loop pipelining} 


Loop pipelining amounts to overlapping multiple iterations of the loop, so that the next iteration can start prior to the completion of the preceding one. The initiation interval (II) measures in cycles the delay between the start of two consecutive iterations. It is easy to prove our formula template accurately integrates the latency of pipelined loops with the $I$ operator.
% 
We compute the minimal II in function of the dependencies of the pipelined loop and the iteration latency of the operations of the statements during the NLP generation. 
Let $RecMII$ and $ResMII$ be the recurrence constraints and the resource constraints of the pipelined loop, respectively. We have $II \geq \max{(ResMII, RecMII)}$. 
% 
$RecMII = \max_i \lceil \frac{ delay(c_i)}{ distance(c_i)} \rceil$ with $delay(c_i)$ the total latency in dependency cycle $c_i$ and $distance(c_i)$ the total distance in dependency cycle $c_i$.
% As we cannot compute accurately $ResMII$ as we don't know how the resource will be used by the compiler 
We suppose that $ResMII=1$, as we do not know how the resource will be used by the compiler.
% 
Hence, if the loop is a reduction loop then the $II \geq \frac{IL_{reduction}}{1}$ with $IL_{reduction}$ the iteration latency of the operation of reduction. For a kernel like the Listing \ref{lst:ex_II}
% $for (j = 0; j < N; j++) y[j] = y[j-2] + 3;$ 
the $II \geq \lceil \frac{IL_+}{2} \rceil$.

\begin{lstlisting}[label={lst:ex_II},caption={Demonstration of a code snippet showcasing a scenario where a loop pipelined with a dependency of distance 2 results in an initiation interval ($II$) that satisfies $II \geq \lceil \frac{IL_+}{2} \rceil$. }]
for (j = 0; j < N; j++) 
    y[j] = y[j-2] + 3;
\end{lstlisting}
\vspace{1cm}

It follows a bound on the minimal latency of a pipelined loop:
\begin{theorem}[Minimal latency of a pipelined loop with known II]
\label{th:minlatpipeline}
Given a loop $l$ with trip count $TC_l$ and loop body $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$ if executed in a pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,P} \ge Lat_{R_{op}}^L + II *( TC_l - 1)
$$    
\end{theorem}


In Listing~\ref{lst:reference_bicg}, loop $L1$ is pipelined. However, loop $L1$ serves is a reduction loop for statement $S2$, meaning that we must await the completion of writing $s[j]$ at iteration $i$ before we can read and write again at iteration $i+1$. Consequently, the initiation interval ($II$) is bounded by or greater than the latency ($IL_{+}$) of the addition operation, which constitutes the reduction operation.


\subsubsection{Loop pipelining and unrolling}

A loop $l$ with trip count $TC_l$ can be pipelined and partially unrolled with $UF < TC_l$, in this case there is loop splitting where the trip count of the innermost loop equal to the unroll factor and the trip count of the outermost loop equal to $\frac{TC_l}{UF}$.



\begin{theorem}[Minimal latency of a pipelined loop with known II and partially unrolled]
\label{th:minlatpipeline_unrolled}
Given a loop $l$ with trip count $TC_l$, partially unrolled by an unroll factor $UF < TC_l$ and a loop body $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^{'}$ the loop body obtained by replicating UF times the original loop body $L$.
Then the minimal latency of $l$ if executed in a pipelined fashion is bounded by:

$$
Lat_{R_{op}}^{l,P} \ge Lat_{R_{op}}^{L^{'}} 
+ II * ( \frac{TC_l}{UF} - 1)
$$    
\end{theorem}


\subsubsection{Non-Parallel, Non-Pipelined Loops}

We continue with a trivial case: if the loop is not optimized by any directive (including any automatically inserted by the compilers), i.e., not parallelized nor pipelined, then every next iteration of the loop starts only after the end of the prior iteration.

\begin{definition}[Lower bound on latency of a non-parallel, non-pipelined loop under resources constraints]
\label{def:loopIteratedSequentially}
Given a loop $l$ with trip count $TC_l$ which is neither pipelined nor parallelized, that is, iteration $i+1$ starts after the full completion of iteration $i$, for all iterations. Given $Lat_{R_{op}}^L$ the minimal latency of its loop body. Then
$$
Lat_{R_{op}}^l \ge TC_l * Lat_{R_{op}}^L
$$

\end{definition}

\subsubsection{Coarse-Grained parallelization}

Coarse-grained parallelization is a performance enhancement technique involving the unrolling of a loop which iterates a loop body not fully unrolled i.e., containing at least a pipelined loop or a loop executed sequentially. It is therefore impossible to do a coarse-grained parallelization with a reduction loop because the $n$ sub loop body are dependent on each other.


It follows a bound on the minimal latency of a coarse-grained unrolled loop:
\begin{theorem}[Minimal latency of coarse-grained unrolled loop]
\label{th:coarse_grained}

Given a loop $l$, which is not a reduction loop, with trip count $TC_l$, an unroll factor $UF \le TC_l$ and  $L$ the loop body iterated by the loop $l$ with a latency lower bound $Lat^{L}_{R_{op}}$. 
Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^{'}$ the loop body obtained by replicating $UF$ times the original loop body $L$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^{L^{'}}
$$
\end{theorem}



\subsubsection{Program latency lower bound under resource constraints} 

We now focus on the latency lower bound of a program, under resource constraints. This bound takes into account the limitations imposed by available resources, which can significantly affect the achievable performance.
% 
We assume here that the resources consumed are only consumed by the computing units and resource use by the computational unit of one operation can not be reused by the computational unit of another operation executing at the same time. We also assume that the compilers have implemented the pragma configuration given as input.


For DSPs we suppose we have a perfect reuse i.e., that the computation units for the same operation can be reused as soon as the computation unit is not in use. Under-estimating the resources used is fundamental to proving the latency lower bound, as otherwise another design that consumes less resources than predicted may be feasible, itself possibly leading to a better latency. 


\begin{theorem}
\label{th:minres}
    Given a loop body $L$,  the set of set of  statements $\mathcal{S}_{seq}$ non executed in parallel, 
$\#L_{op}^s$ the number of operations $op$  for the statements $s$, $DSP_{op}$ the number of resources (DSPs) used for the operation $op$, $MCU_{op}^s$ the maximal number of computational units the statement $s$ can use in parallel at any given time,  and  the configuration of pragma $\vec{PV_i}$ for each loop.
The minimal number of resource (DSPs) consumed, $R_{used}^{min}$, by $L$ for the pragma configuration  is the sum, for each operation, of the maximum number of DSPs used in parallel by a statement.
This corresponds to:
$$R^{min}_{used} =  \sum_{op} \max_{\mathcal{S} \in \mathcal{S}_{seq}}( \sum_{s \in \mathcal{S}}
\#L_{op}^s
\times DSP_{op} 
\times MCU_{op}^{s})$$
\end{theorem}



Given a program and the available resource of DSP $DSP_{avail}$, if $R^{min}_{used} < DSP_{avail}$ the lower bound is valid and the program does not over-utilize the resources. 

% In Listing~\ref{lst:reference_bicg}, S0 and S1 do not utilize any DSP as it is just an initialization. S2 and S3 are unrolled $N$ times and do not depend on each other so they can be executed in parallel, with a tree reduction for S3 as it is a reduction for the loop $L2$.
% In this case let suppose the number of DSP for the addition is 1 and for the multiplication is 2. So we have $DSP_+=1$ and $DSP_*=2$. The maximal number of computational units the statement $S2$ and $S3$ utilize is $N$ for the addition and the multiplication i.e. we have $MCU_{+}^{S2} = N, MCU_{*}^{S2} = N, MCU_{+}^{S3} = N, MCU_{*}^{S3} = N$. And we have only one addition and one multiplication per statement so $\#L^{S2}_+=1, \#L^{S2}_*=1, \#L^{S3}_+=1, \#L^{S3}_*=1$.
% So the minimal number of DSP the Listing~\ref{lst:reference_bicg} used is $N \times (1+2) \times 2$.


In Listing~\ref{lst:reference_bicg}, statements S0 and S1 entail no DSP usage as they solely serve for initialization purposes. S2 and S3 undergo unrolling N times and operate independently, enabling parallel execution. Particularly, S3 necessitates a tree reduction since it acts as a reduction for loop $L2$.

Assuming 1 DSP for addition and 2 for multiplication (denoted as $DSP_{+}$ and $DSP_{*}$ respectively), the maximum number of computational units utilized by S2 and S3 for both addition and multiplication is N. Therefore, $MCU_{+}^{S2} = N$, $MCU_{*}^{S2} = N$, $MCU_{+}^{S3} = N$, and $MCU_{*}^{S3} = N$. Furthermore, each statement entails only one addition and one multiplication, hence $\#L_{+}^{S2} = 1$, $\#L_{*}^{S2} = 1$, $\#L_{+}^{S3} = 1$, and $\#L_{*}*^{S3} = 1$.

Consequently, the minimum number of DSPs utilized by Listing~\ref{lst:reference_bicg} is $N \times (1+2) \times 2$.


\subsubsection{Memory transfer}

AMD/Xilinx Merlin manages automatically the memory transfer. The memory transfer and computation are not overlap (no dataflow) hence the latency is the sum of the latency of computation and communication. We assume that for each array the contents of the array are in the same DRAM bank.

\begin{theorem}[Lower bound of the memory transfer latency for an array]
\label{th:memlatonearray}

Given a loop body $L$,  the set of array $\mathcal{A}$,  an array $a \in \mathcal{A}$, and $LAT^{mem}_a$ the latency to transfer the array $a$ from off-chip to on-chip (inputs) and from on-chip to off-chip (outputs).
$\forall a \in \mathcal{A}, LAT^{mem}_a \geq 
(\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$.
With $\mathds{1}_{cond} = 1$ if $cond$ = true else 0.

\end{theorem}

Within Listing~\ref{lst:reference_bicg}, the matrix A is solely read and possesses a footprint of $N \times M \times 32$ bits. Given the FPGA's limitation to process a maximum of 512 bits per cycle, the latency required for transferring A amounts to $\frac{N \times M}{16}$ cycles.

\begin{theorem}[Lower bound of the memory transfer latency]
\label{th:memlat}

Given a loop body $L$,  the set of array $\mathcal{A}$, the number of cycles to transfer  the array $a$ is bounded by $\max_{a \in \mathcal{A}} (\mathds{1}_{a \in V_O^L} + \mathds{1}_{a \in V_I^L}) \times footprint_a / max\_burst\_size$.

\end{theorem}



In Listing~\ref{lst:reference_bicg}, when transferring all arrays before any computation, we can concurrently transfer each array (assuming they are in different DRAM banks). The primary bottleneck arises from the transfer of array $A$, which incurs a latency of $\frac{N \times M}{16}$ cycles. Upon program completion, arrays $s$ and $q$ need to be transferred back to DRAM, with a minimal latency of $\max(\frac{N}{16}, \frac{M}{16})$ cycles each. Thus, the total communication latency amounts to $\frac{N \times M}{16} + \max(\frac{N}{16}, \frac{M}{16})$ cycles.

\subsection{Summary}



By composing all the theorems, this allows us to end up with the final latency lower bound of the program which is presented in theorems \ref{th:comp_lb} for the computation and \ref{th:global_lb} for the computation and communication.




\begin{theorem}[Computation Latency Lower bound of a Program]
\label{th:comp_lb}

Given available resource $DSP_{avail}$, the properties vector $\Vec{PV}_i$ for each loop and a program which contains a loop body $L$.
The properties vector allows to give all the information concerning the trip counts and the II of the pipelined loops and to decompose the loop body $L$ with a set of loops $\mathcal{L}^{non \; reduction}_{L}$ potentially coarse-grained unrolled with $\forall l \in \mathcal{L}_{L}, UF_l$ and a set of reduction loops executed sequentially $\mathcal{L}^{reduction}_{L}$ which iterates a loop body $L_{pip}$. 
% 
By recursion the loop body $L_{pip}$ contains a pipelined loop $l_{pip}$ which iterate a loop body $L_{fg}$ fully unrolled. The loop body $L_{fg}$ contains operations which can be done in parallel with a latency $Lat^{L_{par}}_{R_{op}}$ 
and operations which are reduction originally iterated by the loops $\mathcal{L}^{reduction}_{L_{fg}}$ with a latency $Lat_{L_{seq}}$. 

The computation latency lower bound of $L$, which respected $DSP^{min}_{ued} \leq DSP_{avail}$, executed with tree reduction is:

$$
Lat^{L}_{R_{op}} \geq \prod_{l\in \mathcal{L}^{par}_{L}} \frac{TC_l}{UF_l} \times 
\prod_{l\in \mathcal{L}^{reduction}_{L}} TC_l \times Lat^{L_{pip}}_{R_{op}}
$$

with 

$Lat^{L_{pip}}_{R_{op}} = (Lat^{L_{fg}}_{R_{op}} + II\times (\frac{TC_{l_{pip}}}{l_{pip}\_UF}-1) )$
and 
$Lat^{L_{fg}}_{R_{op}} = Lat_{L_{par}} +
Lat_{L_{seq}} \times \prod_{l\in \mathcal{L}^{reduction}_{L_{fg}}} \frac{TC_l}{UF_l} \times \log_2(UF_l)   $.

\end{theorem}


% In Listing~\ref{lst:reference_bicg}, let call the loop body, with the loop $L0$ and statement $S0$, $LB0$. And the one with loop $L1$ and $L2$ and statements $S1, S2$ and $S3$ $LB1$.
% The loop body $LB0$ is unroll with an unroll factor $uf$ and there is no dependency between iteration of the loop, so the latency of  $LB0$ is bounded by $\frac{N}{uf} \times 1$, by supposing the initialization take at least 1 cycle.
% For loop body $LB1$, the loop $L2$ is fully unrolled and there is no dependency between iteration of the loop for the statement $S2$ but a tree reduction for the statement $S3$. We can note that for the statement $S3$ the multiplication do not have dependency and hence can be executed in parallel. As the pipelined loop $L1$ is a reduction for the statement $S2$, we have $II > IL_+$ with $IL_+$ the latency of the reduction operation. So the latency of $LB1$ is bounded by $(\max(IL_+ + IL_*, IL_* + \log_2(N) \times IL_+) + IL_+ \times (M-1))$.


In Listing~\ref{lst:reference_bicg}, let's denote the loop body with loop $L0$ and statement $S0$ as $LB0$, and the one with loops $L1$ and $L2$, along with statements $S1$, $S2$, and $S3$, as $LB1$.

For $LB0$, where the loop is unrolled with a factor $uf$ and no dependency exists between loop iterations, the latency is bounded by $\frac{N}{uf} \times 1$, assuming the initialization takes at least one cycle.

Regarding $LB1$, loop $L2$ is fully unrolled, with no dependencies between iterations for statement $S2$. As there is no dependency between $S2$ and $S3$, they can be executed in parallel, and the latency of the unrolled part equals the critical path, which is the maximum between the unrolled parts of $S2$ and $S3$ in this scenario. However, for statement $S3$, despite the absence of dependencies among multiplication operations enabling parallel execution, a tree reduction is involved. Given the pipelined nature of loop $L1$, functioning as a reduction for statement $S2$, we observe $II > IL_+$, where $IL_+$ denotes the latency of the reduction operation. Consequently, the latency of $LB1$ is bounded by $(\max(IL_+ + IL_*, IL_ + \log_2(N) \times IL_+) + IL_+ \times (M-1))$.

\begin{theorem}[Latency lower bound of a program optimized with Merlin pragmas]
\label{th:global_lb}

Given available resource $DSP_{avail}$ and a program which contains a loop body $L$ with a computation latency $Lat_{L}^{computation}$ and a communication latency $Lat_{L}^{communication}$.

The lower bound for $L$ which respected $DSP^{min}_{ued} \leq DSP_{avail}$ and where the computation and communication can not be overlap is:

$$
Lat_{L} = Lat_{L}^{computation} + Lat_{L}^{communication}
$$

\end{theorem}





==> sources/theoretical_and_modeling.tex <==
\label{sec:theoretical}

\REMARK{Details of the approach are difficult to follow. It is not clear whether the latency bound calculation (one of the main contributions) 
includes all relevant program information (i.e., cross-iteration dependencies). The approach is limited to a particular HLS flow (Merlin) 
and a particular type of applications (affine loops).}

\REMARK{The analytical model (Section 4A) is unclear}

\REMARK{ The discussion of the latency lower bound is clear in the basic situations, but the discussion of the latency in the presence of pipelining is minimal. This situation is, probably, the most interesting: how does one know which II to include in the model (i.e., how does one determine the best achievable II without running the HLS scheduler)? }

\REMARK{A major issue/question is whether the latency calculations consider different types of cross-iteration dependencies. None of the equations seem to include this aspect, yet it may significantly impact the unrolling/pipelining capabilities and, therefore, the latency bound. If this aspect is not included, the latencies could be over-optimistic (e.g., assuming that a loop that cannot be unrolled is unrolled, assuming a lower II than is actually possible). How does your approach account for data, memory, and control dependencies across loop iterations? }



\FIXME{Rewrite section 4 to make it more clear, by being really explicit concerning inter and intra dependencies (what they call cross iteration dep.)}
\FIXME{Add a small paragraph to explain how to compute the minimal II \textcolor{red}{DONE}}
\FIXME{Make it more clear concerning automatic optimisation of Vitis and that we take into account this}



% Our method is based on the fact that we calculate the lower bound of the different configurations. Thus, we prove in this section that we estimate the lower bound under some constraint.
%A theoretical lower bound allows us to stop the DSEs if the lower bound (cycles) of a design is higher than the best latency found so far. In this section we prove that we compute a lower bound.


We now outline key elements of our analytical performance model, and the associated proofs this model computes a lower bound on latency under resource constraints. Full proofs cover several pages, and are available in a separate research report: we limit below to summarizing the hypothesis and overall proof approach.

\subsection{Analytical Model Template}
\label{sec:analyticalModelTemplate}


Let $I^{\vec PV_i}_i(X)$ the operators defined as follows:
$$
I^{\vec PV_i}_i(X) = \lfloor II_i * (TC^{avg}_i - ispipelined_i) / (uf_i) \rfloor \odot X
$$
where $\odot$ is $+$ if $ispipelined_i = 1$, $*$ otherwise. We also have:

$
C_i^{\vec PV_i}(X_1, X_2, ..., X_n) = max(X_1, X_2, ..., X_n)~~~if~~~inparallel_i %pf_i + uf_i > 2
$

and

$
C_i^{\vec PV_i}(X_1, X_2, \dots, X_n) = \sum_{k=1}^n X_k~~~if~~~insequence_i 
%pf_i + uf_i = 2
$

with $inparallel_i = 1 = 1 - insequence_i$ if $(X_1, X_2, \dots, X_n)$  do not have dependencies (WaR, RaW, WaW) else 0.
Finally, $SL^{\vec PV_i}_i(\vec S_k)$ denotes a region of straight-line code (e.g., an inner-loop body). 
% which is used below in the formal reasoning on the bounds on latency of this template formula. 
Intuitively, $SL$ will represent a lower bound on the latency of a code block such that by composition across all loops as per the template formula, the result remains a lower bound on the full program latency. 

Given the summary AST of the program in constructor form, and the set of $\vec PV_i$ vectors for each loop, we build the analytical formula template as follows: (1) replace the $Loop_i(\vec X)$ operator by $I^{\vec PV_i}_i(\vec X)$ operator; (2) replace the $\vec X$ list by $C^{\vec PV_i}_i(\vec X)$; and (3) replace statement lists inside loop \texttt{i} $\vec S_x$ by $SL^{\vec PV_i}_i(\vec S_x)$. That is for our example, we simply rewrite:
$
Loop_i(Loop_{j1}(S1), Loop_{j2}(S2,S3))
$
into
$
I^{\vec PV_i}_i(C^{\vec PV_i}(I^{\vec PV_{j1}}_{j1}(SL^{\vec PV_{j1}}_{j1}(S1)), I^{\vec PV_{j2}}_{j2}(SL^{\vec PV_{j2}}_{j2}(S2,S3))))
$

% $$
% Loop_i(Loop_{j1}(S1), Loop_{j2}(S2,S3))
% $$
% into
% $$
% I^{\vec PV_i}_i(C^{\vec PV_i}(I^{\vec PV_{j1}}_{j1}(SL^{\vec PV_{j1}}_{j1}(S1)), I^{\vec PV_{j2}}_{j2}(SL^{\vec PV_{j2}}_{j2}(S2,S3))))
% $$

% \noindent Where we define the operators as follows:
% $$
% I^{\vec PV_i}_i(X) = \lfloor II_i * (TC^{avg}_i - ispipelined_i) / (pf_i * uf_i) \rfloor \odot X
% $$
% where $\odot$ is $+$ if $ispipelined_i = 1$, $*$ otherwise. We also have:

% $
% C_i^{\vec PV_i}(X_1, X_2, ..., X_n) = max(X_1, X_2, ..., X_n)~~~if~~~inparallel_i %pf_i + uf_i > 2
% $
% and
% $
% C_i^{\vec PV_i}(X_1, X_2, \dots, X_n) = \sum_{k=1}^n X_k~~~if~~~insequence_i 
% %pf_i + uf_i = 2
% $

% with $inparallel_i = 1 = 1 - insequence_i$ if $(X_1, X_2, \dots, X_n)$  do not have dependencies (WaR, RaW, WaW) else 0.
% Finally, $SL^{\vec PV_i}_i(\vec S_k)$ denotes a region of straight-line code (e.g., an inner-loop body). 
% % which is used below in the formal reasoning on the bounds on latency of this template formula. 
% Intuitively, $SL$ will represent a lower bound on the latency of a code block such that by composition across all loops as per the template formula, the result remains a lower bound on the full program latency. 


\subsection{Restrictions and Applicability}

Our objective is to formulate a lower bound on the latency of a program, after HLS. We therefore put several restrictions:
\begin{itemize}[leftmargin=*]
    \item The input program is a pure polyhedral program \cite{girbal06ijpp}, and its analysis (loop trip counts for every loop, all data dependences \cite{Fea91}) is exact.
    \item No HLS optimization shall change the number of operations in the computation: strength reduction, common sub-expression elimination, etc. shall either first be performed in the input program before analysis, or not be performed by the HLS toolchain.
    \item The program does not contain "useless" operations. A typical case is when a value is overwritten before being used, e.g. \texttt{x = 42+51; x = 0;}.
    \item We only model DSP and BRAM resources for the considered kernel, ignoring all other resources.
    \item We assume resource (DSP) sharing across different operations executing at the same cycle is not possible.
\end{itemize}


%on it: we assume the input program is a polyhedral program, that is the control-flow is statically analyzable; all loops can be recognized and their trip count computed; and all array / memory accesses can be exactly modeled at compile-time. No conditional can occur in the program. While our approach may generalize beyond this class, we limit it here to these strict assumptions.

%To maintain a lower bound on latency by composition, we operate on a representation of (parts of the) program which is both schedule-independent and storage-independent. Indeed, a lower bound on this representation is necessarily valid under any schedule and storage eventually implemented. \emph{We however require HLS to not change the count and type of operations}. Furthermore, for lower bounding purposes, we assume unless stated otherwise $\forall i,~inparallel_i = 1$. We will discuss in the next section a more realistic but compiler-dependent approach to set $inparallel_i$, based on dependence analysis.

%We assume programs are made of affine 
%% loops, that are loops with statically computable control-flow, with loop bounds made only of intersection of affine expressions of surrounding loop iterators and program constants. 
%loops. These are loops with a statically computable control-flow, with loop bounds made only of an intersection of affine expressions of surrounding loop iterators and program constants.
%% 
%We now assume loop bodies (i.e., statements surrounded by loops) have been translated to a list of statements, with at most a single operation (e.g., \texttt{+,-,/,*}) per statement. Operations are n-ary, that is they take $n \ge 0$ input scalar values as operand, and produce 0 or 1 output scalar value. A memory location can be loaded from (resp. stored to) an address stored in a scalar variable. 

\subsection{Latency Lower Bound}

% This is often referred to as straight-line code \cite{some-good-def}
% , define in the Definition \ref{def:straightlinecode}
% . This normalization of the loop body facilitates the computation of live-in/live-out data for the code block, 
% definine respectively in the Definitions \ref{def:livein, def:liveout}, 
% and the extraction of the computation graph. 

% Note the region can be represented in Static Single Assignment \cite{ssa} form, to ensure different storage location for every assignment, facilitating the construction of the operation graph.



% \begin{definition}[Straight-line code]
% \label{def:straightlinecode}
% An n-ary operation takes n scalar operands $\vec i$ as input, and produces a single scalar $o$ as output. A statement contains a single n-ary operation, or a load from (resp. store to) a memory location to (resp. from) a scalar. A straight-line code region $L$ is a list of consecutive statements, with a single entry and single exit.
% \end{definition}

% \begin{definition}[Live-in set] 
% \label{def:livein}
% The live-in set $V_I^L$ of region $L$ is the set of scalar values, variables and memory locations that read before being written, under any possible valid execution of $L$.
% \end{definition}

% \begin{definition}[Live-out set] 
% \label{def:liveout}
% The live-out set $V_O^L$ of region $L$ is the set of variables and memory locations that written to during any possible valid execution of $L$.
% \end{definition}

An important term is $SL$, a latency lower bound for a region of straight-line code. To maintain a lower bound on latency by composition, we operate on a representation of (parts of the) program which is both schedule-independent and storage-independent: the operation graph, or CDAG \cite{elango2015characterizing}. Indeed, a lower bound on this representation is necessarily valid under any schedule and storage eventually implemented, and can be used to prove I/O lower bounds on programs \cite{elango2015characterizing}. We compute the directed acyclic graph with one node per operation in the code region, connecting all producer and consumer operations to build the operation graph. Then, we can easily compute the length of its critical path, which represents the minimal set of operations to execute serially.


%\emph{We however require HLS to not change the count and type of operations}. Furthermore, for lower bounding purposes, we assume unless stated otherwise $\forall i,~inparallel_i = 1$. We will discuss in the next section a more realistic but compiler-dependent approach to set $inparallel_i$, based on dependence analysis.


% \cite{someothergoodref}
% defined in Definition \ref{def:computationgraph}
% .

% \begin{definition}[Operation Graph] 
 %\label{def:computationgraph}
 %Given a straight-line code region $R$ made of a list $L$ of statements $S \in L$, the operation graph OG is the directed graph $<\{N,V_I,root,V_O\},E>$ such that $\forall S_i \in L,~N_{S_i} \in N$; and for every operation with output $o$ and inputs $\vec i$ in $L$ $\forall S_i, \forall i_k \in \Vec{i}_{S_i}, e_{i_k, o} \in E$, $\forall S_i:(o_{S_i},{\vec i}_{S_i}) \in L, S_j:(o_{S_j},{\vec i}_{S_j}) \in L$ with $S_i \ne S_j$ then we have $E_{S_i,S_j} \in E$ iff $o_{Si}\cap{\vec i}_{S_j}\ne \emptyset$. For every input (resp. output) in $S_i$ which is not matched with an output (resp. input) of another $S_j$ in $L$, create a node $V_{val} \in V_I$ (resp. $V_O$) for this input (resp. output) value. If $dim({\vec i}_{S_i}) = 0$ then an edge $e_{root,S_i}$ is added to $E$.
% \end{definition}



% \cite{someone}
% , defined in Definition \ref{def:ogcriticalpath}
% .

% Let $OG$ the operation graph. %TODO

% \begin{definition}[Operation Graph critical path]
% \label{def:ogcriticalpath}
% Given $OG^L$ an operation graph for region $L$. Its critical path $OG_{cp}$ is the longest of all the shortest paths between every pairs $(v_i,v_o) \in <\{V_I,root\},V_O>$. 
% % Its length, in number of nodes, is noted $\#OG_{cp}^L$.
% Its length is noted $\#OG_{cp}^L$.
% \end{definition}



%\myparagraph{Estimating Latency}

% We can build a simple a lower bound on the latency of an operation graph:
% \begin{theorem}[Lower bound on latency of an Operation Graph]
% \label{def:latlbcp}
% Given infinite resources, and assuming no operation nor memory movement can take less than one cycle to complete, the latency $LAT_{cp}^L \ge \#OG_{cp}^L$ is a lower bound on the minimal feasible latency to execute $L$.
% \end{theorem}

% \begin{proof}[Proof Th \ref{def:latlbcp}]
% Every operation $S_i$ is associated at least one edge with a source in $<\{V_I,root\}>$, so there is a path between one of these nodes and every operation by construction in Def.~\ref{def:computationgraph}. For an operation to produce a useful output, there must be a path from its output to a node in $V_O$, otherwise the operation may be removed by dead code elimination. Therefore the shortest path $sp$ between a pair of node $(v_i, v_o) \in <\{V_I,root\},V_O>$ is the shortest sequence of operations in dependence that must be executed to produce $v_o$. As any operation takes at least one cycle to complete per Def.~\ref{def:latlbcp}, then this path must take at least $\#sp$ cycles to complete. As we take the largest of shortest paths between all possible pairs  $(v_i, v_o)$ then $OG_{cp}^L$ is the length of the longest shortest path to produce any output $v_o$ from some input, via a sequence of producer-consumer operations. Therefore it must take at least $\#OG_{cp}^L$ cycles to execute this path.
% \end{proof}


%\begin{proof}
%% probably have to show that if it was to take less cycles, then it would have to be because there is an operation taking less than 1 cycle?
%By definition the critical path is the longest path of all the shortest paths between every pairs of node $(v_i,v_o) \in <V_I,V_O>$ through the OG graph and the lower bound of the latency is the minimal number of cycles to perform all operations while respecting the dependencies.
%Suppose the critical path is not the lower bound then there is another path through the graph such that all operations are executed that is shorter than the critical path. Which is false by contradiction.
%Hence, the critical path is the lower bound.
%\end{proof}


We can then build a lower bound on the number of cycles a region $L$ may require to execute, under fixed resources, by simply taking the maximum between the weighted critical path and the work to execute normalized by the resources available.
% keep
\begin{theorem}[Latency Lower Bound under Operation Resource Constraints] 
\label{th:latlbresources}
Given $R_{op}$ a count of available resources of type $op$, for each operation type, $OG$ the operation graph, and $LO(op)$ the latency function for operation $op$, with $LO(op) \ge 1$. $\#L(op)$ denotes the number of operations of type $op$ in $L$. We define $LO(\#OG_{cp}^L) = \sum_{n \in cp} LO(n)$ the critical path weighted by latency of its operations.
The minimal latency of a region $L$ is bounded by 
$$
Lat_{R_{op}}^L \ge \max(LO(\#OG_{cp}^L),\max_{o \in op} (\lceil \#L(o) \times LO(o) /R_{o}\rceil))
$$
\end{theorem}

This theorem provides the building block to our analysis: if reasoning on a straight-line code region, without any loop, then building the operation graph for this region and reasoning on its critical path is sufficient to provide a latency lower bound. We now need to integrate loops, and enable composition of latency bounds.

%The intuition of the proof of the Theorem \ref{th:latlbresources} is that  if there is equal or more resources available than the work to execute, the length of the critical path weighted by latency is the minimal latency. In the case there are not enough resources available and the time to execute this work is higher than the critical path the minimal latency is $\lceil \#L(o) \times LO(o) /R_{o}\rceil$ for this operation.

% \begin{proof}[Proof Th \ref{def:latlbresources}]
% Suppose $\forall o \in op,~R_{o} \ge \#L(o) $. Then there is equal or more resources available than work to execute, this is equivalent to the infinite resource hypothesis of Def.~\ref{def:latlbcp}, the minimal latency is $LO(\#OG_{cp}^L)$.

% Suppose $\exists o \in op,~R_{o} < \#L(o)  $. Then there exists at least one unit in $R_{o}$ that is executing $\lceil \#L(o) /R_{o} \rceil$ operations. As every operation $op$ takes at $L(op) \ge 1$ cycle to complete, this unit will execute in at least  $\lceil \#L(o) \times L_{o}/R_{o} \rceil$ cycles. If $\lceil \#L(o) \times L_{o}/R_{o} \rceil \ge LO(\#OG_{cp}^L)$, the computation cannot execute in less than $\lceil \#L(o) \times L_{o}/R_{o} \rceil$ cycles.
% \end{proof}

% \FIXME{May here show an ILP formulation on the CDAG that achieves the lower bound, and reason that all are (over-)approximations of this perfect scheduling+placement solution?}



% \paragraph*{Loop Unrolling: full unroll}

% % We can bound the latency of a loop nest which has been entirely flatten, that is, all loops have been fully unrolled.

% We start by reasoning on the bound for latency of a loop nest which has been fully unrolled, e.g. as a result of \texttt{#pragma ACCEL parallel} or \texttt{#pragma HLS unroll}. full unrolling amounts to fully unrolling all $TC$ iterations of a loop, replacing the loop by $TC$ replications of its original loop body, where the loop iterator has been updated with the value it takes, for each replication.

% It follows a simple corollary:
% \begin{corollary}[Equivalence between fully unrolled and straight-line code]
% \label{cor:fullflattenstraightlinecode}
% Given a loop nest $l$, if full unrolling is applied to $l$ then the code obtained after full unrolling is a straight-line code as per Def.~\ref{def:straightlinecode}.
% \end{corollary}

% \begin{proof}[Proof Co \ref{cor:fullflattenstraightlinecode}]
% By construction the process of fully unrolling all the loops creates a straight-line code region without loop control, which therefore fits Def.~\ref{def:straightlinecode}.
% \end{proof}

% Consequently, we can bound the latency of a fully unrolled loop nest:
% \begin{theorem}[Minimal latency of a fully unrolled loop nest]
% \label{th:minlatflattenednest}
% Given a loop nest $l$, which is first rewritten by fully unrolling all loops to create a straight-line code region $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then its minimal latency is bounded by:
% $$
% Lat_{R_{op}}^l \ge \max(LO(\#OG_{cp}^L),\max_{o \in op} (\lceil \#L(o) \times L_{o}/R_{o} \rceil))
% $$
% \end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatflattenednest}]
% By Corollary~\ref{cor:fullflattenstraightlinecode}.
% \end{proof}

\myparagraph{Loop Unrolling} Loop unrolling is an HLS optimization that aims to execute multiple iterations of a loop in parallel. Intuitively, for an unroll factor $UF \ge 1$, $UF$ replications of the loop body will be instantiated. If $TC_l \mod UF_l \ne 0$ then an epilogue code to execute the remaining $TC_l \mod UF_l$ iterations is needed.



% \FIXME{NOTE: write here some comment on what happens if you unroll non-rectangular loops, loops where UF does not divide TC, etc. from the Merlin/Vitis implementation point of view.}

% bellow describe well enought
% If UF does not divide TC, then Merlin duplicates the sub loop body containing the loop which has a lower bound $lb_{original}$ and upper bound $ub_{original}$, using the corresponding loop of the first loop body with $lb=lb_{original}$ and $ub=x$ (where $x$ is the largest divisor of UF less or equal to $ub_{original}$) and the corresponding loop of the second loop body with $lb=x+1$ and $ub=ub_{original}$. 

Unrolling can be viewed as a two-step transformation: first strip-mine the loop by the unroll factor, then consider the inner loop obtained to be fully-unrolled. The latency of the resulting sub-program is determined by how the outer-loop generated will be implemented. 
We assume without additional explicit information this unrolled loop will execute in a non-pipelined, non-parallel fashion, to provide the following bound:

% keep
\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF]
\label{th:minlatpartunrolled}
Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^'$ the loop body obtained by replicating $UF$ times the original loop body $L$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor * Lat_{R_{op}}^{L^'}
$$    
\end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatpartunrolled}]
% By construction and Theorem~\ref{def:latlbresources}, $Lat_{R_{op}}^L'$ is a lower bound on the latency of $L'$, that is the sub-program made of $UF$ iterations of the loop. $\lfloor TC/UF \rfloor \ge TC_l/UF$ is a lower bound on the number of iterations of the loop. As we assume a non-pipelined execution for the resulting outer loop, every iteration shall start after the completion of the preceding one, that is its iteration latency, itself bounded by $Lat_{R_{op}}^L'$.
% \end{proof}

Note this bound requires to build the operation graph for the whole loop body. This is straightforward for inner loops and/or fully unrolled loop nests, but impractical if the loop body contains other loops. We therefore define a weaker, but more practical, bound \emph{that enables composition}:

%\FIXME{Need to precise that we use DSA. And cite Feautrier papier for transformation Affine -> DSA}
% keep
\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF and complex loop bodies]
\label{th:minlatpartunrolledcomplex}
Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor * Lat_{R_{op}}^L
$$    
\end{theorem}


The intuition of the proof of Theorem \ref{th:minlatpartunrolledcomplex} is that there cannot exist a shorter critical path in the operation graph of the \emph{unrolled} loop nest than in the non-unrolled loop body, that is there is no useless operation. This is therefore essential to require the absence of useless operations in the program, as otherwise a shorter critical path may be exposed after loop unrolling, making this theorem incorrect.

% \begin{proof}[Proof Th \ref{th:minlatpartunrolledcomplex}]
% % Suppose $Lat_{R_{op}}^L > Lat_{R_{op}}^L'$. If $UF=1$, then $L=L'$, a contradiction. 

% % If $TC_l > UF > 1$ then OG^L'


% % necessarily $\forall op, L(op) \le L'(op)$ 

% % If $UF=TC$, this correspond to the case of Theorem \ref{}

% % If $UF=1$, this corresponds to the case of Theorem \ref{def:loopIteratedSequentially} where the loop is neither pipelined nor parallelized.

% Key argument to prove: style of: lat(S1,forloop) >= max(lat(S1),lat(forloop) that is by adding a new instruction we dont reduce the cp length. A counter example is
% \{for i:  a = a+b\};a = 43


% if we consider a CDAG, adding the edge a = 43 gives a shorter path to a than any of the i iteration in the fully unrolled cdag. So we must add conditions such as writes to the same location have to be all executed, in the order of the original code (sensible condition in presence of data dependences WAW).

% Proof flow:
% 1) Given $OG^{i}$ and $OG^j$ two CDAGs, for a pair of distinct iterations $i,j$ of loop $L$. If $V_O^i \cap V_O^j = \emptyset$, then the graph $OG^{i,j}$ made of the two iterations $i,j$ cannot have a smaller critical path length than $OG^{i}$ and $OG^j$: there is no edge crossing $OG^{i}$ and $OG^j$ in $OG^{i,j}$ since outputs are distincts, therfore $Lat(OG^{i,j} \ge \max(Lat(OG^i),Lat(OG^j))$.

% 2) Suppose now  $V_O^i \cap V_O^j \ne \emptyset$. Then iterations $i$ and $j$ produce at least one output in common. IDEA: DSA. If the program is in dynamic single assignent form, this is a contradiction (DSA: only 1 write per location). Need to adjust defs at start to be in DSA form? Mention automatic conversion from affine to DSA exists (Feautrier, 90s).







% %\FIXME{Need to precise that we use DSA. And cite Feautrier papier for transformation Affine -> DSA}

% \end{proof}

% \FIXME{The above theorem covers the composition case of C operator, with children made of loops with a bound and statements. Perhaps worth rewriting the theorem (or a corrollary) to show this composition of children is valid? That would conclude the formulas with the pipelining below.}

% Vitis allows to do a reduction with a tree reduction in logarithmic time with the option ``unsafe-math''. 

% \begin{theorem}[Minimal latency of a partially unrolled loop with factor UF for reduction loop with tree reduction]
% \label{th:minlatunrolled}
% Given a reduction loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$, if executed in a non-pipelined fashion and the tree reduction is legal is bounded by:
% $$
% Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^L \times \lfloor \log_2(UF)  \rfloor
% $$    
% \end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatunrolled}]

    
%     By definition a reduction loop is a loop with a dependency distance of 1. Hence, at each iteration the same memory cell is read and write. 

%     1) Because of the dependency distance of 1, only one element can be add to the same memory cell.
%     2) Each data can be add independently two by two and the result of this independent addition can also be add two by two until we obtained one value. It is a tree of depth $\log_2(UF)$.
    
%     3) The depth of the tree is $\log_2(UF)$ and each node at the same depth can be execute independently in $Lat_{R_{op}}^L$ cycles.
    
% \end{proof}


\myparagraph{Loop pipelining} Loop pipelining amounts to overlapping multiple iterations of the loop, so that the next iteration can start prior to the completion of the preceding one. The initiation interval (II) measures in cycles the delay between the start of two consecutive iterations, it is easy to prove our formula template accurately integrates the latency of pipelined loops with the $I$ operator.


In practice we compute the minimal II in function of the dependencies of the loop pipelined and the iteration latency of the operations of the statements. 
% 
Let $RecMII$ and $ResMII$ which are respectively the recurrence constrained and the resource constraint of the loop pipelined and we have $II \geq \max{(ResMII, RecMII)}$. 
% 
The resource constraint 
$ResMII = \max_i \lceil \frac{uses(r_i)}{count(r_i)} \rceil$ with $uses(r)$ the number of time the resource $r$ is used in 1 iteration and $count(r)$ the number of resource of type $r$
and
$RecMII = \max_i \lceil \frac{ delay(c_i)}{ distance(c_i)} \rceil$ with $delay(c_i)$ the total latency in dependency cycle $c_i$ and $distance(c_i)$ the total distance in dependency cycle $c_i$.
As we cannot compute accurately $ResMII$ as we don't know how the ressource will be used by the compiler we suppose that $ResMII=1$, hence we keep a lower bound on $II$.
% 
Hence, if the loop is a reduction loop then the $II \geq IL_{reduction}$ with $\frac{IL_{reduction}}{1}$ the iteration latency of the operation of reduction.
We thus take the minimum II possible. 



% It follows a bound on the minimal latency of a pipelined loop:
% \begin{theorem}[Minimal latency of a pipelined loop with known II]
% \label{th:minlatpipeline}
% Given a loop $l$ with trip count $TC_l$ and loop body $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$ if executed in a pipelined fashion is bounded by:
% $$
% Lat_{R_{op}}^{l,P} \ge Lat_{R_{op}}^L + II *( TC_l - 1)
% $$    
% \end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatpipeline}]
% $Lat_{R_{op}}^L$ is the minimal latency to complete one iteration of $l$ by Theorem~\ref{def:latlbresources}. The initiation interval measures the number of elapsed cycles before the next iteration can start, it takes therefore at least $TC_l * II - 1$ to start $TC_l - 1$ iterations, irrespective of their completion time. Therefore the latency of the loop is at least the latency of one iteration to complete, and for all iterations to be started.
% \end{proof}


% \paragraph*{Non-Parallel, Non-Pipelined Loops}

% We conclude by a trivial case: if the loop is not optimized by any directive (including any automatically inserted by the compilers), that is is not parallelized nor pipelined, then every next iteration of the loop starts only after the end of the prior iteration.

% \begin{definition}[Lower bound on latency of a non-parallel, non-pipelined loop under resources constraints]
% \label{def:loopIteratedSequentially}
% Given a loop $l$ with trip count $TC_l$ which is neither pipelined nor parallelized, that is, iteration $i+1$ starts after the full completion of iteration $i$, for all iterations. Given $Lat_{R_{op}}^L$ the minimal latency of its loop body. Then
% $$
% Lat_{R_{op}}^l \ge TC_l * Lat_{R_{op}}^L
% $$

% \end{definition}



\myparagraph{Program latency lower bound} 
% \begin{definition}[Statement]
% A statement is a basic unit of computation in a program that performs a specific operation. A statement can either be a single n-ary operation or a load from/store to a memory location. An n-ary operation takes n scalar operands as input and produces a single scalar output. A load operation reads a scalar value from a memory location, and a store operation writes a scalar value to a memory location. A straight-line code region $L$ is a list of consecutive statements, with a single entry and single exit, where each statement in $L$ is either an n-ary operation or a load from/store to a memory location.
% \end{definition}
% \begin{definition}[Configuration of Pragma]
% \end{definition}
We now focus on having the program latency lower bound, with resource constraints. This bound takes into account the limitations imposed by available resources, which can significantly affect the achievable performance.
% 
We assume here that the resources consumed are only consumed by the computing units and resource use by the computational unit of one operation can not be reused by the computational unit of an other operation executing at the same time. We also assume that the compilers have implemented the pragma configuration given as input.
% We consider two extreme cases for the resource DSPs. Knowing that the resources actually used will be between these two bounds for a fixed pragma configuration: 
% 1. A design generation without any reuse i.e. the computation units used by the operation of a statement cannot be reused by another statement.
% 2. A design generation with a perfect reuse i.e. that the computation units for the same operation can be reused as soon as the computation unit is not used. As reminder we consider statement with only one operation, if it was not the case we must have to consider intra statement reuse.

% We consider  for the resource DSPs. Knowing that the resources actually used will be between these two bounds for a fixed pragma configuration: 

For DSPs we suppose we have a perfect reuse i.e., that the computation units for the same operation can be reused as soon as the computation unit is not in use. Under-estimating the resources used is fundamental to proving the latency lower bound, as otherwise another design that consumes less resource than predicted may be feasible, itself possibly leading to a better latency. 
 % As reminder we consider statement with only one operation, if it was not the case we must have to consider intra-statement reuse.



% \begin{proof}[Proof Th \ref{th:minresource}]
    



% Assuming perfect intra- and inter-statement resource reuse, if the formula used to compute the required resources is wrong, and we can use fewer resources at any given time $t$, then the following cases can arise:

% Let suppose the formula is wrong, hence the reuse is not perfect which is in contradiction with our hypothesis.


% % 1. If no resources have been used until time $t$, then we are required to use the minimum number of computational units necessary for executing the operations in parallel, which corresponds to $DSP_{op} \times UF$.

% % 2. If all resources are available for reuse at time $t$, then the number of resources used at time $t$ will be less than or equal to the resources already used.

% % 3. If the number of computational units necessary for the computation at time $t$ exceeds the number of available resources already used and available, we reuse the maximum number of unused resources, plus the difference in new resources required to complete the computation. There are three possible cases:

% % 3.1. If two statements are under the same unrolled loop, then we only count one computation unit per operation for all the statements under the loop(s) unrolled.

% % 3.2. If two statements are not under the same unrolled loop, then when the second statement is executed, all the resources consumed by the first statement will be freed and can be reused.

% % 3.3. If a loop is pipelined and the II (initiation interval) is not as expected, we still use the minimum number of DSPs due to the intra-statement resource reuse, i.e., the minimal number of DSPs will be independent of the II.
% % In all cases, the number of DSPs used is minimal.


    
% \end{proof}




% \begin{theorem}[Maximal resource consumption]
% \label{th:maxresource}


% Given a loop body $L$,  statements $\mathcal{S}$ and  the configuration of pragma which is constitute of  UFs of each loop and the list of loops pipelined. 


% Assuming that resources are exclusively used by the operations in different statements, the maximum number of resources (DSPs) utilized by region $L$ can be computed as the sum, for each operation and statement, of the number of DSPs used by that operation in that statement.



% This correspond to:
% $$
% R^{max}_{used} =  \sum_{op} \sum_{S \in \mathcal{S}}
% % ( \min(1,\#L_{op}^{S}) 
% \#L_{op}^S 
% \times DSP_{op} 
% \times UF^{S}
% $$    

% % with $\#L_{op}^t$ the number of operation $op$ in parallel at time $t$ and $DSP_{op}$ the number of resource (DSPs) used for the operation $op$.

% with
% $\#L_{op}^S$ the number of operation $op$ for the statements $S$, $DSP_{op}$ the number of resource (DSPs) used for the operation $op$ and $UF^S$ the number of duplication of the statement $S$.



% % $$
% % R^{max}_{used} = \ge \sum_{S \in \mathcal{S}} \sum_{op}\max_{t}( \#L_{op}^{S,t}) \times DSP_{op} 
% % $$    
% % with $\#L_{op}$ the number of operation $op$ in parallel  and $\mathcal{S}$ the set of statements.

% \end{theorem}

% \begin{proof}[Proof Th \ref{th:maxresource}]
% % est ce que c'est pas se compliquer la vie ?

% Here we suppose we don't have reuse inter and intra-statement. Hence, if one statement need to do two additions, the two additions will used different computational unit and these computational units will not be used for other statement.

% As we sum all the resource used per operation per statement we have to prove that:

% 1. The same operation for the same statement can't used more resource than $DSP_{op}$. And we have as hypothesis than the operation $op$ used $DSP_{op}$.

% 2. If more parallelism the number of DSP will be greater. However, we know the configuration as input and hence know the parallelism of the kernel.



% % Problem if UF does not divide TC  => False Problem because if Merlin transform we know the code

    
% \end{proof}

% \begin{theorem}[Lower Bound under resource constraint]
% \label{th:minlatpipeline}
% Given a loop body $L$,  statements $\mathcal{S}$ and  the configuration of pragma which is constitute of  UFs of each loop and the list of loops pipelined. 


% On the condition that the resources are only used by the operations of the different statements.


% The lower bound $lb$ can not be achieve under resource constraint if 
% $$
% R_{op} < 
% \sum_{op} \max_{S \in \mathcal{S}_{par}}
% % ( \min(1,\#L_{op}^{S}) 
% \mathbf{1}_{\#L_{op}^S \geq 1}
% \times DSP_{op} 
% \times UF^{S})
% $$    


% The lower bound $lb$ can be achieve under resource constraint if 
% $$
% R_{op} \ge 
% \sum_{op} \sum_{S \in \mathcal{S}}
% % ( \min(1,\#L_{op}^{S}) 
% \#L_{op}^S 
% \times DSP_{op} 
% \times UF^{S}
% % \sum_{S \in \mathcal{S}} \sum_{op}\max_{t}( \#L_{op}^{S,t}) \times DSP_{op} 
% $$    

% with $\mathbf{1}$ the indicator function which is equal to $1$ if the number of operation in the statement is greater or equal to 1 i.e. if there is no operation then the number of DSP is 0 if we have more than one operation we considerate reuse intra statement,
% $\#L_{op}^S$ the number of operation $op$ in parallel for the statements $S$ which are under the same loop unrolled, $DSP_{op}$ the number of resource (DSPs) used for the operation $op$ and $\mathcal{S}_{par}$ the set of set statements which are under the same unrolled loop.

% \end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatpipeline}]
% We compute the resource used for two cases:

% \begin{itemize}
%     \item Perfect Reuse, which is intra and inter statement. If a resource is not use at time $t$, then it can be reuse for the same operation.
%     \item No reuse, i.e. each statement use different resource.
% \end{itemize}


% In the first case (perfect reuse), it is impossible to consume less resource, as proof in Theorem \ref{th:minresource}. In the second case, it is impossible to consume more resource, as proof in Theorem \ref{th:maxresource}. Hence, if a loop body $L$ 
% has a minimum of resource consumption greater than resource available
% the loop body can not be synthesized and run on this board. Hence the lower bound can not be achieve.

% In other way if a loop body $L$, has a maximal amount of resource lesser than resource available the design can be synthetized and run on this board. The lower bound can be achieve.

% If in practice at least one pragma is not applied as expected, then we have an other configuration with it is own lower bound.

% % If the hypothesis of reuse is wrong hence the resource consumed is greater than the one computed and the resource used are greater than resource available.
% \end{proof}

The lower bound of a kernel is therefore the lower bound of the configuration such that the minimal resource consumption is less than or equal to the resource available.
% keep

\begin{theorem}[Lower bound of the kernel under resource constraint]
\label{th:minlatpipelineunderresourceconstraint}
% Given a kernel, available resource $R_{op}$, the set of statements $\mathcal{S}$ and all the configuration of pragmas which are constitute of  the vectors $\Vec{PV_i}$ for each loop.
Given a loop body $L$,  the set of statements $\mathcal{S}$,
$\#L_{op}^s$ the number of operation $op$  for the statements $s$, $DSP_{op}$ the number of resources (DSPs) used for the operation $op$, $MCU_{op}^{s}$ the maximal computational unit the statement $s$ can use in parallel  and  the configuration of pragma which is constitute of  the vectors $\Vec{PV_i}$ for each loop.




% The minimal number of resource (DSPs) consumed, $R^{min}_{used}$, by $L$ for the pragma configuration  is the sum, for each operation, of the maximum number of DSPs used in parallel by a statement.


% This correspond to:
% $$
% R^{min}_{used} =  \sum_{op} \max_{s \in \mathcal{S}}(
% \#L_{op}^s
% \times DSP_{op} 
% \times MCU_{op}^{s})
% $$   

The configuration of pragma, which has the minimal lower bound and which respect $R_{used}^{min} = \sum_{op} \max_{s \in \mathcal{S}}(
\#L_{op}^s
\times DSP_{op} 
\times MCU_{op}^{s}) \leq R_{op}$, is the lower bound of the kernel.


\end{theorem}


The intuition of the proof of the Theorem \ref{th:minlatpartunrolledcomplex} is that $R_{used}^{min}$ is the minimal resource the kernel can used for the configuration of pragma. This implies that if the $R_{used}^{min} > R_{op}$ the configuration over-utilizes resource. Hence, the lowest lower bound which does not over-utilize the resource is the lower bound of the kernel.
% \begin{proof}[Proof Th \ref{th:minlatpipelineunderresourceconstraint}]

%     According to Theorem \ref{th:minresource}, $R_{used}^min$ is the minimal number of DSP a configuration can use. Hence, all configuration which does not respect the constraint $R_{used}^min \leq R_{op}$ have a over-utilization of the resource and hence are invalid.

%     Hence, the minimal lower bound of each configuration of pragma is the lower bound of the kernel.
    
% \end{proof}

%   

==> sources/theoretical_and_modeling2.tex <==
\label{sec:theoretical}

% \REMARK{Details of the approach are difficult to follow. It is not clear whether the latency bound calculation (one of the main contributions) 
% includes all relevant program information (i.e., cross-iteration dependencies). The approach is limited to a particular HLS flow (Merlin) 
% and a particular type of applications (affine loops).}

% \REMARK{The analytical model (Section 4A) is unclear}

% \REMARK{ The discussion of the latency lower bound is clear in the basic situations, but the discussion of the latency in the presence of pipelining is minimal. This situation is, probably, the most interesting: how does one know which II to include in the model (i.e., how does one determine the best achievable II without running the HLS scheduler)? }

% \REMARK{A major issue/question is whether the latency calculations consider different types of cross-iteration dependencies. None of the equations seem to include this aspect, yet it may significantly impact the unrolling/pipelining capabilities and, therefore, the latency bound. If this aspect is not included, the latencies could be over-optimistic (e.g., assuming that a loop that cannot be unrolled is unrolled, assuming a lower II than is actually possible). How does your approach account for data, memory, and control dependencies across loop iterations? }



% \FIXME{Rewrite section 4 to make it more clear, by being really explicit concerning inter and intra dependencies (what they call cross iteration dep.)}
% \FIXME{Add a small paragraph to explain how to compute the minimal II \textcolor{red}{DONE}}
% \FIXME{Make it more clear concerning automatic optimisation of Vitis and that we take into account this}



% \FIXME{APPENDIX or complementary ?}

We now outline key elements of our analytical performance model, and the associated proofs this model computes a lower bound on latency under resource constraints. 
Full proofs cover several pages, and are available in the Appendix
% Full proofs are available in the Appendix
% \ref{sec:appendix}
: we limit below to summarizing the hypothesis and overall proof approach.


\subsection{Analytical Model Template}
\label{sec:analyticalModelTemplate2}

We take as input the summary AST of the program in constructor form, and the set of $\vec PV_i$ vectors for each loop, as defined in Sec.~\ref{subsec:programrepresentation}. Returning to our example in Sec. \ref{subsec:programrepresentation}, this summary AST, capturing the loop structure and all statements, is $Loop_i(Loop_{j1}(S1), Loop_{j2}(S2,S3))$.


Let $I^{\vec{PV_i}}_i( X)$ be an operator that computes the latency of a region of a code represented by $ X$, where $X$ is composed of loops and/or statements. This function is computed as follows:
$
I^{\vec{PV_i}}_i(X) = \lfloor II_i * (TC^{avg}_i / uf_i - pip_i)  \rfloor \odot X
$
where $\odot$ is $+$ if the loop $i$ is pipelined ($pip_i = 1$), $\times$ otherwise. 
% 
Let $C_i^{\vec{PV_i}}( X_1, ...,  X_n)$ the operators which composed the region, defined as follows:
$
C_i^{\vec{PV_i}}(X_1, ..., X_n)$ is  $max_{i=1}^N(X_i)$ if there is no dependency (WaR, RaW, WaW) between the statements of the regions
and
$
 \sum_{i=1}^n X_i$ 
between the statements which have at least one dependency.
% 
Finally, $SL^{\vec{PV_i}}_i(\vec{S_k})$ denotes a region of straight-line code (e.g., an inner-loop body). 
Intuitively, $SL$ will represent a lower bound on the latency of a code block such 
that, by the composition
across all loops as per the template formula, the result remains a lower bound on the full program latency. 

We build the analytical formula template by simple substitution of the operators in the summary AST by the following operators: 
(1) for every $Loop_i(\vec X)$, replace it  by $I^{\vec PV_i}_i(\vec X)$ ; 
(2) for every list $\vec I$ containing the $I^{\vec PV_i}_i(\vec X)$ of the step 1,
replace it by $C^{\vec{PV_i}}_i(\vec I)$; and 
(3) replace statement lists inside loop \texttt{i} $\vec S_x$ by $SL^{\vec{PV_i}}_i(\vec S_x)$. That is for our example, we simply rewrite:
$
Loop_i(Loop_{j1}(S1), Loop_{j2}(S2,S3))
$
into the following formula:

$I^{\vec PV_i}_i(C^{\vec PV_i}(I^{\vec PV_{j1}}_{j1}(SL^{\vec PV_{j1}}_{j1}(S1)), I^{\vec PV_{j2}}_{j2}(SL^{\vec PV_{j2}}_{j2}(S2,S3))))
$




% 
% 
%%% LNP: I don't see the point/value of this example. It's talking about dependence analysis? IMHO the point of having an example was to illustrate the values I, C, SL, etc. take from the prototype formula, but when applied to this particular kernel. Given space is at a premium I advise commenting out. If not, replace the text below the example by the formula for the lb of that kernel. It may be relevant to put it towards the end of that section then, when terms have been introduced.
% 
%% \vspace{-0.4cm}
%\begin{lstlisting}[label={lst:reference_bicg},caption=Bicg]
%L1: for (i = 0; i < N; i++)  S0: s[i] = 0;
%L2: for (i = 0; i < M; i++) { S1: q[i] = 0;
%  L3: for (j = 0; j < N; j++) {
%    S2: s[j]+=r[i]*A[i][j]; S3: q[i]+=A[i][j]*p[j];}}
%\end{lstlisting}
%% \vspace{0.4cm}
% 
%In Listing \ref{lst:reference_bicg}, there is no dependency between $S2$ and $S3$, allowing these two statements to run concurrently. Consequently, the latency is determined by the longer of the two statement's latencies. However, there is a dependency between $S1$ and $S3$, necessitating the completion of $S1(i)$ before initiating the computation of $S3(i) $. In such cases, the latencies of these two statements are added together.
% 
% 





\subsection{Restrictions and Applicability}

Our objective is to formulate a lower bound on the latency of a program, after HLS. We therefore include several restrictions:
\begin{itemize}[leftmargin=*]
    \item The input program is a pure polyhedral program \cite{girbal06ijpp}, and its analysis (loop trip counts for every loop, all data dependencies \cite{Fea91}) is exact.
    \item No HLS optimization shall change the number of operations in the computation: strength reduction, common sub-expression elimination, etc., shall either first be performed in the input program before analysis, or not be performed by the HLS toolchain.
    \item The program does not contain "useless" operations. A typical case is when a value is overwritten before being utilized, e.g., \texttt{x = 42+51; x = 0;}.
    \item We only model DSP and BRAM resources for the considered kernel, ignoring all other resources.
    \item We assume resources (DSP) sharing across different operations executing at the same cycle is not possible.
\end{itemize}



\subsection{Latency Lower Bound}







An important term is $SL$, a latency lower bound for a region of straight-line code. To maintain a lower bound on latency by composition, we operate on a representation of (parts of the) program which is both schedule-independent and storage-independent: the operation graph, or CDAG \cite{elango2015characterizing}. Indeed, a lower bound on this representation is necessarily valid under any schedule and storage eventually implemented and can be used to prove I/O lower bounds on programs \cite{elango2015characterizing} which is the directed acyclic graph with one node per operation in the code region, connecting all producer and consumer operations to build the operation graph. Then, we can easily compute the length of its critical path, which represents the minimal set of operations to execute serially.




Then, we can build a lower bound on the number of cycles a region $L$ may require to execute, under fixed resources, by simply taking the maximum between the weighted critical path and the work to execute normalized by the resources available.
% keep

% \vspace{-0.15cm}
\begin{theorem}[Latency Lower Bound under Operation Resource Constraints] 
\label{th:latlbresources}
Given $\mathcal{O}$ the set of operation type
and $R_{o}$ a count of available resources of type $o \in \mathcal{O}$, $OG$ the operation graph, $cp_L$ the critical path of $OG$, and $LO(o)$ the latency function for operation $o$, with $LO(o) \ge 1$. 
% $\#L(s)$ 
$N_o^L$
denotes the number of operations of type $o$ in $L$. We define $C_L = \sum_{n \in cp_L} LO(n)$ the critical path  of $L$  weighted by latency of its operations.
The minimal latency of a region $L$ is bounded by 
$$
Lat_{R_{o}}^L \ge \max(C_L,\max_{o \in \mathcal{O}} (\lceil N_o^L \times LO(o) /R_{o}\rceil))
$$
\end{theorem}
% \vspace{-0.15cm}

This theorem provides the building block to our analysis: if reasoning on a straight-line code region, without any loop, then building the operation graph for this region and reasoning on its critical path is sufficient to provide a latency lower bound. 


% In Listing \ref{lst:reference_bicg}, if we take as example the sub-loop body constitute of the loops L3 and the statement $S2$ and $S3$ as a strainght-line code regions i.e.  L3 is fully unrolled. The critical path for $S2$ is $cp_{S2} = \max(L(+) + L(*), N \times (DSP_+ + DSP_*) / R_o)$ and for $S3$ is 
% $cp_{S3} = \max(L(+) \times \log(N) + L(*), N \times (DSP_+ + DSP_*) / R_o)$ by considering the possibility to do a tree reduction. So the critical path of this sub-loop body is $\max(cp_{S2}, cp_{S3})$.
% \vspace{-.4cm}
\begin{lstlisting}[label={lst:reference_bicg},caption=Bicg]
L1: for (i = 0; i < N; i++)  
    S0: s[i] = 0;
L2: for (i = 0; i < M; i++) { 
        S1: q[i] = 0;
    L3: for (j = 0; j < N; j++) {
        S2: s[j]+=r[i]*A[i][j]; 
        S3: q[i]+=A[i][j]*p[j];
    }
}
\end{lstlisting}
\vspace{.5cm}
For example in Listing~\ref{lst:reference_bicg}, if we consider the sub-loop body composed of loops L3 (fully unrolled) and the statements $S2$ and $S3$ as straight-line code regions, we can calculate the critical paths for $S2$ and $S3$ as follows:
% 
For $S2$, the critical path is given by: $cp_{S2} = \max(L(+) + L(*), N \times (DSP_+ + DSP_*) / R_o)$ with $DSP_{o}$ the number of DSP for the operation $o$.
For $S3$, the critical path is determined by: $cp_{S3} = \max(L(+) \times \log(N) + L(*), N \times (DSP_+ + DSP_*) / R_o)$,  considering the possibility of a tree reduction.
In this context, the critical path for the entire sub-loop body is the maximum of these two individual critical paths, expressed as $\max(cp_{S2}, cp_{S3})$.

We now need to integrate loops and enable composition of latency bounds.

\myparagraph{Loop Unrolling} Loop unrolling is an HLS optimization that aims to execute multiple iterations of a loop in parallel. Intuitively, for an unroll factor $UF \ge 1$, $UF$ replications of the loop body will be instantiated. If $TC_l \mod UF_l \ne 0$ then an epilogue code to execute the remaining $TC_l \mod UF_l$ iterations is needed.


%%%%%%%% Here comment to reduce section %%%%%%%%%%%
% Unrolling can be viewed as a two-step transformation: first strip-mine the loop by the unroll factor, then consider the inner loop obtained to be fully-unrolled. The latency of the resulting sub-program is determined by how the outer-loop generated will be implemented. 
% We assume without additional explicit information this unrolled loop will execute in a non-pipelined, non-parallel fashion, to provide the following bound:


% \begin{theorem}[Minimal latency of a partially unrolled loop with factor UF]
% \label{th:minlatpartunrolled}
% Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L^'$ the loop body obtained by replicating $UF$ times the original loop body $L$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
% $$
% Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor * Lat_{R_{op}}^{L^'}
% $$    
% \end{theorem}


% Note this bound requires to build the operation graph for the whole loop body. This is straightforward for inner loops and/or fully unrolled loop nests, but impractical if the loop body contains other loops. We therefore define a weaker, but more practical, bound \emph{that enables composition}:

Unrolling can be viewed as a two-step transformation: first strip-mine the loop by the unroll factor, then consider the inner loop obtained to be fully-unrolled. The latency of the resulting sub-program is determined by how the outer-loop generated will be implemented. 
We assume without additional explicit information this unrolled loop will execute in a non-pipelined, non-parallel fashion.
Note this bound requires to build the operation graph for the whole loop body. This is straightforward for inner loops and/or fully unrolled loop nests, but impractical if the loop body contains other loops. We therefore define a weaker, but more practical, bound \emph{that enables composition}:

% \vspace{-0.15cm}
\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF and complex loop bodies]
\label{th:minlatpartunrolledcomplex}
Given a loop $l$ with trip count $TC_l$ and loop body $L$,  unroll factor $UF \le TC$ and $\mathcal{O}$ the set of operation type. Given available resources $R_{o}$ and latencies $L(o) \ge 1$ with $o \in \mathcal{O}$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{o}}^{l,S} \ge \lfloor TC/UF \rfloor * Lat_{R_{o}}^L
$$    
\end{theorem}
% \vspace{-0.15cm}

The intuition of the proof of Theorem \ref{th:minlatpartunrolledcomplex} is that there cannot exist a shorter critical path in the operation graph of the \emph{unrolled} loop nest than in the non-unrolled loop body, that is there is no useless operation. This is therefore essential to require the absence of useless operations in the program, as otherwise a shorter critical path may be exposed after loop unrolling, making this theorem incorrect.

% \FIXME{finish example}

% Let take the example of the loop $L0$, unrolled by a factor $UF \leq TC_{L0}$ with $TC_{L0}$ the trip count of the loop $L0$ and the statement $S0$ on Listing \ref{lst:reference_bicg} with the latency of one iteration of $S0$ equal to $Lat^{S0}_{R_{op}} > 0$, the lower bound of the latency without pipeline is $\lceil TC_{L0} / UF \rceil \times Lat^{S0}_{R_{op}}$.

Consider the scenario of loop $L0$ within Listing \ref{lst:reference_bicg}, which has been unrolled by a factor denoted as $UF \leq TC_{L0}$ where $TC_{L0}$ is the trip count of $L0$. The latency for one iteration of $S0$ is denoted as $Lat^{S0}_{R_{o}} > 0$.
In the absence of pipelining, the lower bound of the latency of this sub-loop body is: $\lfloor TC_{L0} / UF \rfloor \times Lat^{S0}_{R_{o}}$.

% \begin{proof}[Proof Th \ref{th:minlatpartunrolledcomplex}]
% % Suppose $Lat_{R_{op}}^L > Lat_{R_{op}}^L'$. If $UF=1$, then $L=L'$, a contradiction. 

% % If $TC_l > UF > 1$ then OG^L'


% % necessarily $\forall op, L(op) \le L'(op)$ 

% % If $UF=TC$, this correspond to the case of Theorem \ref{}

% % If $UF=1$, this corresponds to the case of Theorem \ref{def:loopIteratedSequentially} where the loop is neither pipelined nor parallelized.

% Key argument to prove: style of: lat(S1,forloop) >= max(lat(S1),lat(forloop) that is by adding a new instruction we dont reduce the cp length. A counter example is
% \{for i:  a = a+b\};a = 43


% if we consider a CDAG, adding the edge a = 43 gives a shorter path to a than any of the i iteration in the fully unrolled cdag. So we must add conditions such as writes to the same location have to be all executed, in the order of the original code (sensible condition in presence of data dependences WAW).

% Proof flow:
% 1) Given $OG^{i}$ and $OG^j$ two CDAGs, for a pair of distinct iterations $i,j$ of loop $L$. If $V_O^i \cap V_O^j = \emptyset$, then the graph $OG^{i,j}$ made of the two iterations $i,j$ cannot have a smaller critical path length than $OG^{i}$ and $OG^j$: there is no edge crossing $OG^{i}$ and $OG^j$ in $OG^{i,j}$ since outputs are distincts, therfore $Lat(OG^{i,j} \ge \max(Lat(OG^i),Lat(OG^j))$.

% 2) Suppose now  $V_O^i \cap V_O^j \ne \emptyset$. Then iterations $i$ and $j$ produce at least one output in common. IDEA: DSA. If the program is in dynamic single assignent form, this is a contradiction (DSA: only 1 write per location). Need to adjust defs at start to be in DSA form? Mention automatic conversion from affine to DSA exists (Feautrier, 90s).







% %\FIXME{Need to precise that we use DSA. And cite Feautrier papier for transformation Affine -> DSA}

% \end{proof}

% \FIXME{The above theorem covers the composition case of C operator, with children made of loops with a bound and statements. Perhaps worth rewriting the theorem (or a corrollary) to show this composition of children is valid? That would conclude the formulas with the pipelining below.}

% Vitis allows to do a reduction with a tree reduction in logarithmic time with the option ``unsafe-math''. 

% \begin{theorem}[Minimal latency of a partially unrolled loop with factor UF for reduction loop with tree reduction]
% \label{th:minlatunrolled}
% Given a reduction loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$, if executed in a non-pipelined fashion and the tree reduction is legal is bounded by:
% $$
% Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^L \times \lfloor \log_2(UF)  \rfloor
% $$    
% \end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatunrolled}]

    
%     By definition a reduction loop is a loop with a dependency distance of 1. Hence, at each iteration the same memory cell is read and write. 

%     1) Because of the dependency distance of 1, only one element can be add to the same memory cell.
%     2) Each data can be add independently two by two and the result of this independent addition can also be add two by two until we obtained one value. It is a tree of depth $\log_2(UF)$.
    
%     3) The depth of the tree is $\log_2(UF)$ and each node at the same depth can be execute independently in $Lat_{R_{op}}^L$ cycles.
    
% \end{proof}


\myparagraph{Loop pipelining} 

Loop pipelining amounts to overlapping multiple iterations of the loop, so that the next iteration can start prior to the completion of the preceding one. The initiation interval (II) measures in cycles the delay between the start of two consecutive iterations. It is easy to prove our formula template accurately integrates the latency of pipelined loops with the $I$ operator.
% 
We compute the minimal II in function of the dependencies of the pipelined loop and the iteration latency of the operations of the statements during the NLP generation. 
% 
Let $RecMII$ and $ResMII$ be the recurrence constraints and the resource constraints of the pipelined loop, respectively. We have $II \geq \max{(ResMII, RecMII)}$. 
% 
$RecMII = \max_i \lceil \frac{ delay(c_i)}{ distance(c_i)} \rceil$ with $delay(c_i)$ the total latency in dependency cycle $c_i$ and $distance(c_i)$ the total distance in dependency cycle $c_i$.
% As we cannot compute accurately $ResMII$ as we don't know how the resource will be used by the compiler 
We suppose that $ResMII=1$, as we don't know how the resource will be used by the compiler.
% 
Hence, if the loop is a reduction loop then the $II \geq \frac{IL_{reduction}}{1}$ with $IL_{reduction}$ the iteration latency of the operation of reduction. For a kernel like $for (j = 0; j < N; j++) y[j] = y[j-2] + 3;$ the $II \geq \lceil \frac{IL_+}{2} \rceil$.



\myparagraph{Program latency lower bound} 

We now focus on having the program latency lower bound, with resource constraints. This bound takes into account the limitations imposed by available resources, which can significantly affect the achievable performance.
% 
We assume here that the resources consumed are only consumed by the computing units and resource use by the computational unit of one operation can not be reused by the computational unit of another operation executing at the same time. We also assume that the compilers have implemented the pragma configuration given as input.
% We consider two extreme cases for the resource DSPs. Knowing that the resources actually used will be between these two bounds for a fixed pragma configuration: 
% 1. A design generation without any reuse i.e. the computation units used by the operation of a statement cannot be reused by another statement.
% 2. A design generation with a perfect reuse i.e. that the computation units for the same operation can be reused as soon as the computation unit is not used. As reminder we consider statement with only one operation, if it was not the case we must have to consider intra statement reuse.

% We consider  for the resource DSPs. Knowing that the resources actually used will be between these two bounds for a fixed pragma configuration: 

For DSPs we suppose we have a perfect reuse, i.e., that the computation units for the same operation can be reused as soon as the computation unit is not in use. Under-estimating the resources used is fundamental to proving the latency lower bound, as otherwise another design that consumes less resources than predicted may be feasible, itself possibly leading to a better latency. 
% 
The lower bound of a kernel is therefore the lower bound of the configuration such that the minimal resource consumption is less than or equal to the resource available.
% keep
% \vspace{-0.15cm}
\begin{theorem}[Lower bound of the kernel under resource constraint]
\label{th:minlatpipelineunderresourceconstraint2}
% Given a kernel, available resource $R_{op}$, the set of statements $\mathcal{S}$ and all the configuration of pragmas which are constitute of  the vectors $\Vec{PV_i}$ for each loop.
Given a loop body $L$,  the set of statements $\mathcal{S}$, $\mathcal{O}$ the set of operation type,
$N_{o}^s$ the number of operations $o \in \mathcal{O}$  for the statements $s$, $DSP_{o}$ the number of resources (DSPs) used for the operation $o \in \mathcal{O}$, $MCU_{o}^{s}$ the maximal computational unit the statement $s$ can use in parallel  and  the configuration of pragma which is constituted of the vectors $\Vec{PV_i}$ for each loop.
% 
The configuration of pragma, which has the minimal lower bound and which respect $R_{used}^{min} = \sum_{o} \max_{s \in \mathcal{S}}(
N_{o}^s
\times DSP_{o} 
\times MCU_{o}^{s}) \leq R_{o}$, is the lower bound of the kernel.


\end{theorem}
% \vspace{-0.14cm}

The intuition of the proof of the Theorem \ref{th:minlatpipelineunderresourceconstraint2} is that $R_{used}^{min}$ is the minimal resource that the kernel can use for the configuration of pragma. This implies that if the $R_{used}^{min} > R_{o}$ the configuration over-utilizes resources. Hence, the lowest lower bound which does not over-utilize the resource is the lower bound of the kernel.


==> sources/theoretical_and_modeling_old.tex <==
\label{sec:theoretical}


We now give a proof of the theoretical lower bound. We can found all the proof in Appendix \ref{sec:appendixA}.

\subsection{Analytical Model Template}
\label{sec:analyticalModelTemplate}
Given the summary AST of the program in constructor form, and the set of $\vec PV_i$ vectors for each loop, we build the analytical formula template as follows: (1) replace the $Loop_i(\vec X)$ operator by $I^{\vec PV_i}_i(\vec X)$ operator; (2) replace the $\vec X$ list by $C^{\vec PV_i}_i(\vec X)$; and (3) replace statement lists inside loop \texttt{i} $\vec S_x$ by $SL^{\vec PV_i}_i(\vec S_x)$. That is for the example in Listing \ref{lst:reference}, we simply rewrite:
$
Loop_i(Loop_{j1}(S1), Loop_{j2}(S2,S3))
$
into
$
I^{\vec PV_i}_i(C^{\vec PV_i}(I^{\vec PV_{j1}}_{j1}(SL^{\vec PV_{j1}}_{j1}(S1)), I^{\vec PV_{j2}}_{j2}(SL^{\vec PV_{j2}}_{j2}(S2,S3))))
$

% $$
% Loop_i(Loop_{j1}(S1), Loop_{j2}(S2,S3))
% $$
% into
% $$
% I^{\vec PV_i}_i(C^{\vec PV_i}(I^{\vec PV_{j1}}_{j1}(SL^{\vec PV_{j1}}_{j1}(S1)), I^{\vec PV_{j2}}_{j2}(SL^{\vec PV_{j2}}_{j2}(S2,S3))))
% $$

\noindent Where we define the operators as follows:
$$
I^{\vec PV_i}_i(X) = \lfloor II_i * (TC^{avg}_i - ispipelined_i) / (pf_i * uf_i) \rfloor \odot X
$$
where $\odot$ is $+$ if $ispipelined_i = 1$, $*$ otherwise. We have also:

$
C_i^{\vec PV_i}(X_1, X_2, ..., X_n) = max(X_1, X_2, ..., X_n)~~~if~~~inparallel_i %pf_i + uf_i > 2
$
and
$
C_i^{\vec PV_i}(X_1, X_2, \dots, X_n) = \sum_{k=1}^n X_k~~~if~~~insequence_i 
%pf_i + uf_i = 2
$
% 
% 
% $$
% C_i^{\vec PV_i}(X_1, X_2, ..., X_n) = max(X_1, X_2, ..., X_n)~~~if~~~inparallel_i %pf_i + uf_i > 2
% $$
% and
% $$
% C_i^{\vec PV_i}(X_1, X_2, \dots, X_n) = \sum_{k=1}^n X_k~~~if~~~insequence_i 
% %pf_i + uf_i = 2
% $$
% \FIXME{LNP: properly define inparallel and insequence}
% 
with $inparallel_i = 1 = 1 - insequence_i$ if $(X_1, X_2, \dots, X_n)$  do not have dependencies (WaR, RaW, WaW) else 0.

Finally, $SL^{\vec PV_i}_i(\vec S_k)$ denotes a region of straight-line code, which is used below in the formal reasoning on the bounds on latency of this template formula. Intuitively, $SL$ will represent a lower bound on the latency of the code block such that by composition across all loops as per the template formula, the result remains a lower bound on the full program latency. 


\subsection{A Formal Model for Latency}

Our objective is to formulate a lower bound on the latency of a program after HLS. We therefore have put several restrictions: we assume the input program is a polyhedral program, that is the control-flow is statically analyzable; all loops can be recognized and their trip count computed; and all array / memory accesses can be exactly modeled at compile-time. No conditional can occur in the program. While our approach may generalize beyond this class, we limit here to these strict assumptions.

To maintain a lower bound on latency by composition, we operate on a representation of (parts of the) program which is both schedule-independent and storage-independent: indeed, a lower bound on this representation is necessarily valid under any schedule and storage eventually implemented. \emph{We however require HLS to not change the count and type of operations}. Furthermore, for lower bounding purposes, we assume unless stated otherwise $\forall i,~inparallel_i = 1$. We will discuss in the next section a more realistic but compiler-dependent approach to set $inparallel_i$, based on dependence analysis.

We assume programs are made of affine loops, that are loops with statically computable control-flow, with loop bounds made only of intersection of affine expressions of surrounding loop iterators and program constants. We now assume loop bodies (i.e., statements surrounded by loops) have been translated to a list of statements, with at most a single operation (e.g., \texttt{+,-,/,*}) per statement. Operations are n-ary, that is they take $n \ge 0$ input scalar values as operand, and produce 0 or 1 output scalar value. A memory location can be loaded from (resp. stored to) an address stored in a scalar variable. This is often referred to as straight-line code \cite{some-good-def}
% , define in the Definition \ref{def:straightlinecode}
. This normalization of the loop body facilitates the computation of live-in/live-out data for the code block, 
% definine respectively in the Definitions \ref{def:livein, def:liveout}, 
and the extraction of the computation graph. Note the region can be represented in Static Single Assignment \cite{ssa} form, to ensure different storage location for every assignment, facilitating the construction of the operation graph.



\begin{definition}[Straight-line code]
\label{def:straightlinecode}
An n-ary operation takes n scalar operands $\vec i$ as input, and produces a single scalar $o$ as output. A statement contains a single n-ary operation, or a load from (resp. store to) a memory location to (resp. from) a scalar. A straight-line code region $L$ is a list of consecutive statements, with a single entry and single exit.
\end{definition}

\begin{definition}[Live-in set] 
\label{def:livein}
The live-in set $V_I^L$ of region $L$ is the set of scalar values, variables and memory locations that read before being written, under any possible valid execution of $L$.
\end{definition}

\begin{definition}[Live-out set] 
\label{def:liveout}
The live-out set $V_O^L$ of region $L$ is the set of variables and memory locations that written to during any possible valid execution of $L$.
\end{definition}

We can compute the directed acyclic graph made of all statements (i.e., all n-ary operations), connecting all producer and consumer operations, to build the operation graph \cite{someothergoodref}
% defined in Definition \ref{def:computationgraph}
.

\begin{definition}[Operation Graph] 
\label{def:computationgraph}
Given a straight-line code region $R$ made of a list $L$ of statements $S \in L$, the operation graph OG is the directed graph $<\{N,V_I,root,V_O\},E>$ such that $\forall S_i \in L,~N_{S_i} \in N$; and for every operation with output $o$ and inputs $\vec i$ in $L$ $\forall S_i, \forall i_k \in \Vec{i}_{S_i}, e_{i_k, o} \in E$,
$\forall S_i:(o_{S_i},{\vec i}_{S_i}) \in L, S_j:(o_{S_j},{\vec i}_{S_j}) \in L$ with $S_i \ne S_j$ then we have $E_{S_i,S_j} \in E$ iff $o_{Si}\cap{\vec i}_{S_j}\ne \emptyset$. For every input (resp. output) in $S_i$ which is not matched with an output (resp. input) of another $S_j$ in $L$, create a node $V_{val} \in V_I$ (resp. $V_O$) for this input (resp. output) value. If $dim({\vec i}_{S_i}) = 0$ then an edge $e_{root,S_i}$ is added to $E$.
\end{definition}

From this representation, we can easily define key properties to subsequently estimate the latency and area of this code region, such as its span, or critical path \cite{someone}
% , defined in Definition \ref{def:ogcriticalpath}
.

\begin{definition}[Operation Graph critical path]
\label{def:ogcriticalpath}
Given $OG^L$ an operation graph for region $L$. Its critical path $OG_{cp}$ is the longest of all the shortest paths between every pairs $(v_i,v_o) \in <\{V_I,root\},V_O>$. 
% Its length, in number of nodes, is noted $\#OG_{cp}^L$.
Its length is noted $\#OG_{cp}^L$.
\end{definition}



\paragraph*{Estimating Latency}

We can build a simple a lower bound on the latency of an operation graph:
\begin{theorem}[Lower bound on latency of an Operation Graph]
\label{def:latlbcp}
Given infinite resources, and assuming no operation nor memory movement can take less than one cycle to complete, the latency $LAT_{cp}^L \ge \#OG_{cp}^L$ is a lower bound on the minimal feasible latency to execute $L$.
\end{theorem}

% \begin{proof}[Proof Th \ref{def:latlbcp}]
% Every operation $S_i$ is associated at least one edge with a source in $<\{V_I,root\}>$, so there is a path between one of these nodes and every operation by construction in Def.~\ref{def:computationgraph}. For an operation to produce a useful output, there must be a path from its output to a node in $V_O$, otherwise the operation may be removed by dead code elimination. Therefore the shortest path $sp$ between a pair of node $(v_i, v_o) \in <\{V_I,root\},V_O>$ is the shortest sequence of operations in dependence that must be executed to produce $v_o$. As any operation takes at least one cycle to complete per Def.~\ref{def:latlbcp}, then this path must take at least $\#sp$ cycles to complete. As we take the largest of shortest paths between all possible pairs  $(v_i, v_o)$ then $OG_{cp}^L$ is the length of the longest shortest path to produce any output $v_o$ from some input, via a sequence of producer-consumer operations. Therefore it must take at least $\#OG_{cp}^L$ cycles to execute this path.
% \end{proof}


%\begin{proof}
%% probably have to show that if it was to take less cycles, then it would have to be because there is an operation taking less than 1 cycle?
%By definition the critical path is the longest path of all the shortest paths between every pairs of node $(v_i,v_o) \in <V_I,V_O>$ through the OG graph and the lower bound of the latency is the minimal number of cycles to perform all operations while respecting the dependencies.
%Suppose the critical path is not the lower bound then there is another path through the graph such that all operations are executed that is shorter than the critical path. Which is false by contradiction.
%Hence, the critical path is the lower bound.
%\end{proof}


We can then build a tighter lower bound on the number of cycles a region $L$ may take to execute, under fixed resources, by simply taking the maximum between the weighted span and the work to execute normalized by the resources available.

\begin{theorem}[Latency Lower Bound under Operation Resource Constraints] 
\label{def:latlbresources}
Given $R_{op}$ a count of available resources of type $op$, for each operation type, and $LO(op)$ the latency function for operation $op$, with $LO(op) \ge 1$. $\#L(op)$ denotes the number of operations of type $op$ in $L$. We define $LO(\#OG_{cp}^L) = \sum_{n \in cp} LO(n)$ the critical path weighted by latency of its operations.
The minimal latency of a region $L$ is bounded by 
$$
Lat_{R_{op}}^L \ge \max(LO(\#OG_{cp}^L),\max_{o \in op} (\lceil \#L(o) \times LO(o) /R_{o}\rceil))
$$
\end{theorem}

% \begin{proof}[Proof Th \ref{def:latlbresources}]
% Suppose $\forall o \in op,~R_{o} \ge \#L(o) $. Then there is equal or more resources available than work to execute, this is equivalent to the infinite resource hypothesis of Def.~\ref{def:latlbcp}, the minimal latency is $LO(\#OG_{cp}^L)$.

% Suppose $\exists o \in op,~R_{o} < \#L(o)  $. Then there exists at least one unit in $R_{o}$ that is executing $\lceil \#L(o) /R_{o} \rceil$ operations. As every operation $op$ takes at $L(op) \ge 1$ cycle to complete, this unit will execute in at least  $\lceil \#L(o) \times L_{o}/R_{o} \rceil$ cycles. If $\lceil \#L(o) \times L_{o}/R_{o} \rceil \ge LO(\#OG_{cp}^L)$, the computation cannot execute in less than $\lceil \#L(o) \times L_{o}/R_{o} \rceil$ cycles.
% \end{proof}

% \FIXME{May here show an ILP formulation on the CDAG that achieves the lower bound, and reason that all are (over-)approximations of this perfect scheduling+placement solution?}



\paragraph*{Loop Unrolling: full unroll}

% We can bound the latency of a loop nest which has been entirely flatten, that is, all loops have been fully unrolled.

We start by reasoning on the bound for latency of a loop nest which has been fully unrolled, e.g. as a result of \texttt{#pragma ACCEL parallel} or \texttt{#pragma HLS unroll}. full unrolling amounts to fully unrolling all $TC$ iterations of a loop, replacing the loop by $TC$ replications of its original loop body, where the loop iterator has been updated with the value it takes, for each replication.

It follows a simple corollary:
\begin{corollary}[Equivalence between fully unrolled and straight-line code]
\label{cor:fullflattenstraightlinecode}
Given a loop nest $l$, if full unrolling is applied to $l$ then the code obtained after full unrolling is a straight-line code as per Def.~\ref{def:straightlinecode}.
\end{corollary}

% \begin{proof}[Proof Co \ref{cor:fullflattenstraightlinecode}]
% By construction the process of fully unrolling all the loops creates a straight-line code region without loop control, which therefore fits Def.~\ref{def:straightlinecode}.
% \end{proof}

Consequently, we can bound the latency of a fully unrolled loop nest:
\begin{theorem}[Minimal latency of a fully unrolled loop nest]
\label{th:minlatflattenednest}
Given a loop nest $l$, which is first rewritten by fully unrolling all loops to create a straight-line code region $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then its minimal latency is bounded by:
$$
Lat_{R_{op}}^l \ge \max(LO(\#OG_{cp}^L),\max_{o \in op} (\lceil \#L(o) \times L_{o}/R_{o} \rceil))
$$
\end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatflattenednest}]
% By Corollary~\ref{cor:fullflattenstraightlinecode}.
% \end{proof}

\paragraph*{Loop Unrolling: partial unroll} Loop unrolling is a HLS optimization that aims to execute multiple iterations of a loop in parallel. Intuitively, for an unroll factor $UF \ge 1$, $UF$ replications of the loop body will be instantiated. If $TC_l \mod UF_l \ne 0$ then an epilogue code to execute the remaining $TC_l \mod UF_l$ iterations is needed.



% \FIXME{NOTE: write here some comment on what happens if you unroll non-rectangular loops, loops where UF does not divide TC, etc. from the Merlin/Vitis implementation point of view.}

If UF does not divide TC, then Merlin duplicates the sub loop body containing the loop which has a lower bound $lb_{original}$ and upper bound $ub_{original}$, using the corresponding loop of the first loop body with $lb=lb_{original}$ and $ub=x$ (where $x$ is the largest divisor of UF less or equal to $ub_{original}$) and the corresponding loop of the second loop body with $lb=x+1$ and $ub=ub_{original}$. 

Partial unrolling can be viewed as a two-step transformation: first strip-mine the loop by the unroll factor, then consider the inner loop obtained is fully-unrolled. The latency of the resulting sub-program is determined by how the outer-loop generated will be implemented. We assume without additional explicit information this outer loop will execute in a non-pipelined, non-parallel fashion, to provide the following bound:

\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF]
\label{th:minlatpartunrolled}
Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Given $L'$ the loop body obtained by replicating $UF$ times the original loop body $L$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor * Lat_{R_{op}}^L'
$$    
\end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatpartunrolled}]
% By construction and Theorem~\ref{def:latlbresources}, $Lat_{R_{op}}^L'$ is a lower bound on the latency of $L'$, that is the sub-program made of $UF$ iterations of the loop. $\lfloor TC/UF \rfloor \ge TC_l/UF$ is a lower bound on the number of iterations of the loop. As we assume a non-pipelined execution for the resulting outer loop, every iteration shall start after the completion of the preceding one, that is its iteration latency, itself bounded by $Lat_{R_{op}}^L'$.
% \end{proof}

Note this bound requires to build the operation graph for the whole loop body. This is straightforward for inner loops and/or fully unrolled loop nests, but impractical if the loop body contains other loops. We therefore define a weaker, but more practical, bound:

%\FIXME{Need to precise that we use DSA. And cite Feautrier papier for transformation Affine -> DSA}

\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF and complex loop bodies]
\label{th:minlatpartunrolledcomplex}
Given a loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$ if executed in a non-pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor * Lat_{R_{op}}^L
$$    
\end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatpartunrolledcomplex}]
% % Suppose $Lat_{R_{op}}^L > Lat_{R_{op}}^L'$. If $UF=1$, then $L=L'$, a contradiction. 

% % If $TC_l > UF > 1$ then OG^L'


% % necessarily $\forall op, L(op) \le L'(op)$ 

% % If $UF=TC$, this correspond to the case of Theorem \ref{}

% % If $UF=1$, this corresponds to the case of Theorem \ref{def:loopIteratedSequentially} where the loop is neither pipelined nor parallelized.

% Key argument to prove: style of: lat(S1,forloop) >= max(lat(S1),lat(forloop) that is by adding a new instruction we dont reduce the cp length. A counter example is
% \{for i:  a = a+b\};a = 43


% if we consider a CDAG, adding the edge a = 43 gives a shorter path to a than any of the i iteration in the fully unrolled cdag. So we must add conditions such as writes to the same location have to be all executed, in the order of the original code (sensible condition in presence of data dependences WAW).

% Proof flow:
% 1) Given $OG^{i}$ and $OG^j$ two CDAGs, for a pair of distinct iterations $i,j$ of loop $L$. If $V_O^i \cap V_O^j = \emptyset$, then the graph $OG^{i,j}$ made of the two iterations $i,j$ cannot have a smaller critical path length than $OG^{i}$ and $OG^j$: there is no edge crossing $OG^{i}$ and $OG^j$ in $OG^{i,j}$ since outputs are distincts, therfore $Lat(OG^{i,j} \ge \max(Lat(OG^i),Lat(OG^j))$.

% 2) Suppose now  $V_O^i \cap V_O^j \ne \emptyset$. Then iterations $i$ and $j$ produce at least one output in common. IDEA: DSA. If the program is in dynamic single assignent form, this is a contradiction (DSA: only 1 write per location). Need to adjust defs at start to be in DSA form? Mention automatic conversion from affine to DSA exists (Feautrier, 90s).







% %\FIXME{Need to precise that we use DSA. And cite Feautrier papier for transformation Affine -> DSA}

% \end{proof}

% \FIXME{The above theorem covers the composition case of C operator, with children made of loops with a bound and statements. Perhaps worth rewriting the theorem (or a corrollary) to show this composition of children is valid? That would conclude the formulas with the pipelining below.}

Vitis allows to do a reduction with a tree reduction in logarithmic time with the option ``unsafe-math''. 

\begin{theorem}[Minimal latency of a partially unrolled loop with factor UF for reduction loop with tree reduction]
\label{th:minlatunrolled}
Given a reduction loop $l$ with trip count $TC_l$ and loop body $L$, and unroll factor $UF \le TC$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$, if executed in a non-pipelined fashion and the tree reduction is legal is bounded by:
$$
Lat_{R_{op}}^{l,S} \ge \lfloor TC/UF \rfloor \times Lat_{R_{op}}^L \times \lfloor \log_2(UF)  \rfloor
$$    
\end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatunrolled}]

    
%     By definition a reduction loop is a loop with a dependency distance of 1. Hence, at each iteration the same memory cell is read and write. 

%     1) Because of the dependency distance of 1, only one element can be add to the same memory cell.
%     2) Each data can be add independently two by two and the result of this independent addition can also be add two by two until we obtained one value. It is a tree of depth $\log_2(UF)$.
    
%     3) The depth of the tree is $\log_2(UF)$ and each node at the same depth can be execute independently in $Lat_{R_{op}}^L$ cycles.
    
% \end{proof}


\paragraph*{Loop pipelining} Loop pipelining amounts to overlapping multiple iterations of the loop, so that the next iteration can start prior to the completion of the preceding one. The initiation interval (II) measures in cycles the delay between the start of two consecutive iterations. 

It follows a bound on the minimal latency of a pipelined loop:
\begin{theorem}[Minimal latency of a pipelined loop with known II]
\label{th:minlatpipeline}
Given a loop $l$ with trip count $TC_l$ and loop body $L$. Given available resources $R_{op}$ and latencies $L(op) \ge 1$. Then the minimal latency of $l$ if executed in a pipelined fashion is bounded by:
$$
Lat_{R_{op}}^{l,P} \ge Lat_{R_{op}}^L + II *( TC_l - 1)
$$    
\end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatpipeline}]
% $Lat_{R_{op}}^L$ is the minimal latency to complete one iteration of $l$ by Theorem~\ref{def:latlbresources}. The initiation interval measures the number of elapsed cycles before the next iteration can start, it takes therefore at least $TC_l * II - 1$ to start $TC_l - 1$ iterations, irrespective of their completion time. Therefore the latency of the loop is at least the latency of one iteration to complete, and for all iterations to be started.
% \end{proof}


\paragraph*{Non-Parallel, Non-Pipelined Loops}

We conclude by a trivial case: if the loop is not optimized by any directive (including any automatically inserted by the compilers), that is is not parallelized nor pipelined, then every next iteration of the loop starts only after the end of the prior iteration.

\begin{definition}[Lower bound on latency of a non-parallel, non-pipelined loop under resources constraints]
\label{def:loopIteratedSequentially}
Given a loop $l$ with trip count $TC_l$ which is neither pipelined nor parallelized, that is, iteration $i+1$ starts after the full completion of iteration $i$, for all iterations. Given $Lat_{R_{op}}^L$ the minimal latency of its loop body. Then
$$
Lat_{R_{op}}^l \ge TC_l * Lat_{R_{op}}^L
$$

\end{definition}



\paragraph*{Latency under resource constraint} 

% \begin{definition}[Statement]
% A statement is a basic unit of computation in a program that performs a specific operation. A statement can either be a single n-ary operation or a load from/store to a memory location. An n-ary operation takes n scalar operands as input and produces a single scalar output. A load operation reads a scalar value from a memory location, and a store operation writes a scalar value to a memory location. A straight-line code region $L$ is a list of consecutive statements, with a single entry and single exit, where each statement in $L$ is either an n-ary operation or a load from/store to a memory location.
% \end{definition}

% \begin{definition}[Configuration of Pragma]

% \end{definition}

We now focus on proving the lower bound with resource constraints. This proof takes into account the limitations imposed by available resources, which can significantly affect the achievable performance.
% 
We assume here that the resources consumed are only consumed by the computing units and resource use by the computational unit of one operation can not be reuse by the computational unit of another operation. We also assume that the compilers have implemented the pragma's configuration given as input.
% We consider two extreme cases for the resource DSPs. Knowing that the resources actually used will be between these two bounds for a fixed pragma configuration: 
% 1. A design generation without any reuse i.e. the computation units used by the operation of a statement cannot be reused by another statement.
% 2. A design generation with a perfect reuse i.e. that the computation units for the same operation can be reused as soon as the computation unit is not used. As reminder we consider statement with only one operation, if it was not the case we must have to consider intra statement reuse.

% We consider  for the resource DSPs. Knowing that the resources actually used will be between these two bounds for a fixed pragma configuration: 

For the resource of DSPs we suppose we have a perfect reuse i.e.
 that the computation units for the same operation can be reused as soon as the computation unit is not used. As reminder we consider statement with only one operation, if it was not the case we must have to consider intra-statement reuse.

\begin{theorem}[Minimal resource consumption]
\label{th:minresource}
Given a loop body $L$,  the set of statements $\mathcal{S}$,
$\#L_{op}^s$ the number of operation $op$  for the statements $s$, $DSP_{op}$ the number of resource (DSPs) used for the operation $op$, $MCU_{op}^{s}$ the maximal computational unit the statement $s$ can use in parallel  and  the configuration of pragma which is constitute of  the vectors $\Vec{PV_i}$ for each loop.



The minimal number of resource (DSPs) consumed, $R^{min}_{used}$, by $L$ for the pragma configuration  is the sum, for each operation, of the maximum number of DSPs used in parallel by a statement.


This correspond to:
$$
R^{min}_{used} =  \sum_{op} \max_{s \in \mathcal{S}}(
\#L_{op}^s
\times DSP_{op} 
\times MCU_{op}^{s})
$$    

\end{theorem}

% \begin{proof}[Proof Th \ref{th:minresource}]
    



% Assuming perfect intra- and inter-statement resource reuse, if the formula used to compute the required resources is wrong, and we can use fewer resources at any given time $t$, then the following cases can arise:

% Let suppose the formula is wrong, hence the reuse is not perfect which is in contradiction with our hypothesis.


% % 1. If no resources have been used until time $t$, then we are required to use the minimum number of computational units necessary for executing the operations in parallel, which corresponds to $DSP_{op} \times UF$.

% % 2. If all resources are available for reuse at time $t$, then the number of resources used at time $t$ will be less than or equal to the resources already used.

% % 3. If the number of computational units necessary for the computation at time $t$ exceeds the number of available resources already used and available, we reuse the maximum number of unused resources, plus the difference in new resources required to complete the computation. There are three possible cases:

% % 3.1. If two statements are under the same unrolled loop, then we only count one computation unit per operation for all the statements under the loop(s) unrolled.

% % 3.2. If two statements are not under the same unrolled loop, then when the second statement is executed, all the resources consumed by the first statement will be freed and can be reused.

% % 3.3. If a loop is pipelined and the II (initiation interval) is not as expected, we still use the minimum number of DSPs due to the intra-statement resource reuse, i.e., the minimal number of DSPs will be independent of the II.
% % In all cases, the number of DSPs used is minimal.


    
% \end{proof}




% \begin{theorem}[Maximal resource consumption]
% \label{th:maxresource}


% Given a loop body $L$,  statements $\mathcal{S}$ and  the configuration of pragma which is constitute of  UFs of each loop and the list of loops pipelined. 


% Assuming that resources are exclusively used by the operations in different statements, the maximum number of resources (DSPs) utilized by region $L$ can be computed as the sum, for each operation and statement, of the number of DSPs used by that operation in that statement.



% This correspond to:
% $$
% R^{max}_{used} =  \sum_{op} \sum_{S \in \mathcal{S}}
% % ( \min(1,\#L_{op}^{S}) 
% \#L_{op}^S 
% \times DSP_{op} 
% \times UF^{S}
% $$    

% % with $\#L_{op}^t$ the number of operation $op$ in parallel at time $t$ and $DSP_{op}$ the number of resource (DSPs) used for the operation $op$.

% with
% $\#L_{op}^S$ the number of operation $op$ for the statements $S$, $DSP_{op}$ the number of resource (DSPs) used for the operation $op$ and $UF^S$ the number of duplication of the statement $S$.



% % $$
% % R^{max}_{used} = \ge \sum_{S \in \mathcal{S}} \sum_{op}\max_{t}( \#L_{op}^{S,t}) \times DSP_{op} 
% % $$    
% % with $\#L_{op}$ the number of operation $op$ in parallel  and $\mathcal{S}$ the set of statements.

% \end{theorem}

% \begin{proof}[Proof Th \ref{th:maxresource}]
% % est ce que c'est pas se compliquer la vie ?

% Here we suppose we don't have reuse inter and intra-statement. Hence, if one statement need to do two additions, the two additions will used different computational unit and these computational units will not be used for other statement.

% As we sum all the resource used per operation per statement we have to prove that:

% 1. The same operation for the same statement can't used more resource than $DSP_{op}$. And we have as hypothesis than the operation $op$ used $DSP_{op}$.

% 2. If more parallelism the number of DSP will be greater. However, we know the configuration as input and hence know the parallelism of the kernel.



% % Problem if UF does not divide TC  => False Problem because if Merlin transform we know the code

    
% \end{proof}

% \begin{theorem}[Lower Bound under resource constraint]
% \label{th:minlatpipeline}
% Given a loop body $L$,  statements $\mathcal{S}$ and  the configuration of pragma which is constitute of  UFs of each loop and the list of loops pipelined. 


% On the condition that the resources are only used by the operations of the different statements.


% The lower bound $lb$ can not be achieve under resource constraint if 
% $$
% R_{op} < 
% \sum_{op} \max_{S \in \mathcal{S}_{par}}
% % ( \min(1,\#L_{op}^{S}) 
% \mathbf{1}_{\#L_{op}^S \geq 1}
% \times DSP_{op} 
% \times UF^{S})
% $$    


% The lower bound $lb$ can be achieve under resource constraint if 
% $$
% R_{op} \ge 
% \sum_{op} \sum_{S \in \mathcal{S}}
% % ( \min(1,\#L_{op}^{S}) 
% \#L_{op}^S 
% \times DSP_{op} 
% \times UF^{S}
% % \sum_{S \in \mathcal{S}} \sum_{op}\max_{t}( \#L_{op}^{S,t}) \times DSP_{op} 
% $$    

% with $\mathbf{1}$ the indicator function which is equal to $1$ if the number of operation in the statement is greater or equal to 1 i.e. if there is no operation then the number of DSP is 0 if we have more than one operation we considerate reuse intra statement,
% $\#L_{op}^S$ the number of operation $op$ in parallel for the statements $S$ which are under the same loop unrolled, $DSP_{op}$ the number of resource (DSPs) used for the operation $op$ and $\mathcal{S}_{par}$ the set of set statements which are under the same unrolled loop.

% \end{theorem}

% \begin{proof}[Proof Th \ref{th:minlatpipeline}]
% We compute the resource used for two cases:

% \begin{itemize}
%     \item Perfect Reuse, which is intra and inter statement. If a resource is not use at time $t$, then it can be reuse for the same operation.
%     \item No reuse, i.e. each statement use different resource.
% \end{itemize}


% In the first case (perfect reuse), it is impossible to consume less resource, as proof in Theorem \ref{th:minresource}. In the second case, it is impossible to consume more resource, as proof in Theorem \ref{th:maxresource}. Hence, if a loop body $L$ 
% has a minimum of resource consumption greater than resource available
% the loop body can not be synthesized and run on this board. Hence the lower bound can not be achieve.

% In other way if a loop body $L$, has a maximal amount of resource lesser than resource available the design can be synthetized and run on this board. The lower bound can be achieve.

% If in practice at least one pragma is not applied as expected, then we have an other configuration with it is own lower bound.

% % If the hypothesis of reuse is wrong hence the resource consumed is greater than the one computed and the resource used are greater than resource available.
% \end{proof}

The lower bound of a kernel is therefore the lower bound of the configuration such that the minimal resource consumption is less or equal than the resource available.

\begin{theorem}[Lower bound of the kernel under resource constraint]
\label{th:minlatpipelineunderresourceconstraint}
Given a kernel, available resource $R_{op}$, the set of statements $\mathcal{S}$ and all the configuration of pragmas which are constitute of  the vectors $\Vec{PV_i}$ for each loop.

The configuration of pragma which has the minimal lower bound and which respect $R_{used}^{min} \leq R_{op}$ is the lower bound of the kernel.


\end{theorem}


% \begin{proof}[Proof Th \ref{th:minlatpipelineunderresourceconstraint}]

%     According to Theorem \ref{th:minresource}, $R_{used}^min$ is the minimal number of DSP a configuration can use. Hence, all configuration which does not respect the constraint $R_{used}^min \leq R_{op}$ have a over-utilization of the resource and hence are invalid.

%     Hence, the minimal lower bound of each configuration of pragma is the lower bound of the kernel.
    
% \end{proof}

%   
